Technical Design Report of the Spin Physics Detector at NICA

The Spin Physics Detector collaboration proposes to install a universal detector in the second interaction point of the NICA collider under construction (JINR, Dubna) to study the spin structure of the proton and deuteron and other spin-related phenomena using a unique possibility to operate with polarized proton and deuteron beams at a collision energy up to 27 GeV and a luminosity up to $10^{32}$ cm$^{-2}$ s$^{-1}$. As the main goal, the experiment aims to provide access to the gluon TMD PDFs in the proton and deuteron, as well as the gluon transversity distribution and tensor PDFs in the deuteron, via the measurement of specific single and double spin asymmetries using different complementary probes such as charmonia, open charm, and prompt photon production processes. Other polarized and unpolarized physics is possible, especially at the first stage of NICA operation with reduced luminosity and collision energy of the proton and ion beams. This document is dedicated exclusively to technical issues of the SPD setup construction.

==> Makefile <==
MAINFILE=SPD_CDR
TEXFILES=$(wildcard *.tex) \
         $(wildcard ./*/*.tex) \
         $(wildcard ./*/*/*.tex)
INCFILES=$(wildcard *.tex)
AUXFILES=$(patsubst %.tex, %.aux, $(INCFILES)) 
#AUXFILES=$(wildcard *.aux)
BIBFILES=$(wildcard ./bib/*.bib)
BBLFILES=$(patsubst %.tex, %.bbl, $(INCFILES)) 
#BBLFILES=$(MAINFILE).bbl
FIGFILES=$(wildcard ./fig/*.pdf) \
         $(wildcard ./fig/*.jpg) \
         $(wildcard ./fig/*.png) 

export TEXINPUTS=.:./sty:./tex:./bib:$TEXINPUTS:
export BSTINPUTS=.:./sty:$BSTINPUTS:
export BIBINPUTS=.:./bib:$BIBINPUTS:

all:	$(MAINFILE).pdf

test:
	@echo ``TEXFILES:'' $(TEXFILES)
	@echo ``INCFILES:'' $(INCFILES)
	@echo ``AUXFILES:'' $(AUXFILES)
	@echo ``BIBFILES:'' $(BIBFILES)
	@echo ``BBLFILES:'' $(BBLFILES)
	@echo ``FIGFILES:'' $(FIGFILES)

emacs:
	emacs $(TEXFILES) &

$(MAINFILE).pdf: $(MAINFILE).tex $(FIGFILES) $(TEXFILES) $(BBLFILES)
	@echo "============ Main LaTeX pass ============"
	-pdflatex --shell-escape $(MAINFILE) 
	pdflatex --shell-escape $(MAINFILE) 
#	pdflatex --shell-escape $(MAINFILE) 

%.bbl:	%.aux 
	@echo "============ BibTeX pass ============"
	-bibtex $(patsubst %.aux,%,$^)

#%.bbl: %.tex $(BIBFILES)
#	-bibtex $(MAINFILE)

%.aux: 	%.tex
	@echo "============ TEX -> AUX pass for" $@ "============" 
	-pdflatex --shell-escape $(MAINFILE) 

clean:
	@echo "============ Cleaning ============" 
	-rm -rf *.aux *.blg *.bbl *.log *.out *.toc *.lof *.brf

distclean: clean
	@echo "============ Thorough cleaning ============" 
	-rm -rf $(MAINFILE).pdf *~

.PRECIOUS: %.bbl %.aux

.PHONY: clean distclean test all emacs



==> tex/TDR_Aerogel.tex <==

\chapter{Aerogel counters}
For particle identification in the end-cap regions, it is proposed to install threshold Cherenkov
aerogel counters (in addition to another PID detector, MRPC). This will extend the momentum range of $\pi$/K/p separation compared with
the TOF detectors of SPD.

\section{Aerogel properties and production}
Aerogel, first synthesized by S.S.Kistler in 1931, is a highly porous material of silica clusters with a micro-structure smaller than the wavelength
of visible light. The first successful attempt to use silica aerogel in Cherenkov counter was made in 1974 \cite{Cantin:1974ci}.
This material is ultra-light and contains more than 90\% air inside a volume.
The complicated and prolonged process of the aerogel production includes two main stages:
forming of gel in the medium of a corresponding solvent, and drying at the super-critical conditions
of  high pressure and density.

The technology of the aerogel production is well mastered at present in two centers: one in Japan (KEK/Chiba/Panasonic groups),
another one in Russia (Budker INP and Boreskov Institute of Catalysis, Novosibirsk).

Aerogel has found an application,
in particular, as a radiator in Cherenkov counters. Actually, aerogel fills the gap in the refractive index values
between gases and liquids.  This feature of aerogel allows one to use it in Cherenkov counters
for particle identification in conditions when other Cherenkov radiators are not applicable,
for instance, for $\pi$/K separation at the momenta from a few hundred MeV/c to about 3\,GeV/c.
Aerogel may have a refractive index in the range between 1.0006 and $\sim$1.25, the refractive index for various density aerogel materials is roughly given by $n = 1 + 0.21 \rho$.
The exact value of $n$ is specified at the production stage.
Selection of the refractive index value defines the region of momenta where separation is
effective. The momentum threshold $P$ of a particle with mass $m$ is given by $P= m/\sqrt{n^2 -1}$. Table \ref{thresholds} shows the threshold momenta of particles for different $n$ values.

\begin{table}
  \begin{center}
\caption{\label{thresholds} Threshold of Cherenkov radiation in GeV/c for different particles and refractive indices $n$ of aerogel.}

\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
 $n$ & 1.05  & 1.04 & 1.03 & 1.02 & 1.015 & 1.01 \\ \hline \hline
$\pi$    & 0.44  & 0.49 & 0.57 & 0.70 & 0.80  & 0.99 \\ \hline
$K$      & 1.54  & 1.73 & 2.00 & 2.46 & 2.84  & 3.48 \\ \hline
$p$      & 2.93  & 3.29 & 3.80 & 4.67 & 5.40  & 6.62 \\ \hline
\end{tabular}
  \end{center}
\end{table}

Aerogel has a short scattering length of light, 12$\div$40\,mm depending on wavelength. Therefore,
the directivity of Cherenkov light cannot be used because directivity disappears soon after emission. For this reason,
diffusive reflectors are used at the walls. No scintillation has been observed in aerogel. No detectable degradation of the optical properties of the aerogel (transmittance, refractive index) was observed up to radiation doses of $\sim$10\, Mrad \cite{Sumiyoshi:1999sy}. Aerogel samples
suffered from hygro\-scopicity for a long time, but in the 1990s the technology of hydrophobic aerogel has been developed.

Aerogel is manufactured in the form of tiles with dimensions up to 20$\times$ 20 $\times$ (1 $\div$ 5)\,cm$^3$. If a thicker radiator is needed,
it is arranged as a stack of a few tiles. In order to put tiles into a needed shape, mechanical treatment is done with a diamond saw
or with a water-jet cutter.

There exists a positive experience of using threshold aerogel Cherenkov counters, in particular,
in experiments KEDR (BINP, Novosibirsk) \cite{KEDR-JINR}, \cite{KEDR-NIM}, BELLE (KEKB, Tsukuba) \cite{Iijima:2000uv, Belle:2000cnh},
DIRAC \cite{Allkofer:2008zz}.
In the BELLE experiment a threshold aerogel Cherenkov counter with refractive index from 1.010 to 1.030
provided $\pi$/K separation in the momentum region up to 3.5 GeV/c. In the KEDR detector, the aerogel counters
with refractive index 1.05 provided $\pi$/K separation in the range from 0.6 to 1.5\,GeV/c. In DIRAC aerogel radiators
with refractive indices 1.015 and 1.008 were used, the resulting amplitudes for kaons were on average 6.9 photoelectrons
in the momentum range 4.0$\div$5.2\,GeV/c (for n=1.015) and 3.9 p.e. for momenta 6$\div$8\,GeV/c (for n=1.008).

In SPD, to extend to higher momentum values the region of $\pi$/K identification, compared with provided by the TOF system,
we have to use a rather low refractive index, below the most commonly used $n=1.05$. 
 On the other hand, the lower the value of the refractive index, the lower the Cherenkov photon output, which is proportional to 
 {\em n-1}.

As is well known, the maximum of the Cherenkov light emission spectrum lies in a short-wave region, below the visible light.
Light absorption length in aerogel decreases with decreasing of the wavelength, and below $\lambda$=300\,nm it drops
very sharply. Therefore, it is needed to shift the original Cherenkov light to larger wavelengths, to a region of
maximum sensitivity of light detectors (PMT, APD, MPPC).

In Fig.~\ref{ashiph}(a) the principle of the KEDR aerogel counter (ASHIPH) operation is shown.
Cherenkov light from aerogel is captured by a wavelength shifter (WLS) and leads it to a light sensor.
Fig.~\ref{ashiph}(b) shows the drawings of the KEDR counter.
A PMMA light guide doped with BBQ dye is used as a wavelength shifter. BBQ has 250--430\,nm absorption band, and $\lambda$=500\,nm
emission peak, Fig.~\ref{BBQspectra}(a), which matches a sensitivity region of many light sensors. Cross-section of WLS is 3$\times$17\,mm$^2$.
The microchannel plate photomultipliers served as light sensors in KEDR, but for later developments the APDs were used (BELLE-II),
also, SiPMs were proposed for aerogel detectors in PANDA (GSI) and FARICH (c$\tau$-factory in Novosibirsk).

\begin{figure}[!ht]
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{ashiph-pic2} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{aship-KEDR-2} \\ (b)}
  \end{minipage}
  \caption{(a) Principle of ASHIPH operation.
  	(b) KEDR aerogel counters: two barrel counters in a single housing (left), end-cap counter (right) \cite{KEDR-JINR}.
	}
  \label{ashiph}
\end{figure}

\begin{figure}[!ht]
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{BBQ} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{tiles-layer-2.pdf} \\ (b)}
  \end{minipage}
  \caption{(a) Absorption and emission spectra of the BBQ wavelength shifter.
  	(b) Aerogel layer composed of tiles.
	}
\label{BBQspectra}
\end{figure}


If a particle crosses WLS, it produces a signal much higher than a particle traversing aerogel.
To avoid misidentification, a two-layer structure is used with shifted layers with respect
to the WLS position, so that a particle cannot cross WLS in both layers. The thickness of one layer in KEDR
is 74\,mm, the total amount of material in both layers is 0.24 $X_0$.

For relativistic cosmic muons that cross both counter layers of KEDR, the average number of photoelectrons was $9.3 \pm 0.4$,
and the detection efficiency $99.3 \pm 0.1$\% at the threshold equal to 2 p.e. For under-Cherenkov-threshold muons ($200 < p_{\mu} < 300$ MeV/$c$)
the efficiency was $3 \pm 1$\%.


\section{Aerogel detector in SPD}
In the SPD a threshold aerogel counter in SPD, similar to the one used in the KEDR experiment, can be inserted between the ST end-caps and the Beam-Beam Counter. The available gap is 200\, mm.

The value of the refractive index has to be selected for the momentum region where $\pi$/K separation with the TOF system
becomes less reliable, that is above 1.5\,GeV/c. This requires rather low $n$ values.
At the same time, the Cherenkov light output drops with decreasing refractive index, therefore, some compromise is needed.

As was illustrated in SPD CDR (Fig. 4.38 (d) in SPD CDR \cite{SPD:2021hnm}), refractive index $n=1.02$ allows for $\pi$/K separation in the
region of momenta from 1 to 2.5\,GeV/c. From a numerical estimation, it follows that in aerogel with $n=1.02$ a relativistic particle
produces 30 Cherenkov photons per cm in the wavelength range 250$\div$430\,nm (this is just an absorption band
of the wavelength shifter BBQ).

The plan is to build the end-cap aerogel detector consisting of two layers with a shifted position of the wavelength shifters in each layer with respect to each other.
Each layer has 80\,mm thickness, the surface of a layer is composed of 32 rectangular aerogel tiles of different dimensions up to 200$\times$470\,mm$^2$ as shown in Fig.~\ref{BBQspectra} (b).
The innermost tiles are machined so that their form fits a circular beam pipe.

WLS is made of polymethylmethacrylate with a BBQ dye. It extends along the full length of a tile and has a 3$\times$14\,mm$^2$ cross-section, with a long side (14\,mm) along the $Z$ direction. With a 3\,mm thickness of a WLS bar, the Cherenkov photons are re-emitted with about 100\% probability. An output surface of the shifter (3 $\times$14\,mm$^2$) is attached to two  MPPCs Hamamatsu S13360-6075, each having  a 6$\times$6\,mm$^2$ photosensitive area, 50\% photon detection efficiency and  a high gain  (4$\times 10^6$), Fig.~\ref{hamamatsu} (a).  Another option is to use four MPPCs  S13360-3060 with a 3$\times$3\,mm$^2$ sensitive area, and  a 40\% photon detection efficiency. We are planning to collect light from both ends of a shifter bar. Low noise of the photosensors is an important condition for  a clear detection of weak Cherenkov signals.

In KEDR the probability of a Cherenkov photon conversion into a photoelectron was 2\%-4\%, depending on the distance between the point of a photon absorption and a light sensor, ranging between 5 and 40\,cm. This was achieved with MCP of 23\% quantum efficiency and one-end light collection. In SPD, light collection from both ends and higher quantum efficiency of MPPC (40\% or 50\%), though with a shorter long side of WLS (14\,mm instead of 17 in KEDR), would allow to reach not less than  about 4\% conversion efficiency. Then, with 30 Cherenkov photons per cm and 8\,cm aerogel thickness, a total of 240 Cherenkov photons would produce about 10 photoelectrons.

The position of the shifters is seen from Fig.~\ref{hamamatsu}~(b). WLS bars in adjacent tiles are slightly shifted in order to avoid collision of MPPCs.
The probability for a particle to hit the shifter in one layer is about 3~mm/200~mm $\approx$2\%, a high signal, in this case, may lead to misidentification.
The second layer of the aerogel detector has the same structure, but the WLS are shifted so that a particle cannot hit WLS in both layers, thus excluding misidentification. Horizontal gaps of a few millimeters between the tiles serve for placing MPPCs and the connecting cables. Similarly, horizontal gaps in the two layers are shifted so that a particle cannot pass through the gaps in both layers and escape detection. The aerogel volume of each tile is covered with the diffusive reflective material like Millipore paper or Gore\textregistered DRP\textregistered Diffuse reflector which have reflectivity above 97\%.





\begin{figure}[!ht]
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{MPPC.pdf} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{layer-shifter-2} \\ (b)}
  \end{minipage}
  \caption{(a) Drawings of the MPPC Hamamatsu S13360-6075.
  	(b) Wavelength shifters (blue) and light sensors MPPC (red) in the aerogel layer.
	}
\label{hamamatsu}
\end{figure}

\begin{table}[h]
  \begin{center}
\caption{\label{aerogeltab}
Aerogel detector components and cost estimate.}
\begin{tabular}{|l|l|l|l|l|} \hline
Component & Units & Quantity & Price per unit, \$ & Total price, k\$  \\ \hline \hline
Aerogel   & {\em l}    & 800       & 2500                 & 2000 \\ \hline
Reflective &           &           &                    & \\
material   & m$^2$     & 40        & 1000           & 40 \\ \hline
WLS       & pc   & 128       & 150                  & 20 \\ \hline
MPPC      & pc   & 1024       & 40                   & 40   \\ \hline
Electronics & channels & 256 & 150                  & 40 \\ \hline
Mechanics &      &           &                      &      \\
and assembling & &           &                      & 260  \\ \hline
Total & &     &                       & 2400  \\ \hline
\end{tabular}
  \end{center}
\end{table}

The electronic channel of the aerogel counter consists of an amplifier and a digital part. The amplifier should include the summing of the analog signals of all (2 or 4) MPPCs at the end of a shifter. The digital part may be arranged similar to that of the electromagnetic calorimeter of SPD. Only MPPCs are positioned at the front view of the aerogel layer, the amplifiers and digital electronics can be placed outside of the aerogel aperture.

Rectangular tiles leave empty areas at the outer region of a circular aperture of the end-cap, this results in 10\% geometrical inefficiency, which is quite affordable, especially since it happens at the periphery of the end-cap. In principle, we could fill these empty areas with aerogel, too, but at the moment we do not consider this obligatory.

One end-cap includes two aerogel layers with 32 tiles in each layer. When WLS is viewed from both ends, the number of the electronic channels in one end-cap will be 2 (layers) $\times$ 32 (tiles)  $\times$ 2 (ends) = 128, or 256 channels for both end-caps. The number of MPPCs is 256  $\times$ 2 (4) = 512 (1024) depending on the selected MPPC type. Table ~\ref{aerogeltab} summarizes information about the SPD aerogel detector and the cost estimate. Thus, the cost of two aerogel end-caps is estimated at 2.4 M\$.


==> tex/TDR_Assembling.tex <==
\chapter{Setup assembling}

==> tex/TDR_BBC.tex <==
\chapter{Beam-Beam Counter}

\section{Local polarimetry with beam-beam counters}

The main goal of the local polarimetry at SPD is  the permanent monitoring of the beam polarization during data 
taking to reduce the systematic error coming from the beam polarization variation.  
Another task for the local polarimetry at SPD  is  
monitoring of the beam polarization, the independent from the major polarimeters (CNI and absolute), and possible usage of this tool to tune
the beam polarization axis.  

The energy range of SPD (below $\sqrt{s}$=27~GeV) is new, therefore, there is a lack of the polarization data to find an explicit solution for the local polarimetry.   
One of the methods to control the proton beam polarization is the measuring of the azimuthal asymmetry in the inclusive production of charged particles in collision of transverse polarized proton beams.
Such a method is well adopted  at the STAR detector. 
Two Beam-Beam Counters (BBCs) are  used for this purpose. 
%Each BBC consists of two parts, inner and outer, corresponding to  a different rapidity range. The inner and outer parts have different positions along the beam line and technically they are different detectors. This Chapter is devoted to the outer part of the BBC while the inner, MCP-based part, is described in Chapter \ref{Ch_pipe} together with the beam pipe  to which it adjoins.
%The inner and outer zones cover 
%3.3$<|\eta|<$ 5.0  and 2.1$<|\eta|<$3.3, respectively. 
BBCs detect
all the charged particles produced in the forward direction within their acceptance. 
The measurements by BBCs at STAR are sensitive to  the transverse polarization of the colliding beams.  The value of the effective analyzing power $A_N$ for the inclusive production of charged particles at $\sqrt{s}$= 200~GeV is about $(6\div 7)\times$10$^{-3}$. At NICA energies,  we could expect, in principle, the same or even larger value, due to a larger analyzing power for the $p$-$p$ elastic scattering. Therefore, the BBC can be used for the local polarimetry at SPD. 
%The design of SPD BBCs  is described previously. 


\section{Beam-Beam Counters}

Two Beam-Beam Counters (BBCs) are planned to be located  in front of the TOF system in the end-caps of the SPD setup \cite{SPD:2021hnm}. 
%The detector should consist of two parts: the inner and the outer one, 
%which are based on different technologies.
 Schematic view of the SPD Beam-Beam Counter, produced from  the tiles of fast plastic scintillator, is presented in  Fig.\ref{baldin_fig00}.  
 Each detector has 80 large pads in 5 radial layers while the internal ring is subduivided into 32 sectors (not shown in the Figure).
 The BBC will cover the polar angles between 60 and 500 mrad, it will be divided into
 6 concentric layers with 16 azimuthal sectors in each of them. The final granularity is the matter of further optimization for the entire energy range of collisions at SPD.  
%The inner part of BBC will use fast, segmented MicroChannel Plate (MCP) detectorsectors.s and should operate inside the beam pipe,
%while the BBC outer part will be .


\begin{figure}[!h]
  \begin{minipage}[ht]{1\linewidth}
    \center{\includegraphics[width=1\linewidth]{BBC_new}}
  \end{minipage}
  \caption{Schematic view of the SPD Beam-Beam Counter.}
\label{baldin_fig00}
\end{figure}

%The inner part covers the acceptance  of  30$\div$60 mrad and should be separated into 
%4 layers consisting of 32 azimuthal sectors. The outer part, covering the polar angles between 60 and 500 mrad, will be divided into
%5 or 6 concentric layers with 16 azimuthal sectors in each of them.

%The concept of the BBC is shown in Fig.\ref{baldin_fig0}. The magenta part represents the MCP detector while the internal layer of the outer part is shown in red.


%\begin{figure}[!h]
%  \begin{minipage}[ht]{.9\linewidth}
%    \center{\includegraphics[width=1\linewidth]{sector}}
%  \end{minipage}
%  \caption{Beam-Beam Counter: azimuthal and polar angle segmentation. All dimensions are in millimeters.}
%\label{baldin_fig0}
%\end{figure}

        The main goals of the Beam-Beam Counters are: i) the local polarimetry at SPD, based  on  the measurements of the azimuthal asymmetries in the inclusive production of charged particles in the collisions of transversely polarized proton beams, ii) the monitoring of  the beam collisions, and iii) participation in the precise determination of the collision time $t_0$ for events in which other detectors can not be used (for instance, in  the case of elastic scattering).



Another important goal of BBCs is fast preselection of different types of events for monitoring purposes. 
The Monte Carlo simulation shows that in the $p$-$p$ collisions at $\sqrt{s}$=27~GeV   
at least one BBC should have a signal in 79\% of events (51\% of events has a signal in the both BBCs).
%However, for the hard processes a one and both BBCs will be hitted in 97\%  and  68\% of cases, respectively. 
However, for the hard processes,   in 97\% of events  the only one  
BBC will be hit, while   hits  for both counters could be expected in 68\% of cases.
Therefore, the requirement of the BBC signals allows one to preselect hard processes. 

 The  BBC will consist of  the tiles viewed by the SiPMs. The measurement of the signal amplitude is required for the time-walk correction to improve the time resolution. 

\subsubsection{First R\&D results for FEE}

\begin{figure}[!t]
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{ladygin_tot} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{BBC_tot} \\ (b)}
  \end{minipage}
  \caption{ (a) Schematic view of the front-end electronics with a ToT function,
 (b)  Distribution of the ToT for different LED signal amplitudes. }
\label{ladygin_fig1}
\end{figure}


With a single-channel prototype of the detector, we will be able to measure the amplitude using the developed FEE based on the Time-over-Threshold (ToT) technique. This technique is a well-known method that allows us to measure the energy deposited in the material by reconstructing the given property of the output current pulse -- the total charge collected, the pulse amplitude, etc. The ToT method converts the signal pulse height into a digital value in the early stage of the FEE, which greatly simplifies the system in comparison to analog detectors with serial readout through ADCs. The measurement of the ToT is composed of two measurements of time for the signal going above (leading) and returning below (trailing) the given threshold. The first version of the prototype includes a power supply and electronics 
(Fig. \ref{ladygin_fig1} (a)) made on a separate PCB  used for  a single SiPM. The power supply for the SiPM 
provides a voltage of up to 65 V with an individual channel adjustment within 0$\div$10 V, manual tuning, and a built-in voltmeter for the voltage monitoring.
It is possible to connect eight PCBs simultaneously. The amplifiers used for that do not change the leading edge of the signal. This allows us to get a time stamp of the event. Afterwards, the signal is integrated and transmitted to the comparator.
\begin{figure}[!t]
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{BBC1} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{BBC4} \\ (b)}
  \end{minipage}
  \caption{ (a) $dT$ ($T_{SiPM1} - T_{SiPM2}$) correlation on the ToT.  
 (b) Result after the time-walk correction for the 
$dT$ ($T_{SiPM1} - T_{SiPM2}$) correlation on the ToT. }
\label{ladygin_fig2}
\end{figure}


\begin{figure}[!t]
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{BBC2} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{BBC3} \\ (b)}
  \end{minipage}
\caption {(a) $dT$ ($T_{SiPM1} -T_{SiPM2}$).  
 (b) Result after the time-walk correction for the 
$dT$ ($T_{SiPM1} - T_{SiPM2}$).}
\label{ladygin_fig3}
\end{figure}

The response of the Hamamatsu S12572-010P SiPM \cite{hamamatsu_tot} with the FEE to the LED has been studied. A separate board with internal generator with controlled frequency and amplitude for LED  has been used \cite{hvsys_LED}.  The NIM synchropulse from this board 
was  used  as a trigger.    The illumination was performed  by uniform light with different amplitudes in a light-isolated box. 
In addition to the ToT information (Fig. \ref{ladygin_fig1} (b)), the time stamp of the event for each SiPM   was investigated. The distribution (Fig. \ref{ladygin_fig2} (a)) shows the correlation of these values and that the signal in the region of small amplitudes comes later in time. This is due to signal latency (the so-called time-walking effect). This delay occurs due to the difference between the time when a photon or a charged particle passes through the detecting element and the time when the electronics register this signal. This leads to deterioration in the time resolution.  After performing the correction (see Fig. \ref{ladygin_fig2} (b)), the time-walking effect has been removed \cite{FEEtot1}.


The time resolution was defined as the RMS and was approximately 600 ps. Taking into account the non-Gaussian distribution (Fig. \ref{ladygin_fig3} (a)) and the fact that the time resolution is not the maximum allowed for this type of the detector, the time-walk correction has been applied.  The most important result of the correction was a time resolution of approximately 400~ps (Fig. \ref{ladygin_fig3} (b)), which is 1.5 times better than the resolution before the correction.

Therefore, the first version of the front-end electronics based on the Time-over-Threshold method was tested with LED. After the time-walk correction, the time resolution improved up to 400 ps. Taking into account the SiPM suboptimal for precise time measurements, the result was promising.
Further development of the FEE with a ToT function allows  us to use standard TDCs for timing
measurements.
 
\subsubsection{Description of the detector prototype and test equipment}

Since the concept of the BBC outer part is  based on highly granular scintillation tiles with SiPM  
readout (SiPM), a prototype of a scintillation detector was developed (see Fig. \ref{ladygin_fig5}) with  two  different types of FEE. Both types are based on the Hamamatsu SiPM readout (S12572-010P) \cite{hamamatsu_tot}.


\begin{figure}[!t]
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{BBC_test} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{BBC_prototype1} \\ (b)}
  \end{minipage}
\caption {(a) Schematic view of tests without a scintillator. (b) Picture of the tests with scintillator.}
\label{ladygin_fig5}
\end{figure}

The initial version of the scintillation detector for tests includes a 40-cm plastic scintillator and ten channels of electronics (Fig. \ref{ladygin_fig5} (b)). To increase the light collection, the scintillator is wrapped in a mylar film. Holes are made in the film on the upper face of the scintillator for studies related to the position of the source of calibrated light pulses (LED): in the center, in increments of 5 cm in both directions, and several additional holes on each side. Along the side face there is a similar version of electronics with SiPM in the holes: in the center and in increments of 10 cm in both directions. At the ends of the scintillator, one channel of each electronics option was located. In the case of electronics with the ToT function, the second version of the boards was used. This version is characterized by comparator stability and extended operating range.

Testing of the electronics  and the prototype detector was carried out in a light-insulating box (Fig.\ref{ladygin_fig5}(b)), where the temperature during the measurements was 27.1$\pm$0.4 $^{\circ}$C. As a light source, an LED was used.
The synchropulse  from the  LED board \cite{hvsys_LED} was used   as a trigger for a VME-based data acquisition system \cite{isupov_VME}. The system included the FVME-V2.0 controller, digitizing modules TQDC16 and TDC32, and the trigger module TMWR  \cite{afi_VME}. The data collected was processed in the ROOT software package.

\begin{figure}[!t]
  \begin{minipage}[ht]{0.30\linewidth}
    \center{\includegraphics[width=1\linewidth]{FEE_TOT} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{FEE_DANSS} \\ (b)}
  \end{minipage}
\caption { (a) Single-channel FEE board with ToT method. (b) 15-channels FEE board from DANSS experiment \cite{DANSS} (b).}
\label{ladygin_fig6}
\end{figure}


\subsubsection{FEE used for detector prototype}


First type of the  electronics used for the detector prototype SiPM readout 
is the second release of the FEE, based on the ToT method described above. 
The single-channel electronics  are made on a 4$\times$2.5 cm$^2$ printed circuit board 
shown in Fig. \ref{ladygin_fig6} (a). As it was described above, the ToT method itself consists of two time measurements -- the passage of a negative signal below (leading) and the return above (trailing) a given threshold, and allows to measure the charge along the width of the electric pulse.
In addition, the amplifiers were used that  keep the leading edge of the signal.  After the amplifier the signal is integrated and transmitted to the comparator, from where it is outputted to the reading electronics via the LVDS interface. Thus, thanks to the developed electronics board, we have the opportunity to get a timestamp of the event and measure the charge.
The power is supplied by a power supply (PS) with the possibility of simultaneous connection of up to eight channels of electronics. The PS contains a push-button interface, a display and a built-in voltmeter. The bias voltage consists of a constant (38/52/67 V) and  an adjustable part  for each channel (in the range from 0 V to +10 V).

Another FEE option for the prototype detector was the electronics produced by the ITEP group 
for the DANSS experiment \cite{DANSS}.  It has a multi-channel platform created from several printed circuit boards. The first board provides power and communication with the PC via RS-232 and is connected via IDC-34 to a common board, on which 15 electronics boards are installed. Power is supplied in a wider range and consists of a constant (10-65 V) and a bias voltage adjustable for each channel ($\pm$10 V). Each 1.7$\times$1.9 cm$^2$ board contains an offset voltage output for SiPM and an input for the signal. The signal passes through the amplifier and is then outputted via the IDC-34 connector to the reading electronics.
The picture of the 15-channels FEE board \cite{DANSS} is shown in Fig.\ref{ladygin_fig6} (b).

\subsubsection{Test results}

The SiPM response from a light source for two versions of the electronics was investigated in the presence and absence of a scintillator. Histograms of the time difference at different amplitudes of the LED were obtained and analyzed.
Earlier, when testing the first version of the electronics with the ToT function \cite{SPD:2021hnm}, it was revealed that the signal in the region of small amplitudes arrives later in time. 
%This is due to the delay of the signal, often called the "time-walking" effect. This effect 
%occurs due to the difference in the moment of time when a photon or a charged particle passes 
%through the detecting element and the moment of time when the electronics register this 
%signal. This leads to a deterioration of the time resolution. In this regard, the method of 
%correction of time spectra described in \cite{FEEtot1} was proposed.

\begin{figure}[!t]
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{Tish2021_fig1} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{Tish2021_fig2} \\ (b)}
  \end{minipage}
\caption {$T_{SiPM1}$ - $T_{SiPM2}$ histogram after "time-walking" correction for tests of FEE with the ToT function \cite{Tish2021} in the case of: absence of a scintillator (a); presence of a scintillator (b).}
\label{ladygin_fig7}
\end{figure}


\begin{figure}[!t]
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{Tish2021_fig3} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{Tish2021_fig4} \\ (b)}
  \end{minipage}
\caption {$T_{SiPM1}$ - $T_{SiPM2}$ histogram after "time-walking" correction for  tests of the DANSS exepriment FEE \cite{DANSS} in the case of: absence of a scintillator (a); presence of a scintillator (b).}
\label{ladygin_fig8}
\end{figure}

The proposed correction is relevant when comparing time spectra in the presence and absence of a scintillator. Figures \ref{ladygin_fig7}  and  \ref{ladygin_fig8} show the difference in the arrival times of the $T_{SiPM1} - T_{SiPM2}$ signals for the SiPMs placed at the prototype end-caps after applying the correction. The distributions were approximated by the Gaussian function, and the time resolution was determined as a parameter of the sigma ($\sigma$) Gaussian function. It can be seen from the figures that in the presence or absence of plastic scintillator for two types of the electronics, the time resolution is almost invariable.
When comparing the front-end electronics with the ToT function and the DANSS experiment, the time resolution was approximately 130 ps and 225 ps, respectively.

Therefore, the developed second version of the front-end  electronics with the ToT function demonstrated good performance during LED tests.
Two options of the FEE  have been tested: with the ToT function and the electronics of the DANSS experiment with SiPM readout manufactured by Hamamatsu (S12572-010P).
The difference in the time resolution for both FEE options was found to be approximately 40\%.
A prototype of a scintillation detector was manufactured and tested. 
The proposed prototype is an important step in the development of the BBC subsystem. Given the suboptimality of the SiPM used for accurate time measurements, the result is promising.

%\newpage

\subsubsection{Cost estimate}

The cost estimate of the BBC outer part is presented in Table~\ref{table:BBC}.
The FEE and digitizers cost is estimated based on the options used
for the tests.

\begin{table}[hbt]
\centering
\caption{The cost estimate of the BBC outer part.
\label{table:BBC}}  
 
\begin{tabular}{|l|c|c|}
\hline\hline
 Item &  number & cost, k\$ \\
\hline
Fast BC-404 scintillators  &     250 &  25 \\
SiPMs  &    500 &  25 \\
Composite frames &   2  &  20   \\ 
FEE   & 500 &   50 \\
Digitizers & 12  &  36 \\
Cables, WLS etc.&  & 12 \\
LED boards & 32  & 10 \\
Assembling, tests    &  & 30 \\
\hline 
Total     &  &   208 \\     
\hline         
\end{tabular}
\end{table}
 
\begin{comment}
\section{MCP part}
Two compact detector systems are proposed to meet the challenges of the fast beam-beam collisions monitoring, event selection and the precise timing determination in proton-proton and nucleus-nucleus collisions at NICA. A Beam Position Monitor (BPM) and Fast Beam-Beam Collision (FBBC) monitor are capable to provide the information for each bunch crossing both on the beams location and on the intensity of collisions, as well as on the azimuthal distribution of the particles in the event. The systems use fast Micro Channel Plate detectors (MCPs). The ultra-high vacuum (UHV) compatibility and low-mass compact design of the BPM and FBBC components allow one to consider their application inside the vacuum beam line of the NICA collider. The BPM is based on the effect of the residual gas ionization and provides high accuracy, fast, bunch-by-bunch measurements of the beam position. FBBC uses the concept of the fast isochronous timing for the multi-pad readout of short ($\sim$ 1 ns) MCP signals, produced by the particles in the collisions of the beams. Studies of the polarization phenomena in light- and heavy-ion interactions at SPD NICA is one of the goals of research at NICA, and FBBC is also considered for the local polarimetry at SPD. 

Two compact systems based on MCPs are proposed for the fast beam-beam collisions monitoring, event selection and determination of the precise timing signal ($t_0$) of the collisions, see Fig. \ref{baldin_fig1}. These systems of monitor detectors consist of 2D position-sensitive beam imaging detectors (BPM) and two ring beam-beam collision detectors (FBBC-left and FBBC-right) that are situated inside the vacuum beam line.

\begin{figure}[!h]
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{B1_1} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{B2} \\ (b)}
  \end{minipage}
  \caption{ (a) General layout: the Fast Beam-Beam Collision (FBBC) monitor composed of MCP discs (1 and 2) in combination with the Beam Position devices (BPM) (3 and 4) are situated symmetrically with respect to the Interaction Point (5) inside the vacuum beam line of the NICA collider.
(b) Compact module of the Fast Beam-Beam Collision Monitor (FBBC) based on circular MCPs. Sector cathode readout pads and two MCP setups are embedded into a separate flange with a hermetic 50-$\Omega$ signal and HV feedthroughs (the latter are not shown).}
\label{baldin_fig1}
\end{figure}

The ultra-high vacuum (UHV) compatibility and low-mass compact design of the Fast Beam-Beam Collisions (FBBC) monitor in combination with the Beam Position device (BPM) \red{[???10]}, allow their application inside the vacuum beam line of NICA collider. 
\begin{figure}[!h]
\begin{center}
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{bald3}}
  \end{minipage}
  \end{center}
  \caption{ A typical MCP signal the detector  prototype. }
\label{baldin_fig2}
\end{figure}
FBBC uses the concept of the isochronous multi-pad fast readout and the precise timing determination of short ($\sim$ 1 ns) MCP signals. New MCPs with the improved characteristics, such as small diameter (6-12 $\mu$m) channels, low resistivity (100-1000 M$\Ohm$), high gain ($\sim$10$^{7}$), short fast rise-time ($\sim$ 0.8 ns) signals, will be used.
	The colliding beams pass through the central opening of the MCP, and the outer edges of the MCP capture secondary particles flying some definite distance from the interaction point (IP). Signals are recorded at 12 sector cathode and their arrival times are digitized along with the multiplicity information. 
	The main feature of the new MCP is a high secondary emission coefficient and fast fronts of the output signal. The new MCPs have a fast leading edge and high gain.

A compact set of two detectors with high timing capabilities based MCs -- the Fast Beam-Beam Collision counters (FBBC) and the Beam Position Monitor (BPM), is proposed to meet the wide range of requirements including those of the future physics program with polarized beams at SPD NICA .

The feasibility of the event-by-event monitoring of the beam-beam interactions at NICA is confirmed both by the previous developments of the UHF-UHV technology and by the beam tests at JINR and CERN of the prototype detectors and electronics, as well as by the in-lab tests of new 8-channels MCPs with the improved characteristics.

\begin{figure}[!h]
  \begin{minipage}[ht]{0.44\linewidth}
    \center{\includegraphics[width=1\linewidth]{MCP_1}}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.54\linewidth}
    \center{\includegraphics[width=1\linewidth]{MCP_2}}
  \end{minipage}
  \caption{ Schematic diagram of the BBC MCP detector.}
\label{baldin_fig3}
\end{figure}

\subsection{Testing of the prototype MCP detectors for SPD BBC}
Testing was performed using the system of dynamic diagnostics of the Booster and Nuclotron circulating beams, as well as HILAC beams of the accelerator complex NICA. The objective was to measure the loading characteristics of chevron MCPs with pad-wise signal readout, similar to the design to be implemented in BBC MCP. Signals and loading characteristics of chevron MCP based on PEM TOPAS and PEM SAPFIR were also measured. All microchannel plates were manufactured by VTC ''Baspik'' (Vladikavkaz, Russia). Plates of the following size were chosen for testing: 40$\times$60 mm, 54$\times$54 mm, and circular plates with diameters of 18 mm and 25 mm. The tested plates had different MCP channel diameters: 6, 8, and 12 $\mu$m, and different resistivity in a range from 100 M$\Ohm$ to 1 G$\Ohm$. Signals with a duration not larger than 4 ns and a front of 0.5$\div$1 ns were obtained for all MCP assemblies. Such signals provide a detector time resolution of at least 50 ps. The loading characteristics were studied in a range from single pulses to $5\times10^6$ particles/(cm$^2$ s). Thus, the possibility of application of detectors of this type for BBC SPD was demonstrated. Two configurations are possible: BBC MCP can be installed either in the vacuum volume of the collider chamber or beyond the vacuum beam line in a special vacuumed box. In the case of MCP position out of the collider vacuum volume, the service and replacement of detector elements will be simplified. In this case it is possible to manufacture specialized PEMs with given pad size and geometry for signal readout at VTC ''Baspik''.

A specialized portable vacuum chamber with thin (50 $\mu$m) Ti windows was manufactured for investigation of particle registration efficiency by chevron MCPs in the case of particles with minimum ionizing power; two independent prototypes of MCP detectors can be installed in this vacuum chamber. It is planned to perform full-scale testing of registration efficiency, time resolution, and loading characteristics of such detectors at extracted beams of Nuclotron and electron beams of the linear accelerator LINAC-200 (LNP JINR). Figure \ref{baldin_fig4}(a) shows the photo of the specialized vacuum chamber and its flanges. Figure  \ref{baldin_fig4}(b) shows the MCP installed in the specialized vacuum chamber for testing. Figure  \ref{baldin_fig5} shows the prototype BBC MCP detector mounted in a vacuum chamber.

\begin{figure}[!h]
  \begin{minipage}[ht]{0.36\linewidth}
    \center{\includegraphics[width=1\linewidth]{MCP_3}}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.64\linewidth}
    \center{\includegraphics[width=1\linewidth]{MCP_4}}
  \end{minipage}
  \caption{(a) Prototype MCP detector in the specialized vacuum chamber for testing. }
\label{baldin_fig4}
\end{figure}

The question of high vacuum compatibility of MCP based detectors was answered positively during the latest Booster and Nuclotron run in January, 2022. The two-coordinate profilometer based on MCPs was used to monitor the time evolution of the circulating carbon beam profile and intensity. The profilometer proved capable of operating in ultrahigh vacuum of the beam line and provide information on the circulating beam during the whole cycle from injection into the Booster to transmission into Nuclotron, thus proving that all the applied materials and technologies are appropriate for manufacturing detectors for the NICA collider.

\begin{figure}[!h]
\begin{center}
  \begin{minipage}[ht]{0.79\linewidth}
    \center{\includegraphics[width=1\linewidth]{MCP_5}}
  \end{minipage}
  \end{center}
  \caption{ BBC MCP prototype mounted in a high vacuum chamber.}
\label{baldin_fig5}
\end{figure}

\begin{figure}[!h]
\begin{center}
  \begin{minipage}[ht]{0.99\linewidth}
    \center{\includegraphics[width=1\linewidth]{MCP_6}}
  \end{minipage}
  \end{center}
  \caption{Horizontal (x) and vertical (y) beam profile as a function of time measured using MCP-based two-coordinate profilometer installed in the ultrahigh vacuum beam line of the Booster. The data were obtained in January, 2022.}
\label{baldin_fig6}
\end{figure}

\subsection{Software for data processing}
An important part of experiment preparation at NICA SPD is the development of an adequate software for event reconstruction and analysis.
The possibility of application of MCP-based BBC for determination of the coordinate Z (ion interaction point in an event) by the difference of the times of flight of particles from the symmetrically situated MCP detectors was studied numerically. The Monte Carlo event generator DQGSM was used. One million events of Au+Au collisions at $\sqrt{s}=11$ GeV were simulated. A special library FBBClib was applied. The efficiency of charged particle registration by MCP was taken equal to 90\%, the time tagging precision was 50 ps. The Z coordinate of a vertex event was reconstructed using machine learning, in particular neural networks and the algorithm of gradient boosting on decision trees XGBoost. These methods of machine learning are widely used and have proved quite efficient. Learning samples included the following parameters: average times of particles arrival at separate MCPs, time of first particle arrival at separate MCPs, multiplicity of charged particles, ratios of multiplicities at separate MCPs and total event multiplicity. The neural network included 6 layers: the input layer, the normalization layer, three inner layers with the number of neurons equal to the number of parameters, one summing inner layer, and an output layer. The maximum decision tree depth in XGBoost was equal to 6. All possible detection configurations were considered with an ideal time resolution ($\sigma = 0$ ps) and a realistic time resolution ($\sigma = 50$ ps and 100 ps).
The numerical study showed that the root mean square deviation of event vertex coordinate is on a level of 7 mm and the maximum RMS does not exceed 12 mm even for MCP time resolution $\sigma = 100$ ps.

Another important parameter in collision experiments is the impact parameter. Event-wise estimation of this parameter is crucial for efficient data processing with pre-selection of desirable high centrality events at the data acquisition stage.
The application of neural networks for estimation of the impact parameter from the data obtained from the MCP-based BBC was tried out numerically. Au--Au collisions at $\sqrt{s}=11$ GeV were simulated using QGSM event generator. The simulated data set was divided into the reference and test samples with a ratio of 80/20. The reference sample was used to determination of the weights in the artificial neural network to match the given parameters in the best way. Then the network parameters were fixed and it was applied to processing the test sample. The obtained error matrix provided information on the network operation efficiency. On the whole, the general accuracy of correct event identification in a certain class (part of the detector) was about 80\%. Taking into account that average times of pion and proton arrival are close, an additional possibility of distinguishing between these types of particles would increase the network efficiency. It should also be noted that this approach proved quite efficient for separation between events with large and small impact parameters, demonstrating the highest error in the intermediate interval of impact parameters. For small impact parameters, which are of most interest in collision experiments, an additional binary classifier was constructed. This increased the accuracy of the network operation to 93\%.
Thus, it is possible to use the developed numerical tools for processing experimental data from MCP-based BBC detector at SPD in order to select central collisions both on-line and in post-processing.
\end{comment}




==> tex/TDR_Hall.tex <==
\chapter{Experimental hall}

==> tex/TDR_Infrastructure.tex <==
\chapter{Infrastructure}
\section{Cryogenic system}
The magnetic field is formed by a superconducting (SC) coil. The NbTi superconductor, which has an operating temperature of 4.5 to 9.0 K, has been selected for the SC coil of the detector SPD. Keeping the SC coil in the SC state implies the use of a non-standard cryogenic system operating at 4.5 K. The working substance being gas/liquid helium.
For the SPD magnetic system project, two fundamentally different variants of structures and technical solutions of SC coils are being developed.  One concept is based on the application of a tubular SC cable of the Nuclotron type; this variant is proposed by the JINR LHEP working group (the first variant). To cool the proposed SC coil, supercritical helium is required, which requires the use of a refrigerator-type cryogenic plant.  The second concept implies the use of a Rutherford SC cable and for this SC coil a thermosiphon cooling method is used, which means the use of a liquefier type of cryogenic plant, this variant was proposed by the INP working group (second variant).
The cryogenic helium plant with the input cryostat will be placed on a technical platform, which is moved together with the SPD detector.  The   cryogenic system consists of three main subsystems: helium and nitrogen systems, as well as auxiliary systems. The helium system includes the cryogenic plant, high- and low-pressure helium flow pipelines, and cryogenic flexible pipeline for liquid and vapor helium.  Nitrogen system:  two cryogenic tanks for liquid nitrogen storage, cryogenic pipeline, pipeline for nitrogen vapor. Auxiliary systems: vacuum, measuring, cryogenic monitoring and control system, order gas system and water-cooling system. 
The cryogenic systems for both variants of SC coils will differ in the type of cryogenic plant and the design of the input cryostat.

\subsection{Helium cryogenic system}
\subsubsection{Cryogenic plant for the JINR variant of the SPD magnet}
The concept of the first version of the SC coil requires the use of a cryogenic helium plant of refrigeration type. It has the ability to work with supercritical helium flow and allows slow cooling of the SC coil by helium vapor, at a rate of about 4 K/h, as well as step-by-step cooling of the heat shields. The main operating parameters of the cryogenic plant are given in Table \ref{tab:cryo_1}.

\begin{table}[]
\centering
\caption{Main operating parameters of the cryogenic plant for the JINR option of the magnet.}
\label{tab:cryo_1}
\begin{tabular}{|c|l|c|}
\hline
p. & Operating parameters                            & Unit                                                                \\
\hline
1  & Cooling capacity                                & 100 W \@ 4.5K                                                        \\
2  & Temperature of outlet flow from the SPD         & 4.8 K (2.5 bar)                                                     \\
3  & Temperature of inlet flow from the SPD          & 4.8 K (3.0 bar)                                                     \\
4  & Hydraulic resistance of the SC coil             & 0.5 bar                                                             \\
5  & Cold weight                                     & 7865 kg                                                             \\
6  & Maximum pressure in coil                        & 5 MPa                                                               \\
7  & Mass flow rate                                  & $\leq$16 g/s                                                            \\
8  & Equipment Requirement                           & Maximum reliability,  \\
    & & energy efficiency, \\
    &  & compactness, automatic mode \\
9  & Interval of repair/regulatory work of the plant & Not more than once a year      \\
\hline                                    
\end{tabular}
\end{table}

The plant must have an additional outlet of liquid nitrogen from the nitrogen vessel to provide cooling of the SC coil heat shields, as well as meet all modern solutions in the cryogenic technology. 

The plant includes flexible lines to connect to the input cryostat for transportation of liquid and gaseous helium and nitrogen flows. Maximum heat load for flexible lines: for helium communications is 3 W/m; for nitrogen communications is 5 W/m.  All cryogenic flexible lines and pipelines are vacuum insulated, condensate formation on external surfaces of communications is not allowed. 

The power consumption of the cryogenic plant is 2 kW.

\subsubsection{Cryogenic plant for the Novosibirsk option of the SPD magnet}

The concept of the second variant of the SC coil requires the use of a cryogenic helium liquefaction plant, which allows to cool the SC coil and heat shields with helium vapor, the maximum cooling rate is 1 K/h. This variant uses the thermosiphon method of SC coil cooling. A similar cooling principle and SC coil design is used in such projects of MPD, PANDA, etc. detectors.

\begin{table}[]
\centering
\caption{Main operating parameters of the cryogenic plant for the Novosibirsk option of the magnet.}
\label{tab:cryo_2}
\begin{tabular}{|c|l|c|}
\hline 
p. & Operating parameters                            & Unit                                                                \\
\hline 
1  & Cooling capacity                                & 140 l/h                                                             \\
2  & Temperature of outlet flow from the SPD         & 4.3 K (1.05 bar)                                                    \\
3  & Temperature of inlet flow from the SPD &          4.5 K (1.15 bar)                                     \\
4  & Hydraulic resistance of the SC coil             & 0.1 bar                                                             \\
5  & Cold weight                                     & 3800 kg                                                             \\
6  & Maximum pressure in coil                        & 5 MPa                                                               \\
7  & Maximum heat load                               & 45 W                                                                \\
 8  & Equipment Requirement                           & Maximum reliability,  \\
    & & energy efficiency, \\
    &  & compactness, automatic mode \\
9  & Interval of repair/regulatory work of the plant & Not more than once a year      \\         
\hline                    
\end{tabular}
\end{table}

The plant must have an additional outlet of 50 K helium flow with a smooth adjustable temperature from 297 K to 50 K, to cool the heat shield of the detector SC coil. 
The plant includes flexible lines to connect to the input cryostat for transportation of liquid and gaseous helium flows. The maximum heat load for flexible lines of helium communications is 3 W/m. All cryogenic flexible lines and pipelines are vacuum insulated, condensate formation on external surfaces of communications is not allowed. 
The power consumption of the cryogenic plant is 2 kW.

\subsubsection{Helium pipelines}

The cryogenic system requires pipeline installation along the route from the central cryogenic station to the location of the SPD detector. Figure \ref{lb_cryo_1} shows the routing of the high- and low-pressure helium flows. The total length of the traces is about 220 meters. Pipelines of high-pressure helium flow have a 60 mm diameter and low-pressure helium flow has a 100 mm diameter. The material of the pipelines is stainless steel 12X18H10T or analog. Tracing has the following route. From the room 177 the route goes piping with other communications in one route to room 109/1 (about 120 meters of traces). From the room 109/1 the route goes to the courtyard of building 17 and on the ramp comes to the room 140/2.

The pipelines section from the entrance to room 140/2 to the cryogenic plant is made of flexible lines. Figure \ref{lb_cryo_1} shows the location of the cryogenic equipment on the technical platform and the flexible line. The pipelines have a system of safety devices, to provide safe operation.

\begin{figure}[!ht]
    \center{\includegraphics[width=1.\linewidth]{cryo_1}}
  \caption{ Tracing pipelines of high- and low-pressure helium flows.
	}
\label{lb_cryo_1}
\end{figure}

\begin{figure}[!h]
  \begin{minipage}[ht]{1.\linewidth}
    \center{\includegraphics[width=1\linewidth]{cryo_2} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{1.\linewidth}
    \center{\includegraphics[width=1\linewidth]{cryo_3} \\ (b)}
  \end{minipage} 
  \caption{Flexible lines in the room 140/2 when  SPD is in the ''beam'' (a) and ''servise'' (b) position.
	}
\label{lb_cryo_2}
\end{figure}

\subsubsection{	Nitrogen system}
To provide operation of the cryogenic helium plant it is necessary to create a nitrogen system. The nitrogen system includes the following main elements: two cryogenic storage tanks for liquid nitrogen, cryogenic pipeline and flexible line. 
The system uses two cryogenic tanks each with a capacity of 20 m$^3$, the main technical parameters are presented in Table \ref{tab:cryo_3}.

The cryogenic storage tanks are located on a special foundation to the Building 17 on the side of the room 140/1. 
Liquid nitrogen is supplied through a cryogenic pipeline by raising the pressure to 4.0 bar in the cryogenic storage tank. When the minimum liquid nitrogen level in the first cryogenic storage tank is reached, the control system automatically switches the liquid nitrogen supply from the first cryogenic storage tank to the second cryogenic storage tank.  The cryogenic pipeline is vacuum insulated and condensate formation on external surfaces of communications is not allowed. Total length of the route is about 120 meters. The pipeline is made on a tube-in-tube type, the inner pipeline is 30 mm in diameter, the outer pipeline is 70 mm in diameter. The material of the pipeline is stainless steel 12X18H10T or analog. The route has the following (Figure \ref{lb_cryo_3} shows a preliminary route): from the tanks the pipeline rises to a height of 6 meters for the passage over the road, then along the wall of the building 17, room 140/1, enter the room and bring it to the cryogenic plant. The route has a system of safety devices, to ensure safe operation. 

The discharge of gaseous nitrogen is carried out according to the principle of the shortest route with exit to the atmosphere. The discharge pipelines?s diameter is 70 mm.  Energy consumption of the system is 2 kW.
\begin{table}[]
\centering
\caption{Main technical parameters of the cryogenic storage tank.}
\label{tab:cryo_3}
\begin{tabular}{|c|l|c|}
\hline
p. & Operating parameters                                                                       & Value                        \\
\hline
1  & Overall volume                                                                             & 20 000 l                    \\
2  & Maximum daily evaporation rate depending & 0.17 \%                      \\
    & on pressure 100 kPa and ambient temperature15 $^{\circ}$ C       & \\
3  & Maximum outlet flow rate (nitrogen)                                                        & 600 Nm$^3$ / h                 \\
4  & Maximum operating pressure                                                                 & 1.8 MPa                     \\
5  & Operating pressure range                                                                   & From 1.2 bar to 4.0 bar     \\
6  & Minimum permissible wall temperature (inner vessel)  & 77 K \\
7  & Maximum pressure in vacuum space at T=293 K & 10 Pa \\
8  & Interval of repair / regulatory work of the plant & Not more than once a 7 years. \\
\hline
\end{tabular}
\end{table}%


\begin{figure}[!ht]
    \center{\includegraphics[width=1.\linewidth]{cryo_4}}
  \caption{ Tracing cryogenic pipelines of nitrogen flow.
	}
\label{lb_cryo_3}
\end{figure}

\subsubsection{Auxiliary systems}

Vacuum subsystem provides maintenance of discharged medium in isolation volumes of the cryogenic plant, input cryostat and SC coil cryostat. Maximum pressure value in the isolation volumes at 293 K (before start of cooling) is $1\times10^0$ Pa, maximum pressure value at 4.5 K (after cooling) for the cryogenic plant is $1\times10^{-3}$ Pa, for inlet cryostat and SC coil cryostat is $1\times10^{-5}$ Pa.

The subsystem includes several types of vacuum pumps: rotary vane pumps, Roots pumps, diffusion vapor pumps and turbomolecular pumps. The subsystem equipment is located on the technological platform of the detector SPD. The total power consumption of the subsystem is 14 kW.

Pneumatic valves and valves are used to control technological processes of the cryogenic system, their stable operation is ensured by the ordering of gas. The ordered gas subsystem has the following characteristics: working pressure 6 bar, working gas -- dry air. The system includes: air screw compressor, receiver, moisture separator and various fittings (valves and reducers). Power consumption of the subsystem is 3 kW.

The cryogenic system is controlled by means of data acquisition from all related subsystems (cryogenic unit, helium pipelines, nitrogen system, pneumatic system, vacuum system and data from SC coil control system). Figure \ref{lb_cryo_4} presents a block diagram of cryogenic control system. The control system has automatic circuits with which the following steps are carried out: preparation, cooling of the SC coil, cryostatting at workloads, and heating.
\begin{figure}[!ht]
    \center{\includegraphics[width=0.8\linewidth]{cryo_5}}
  \caption{ Tracing cryogenic pipelines of nitrogen flow.
	}
\label{lb_cryo_4}
\end{figure}

\subsection{Cost estimate}
The cost of the equipment described above and the required capacity are presented in Tab. \ref{tab:cryo_4}.

\begin{table}[]
\centering
\caption{Costs and required equipment capacity}
\label{tab:cryo_4}
\begin{tabular}{|c|l|c|c|}
\hline
p.  & Name of system                           & Cost, k\$ & Power consumption, kW \\
\hline
1.1 & Cryogenic plant (JINR option)  & 3 000     & 2         \\
1.2 & Cryogenic plant (Novosibirsk option) & 3 330     & 2         \\
2   & Helium pipeline                          & 500       & -         \\
3   & Nitrogen system                          & 1 500     & 2         \\
4   & Vacuum subsystem                         & 500       & 14        \\
5   & Pneumatic subsystem                      & 50        & 3         \\
6   & Cryogenic system control                 & 500       & 2         \\
\hline
    & Total (JINR option)                  & 6 050     & 23        \\
\hline
    & Total (Novosibirsk option)                 & 6 380     & 23      \\ 
\hline
\end{tabular}
\end{table}

\section{Gas}
\section{Electricity}
\section{Water}

==> tex/TDR_Lodgement.tex <==
\chapter{Lodgement}

==> tex/TDR_Magnet_2022.tex <==
\chapter{Magnetic system}

A superconducting magnet is one of the most important parts of the SPD setup. Together with the tracking system, it provides the measurement of charged particle momenta with accuracy of about 2\%. The steel elements of the Range System serve as a yoke of this magnet. Two fundamentally different magnet designs were considered in early versions of this document:
 \begin{enumerate}
\item  Novosibirsk project: The use of a Rutherford-type cable made of NbTi/Cu superconductor. The cable will be encased in an aluminum stabiliser using a co-extrusion process that provides a good bond between aluminum and superconductor in order to ensure quench protection during operation. Indirect cooling of the superconductor will be provided by two-phase helium, which will circulate in pipes welded to the outside of the coil former.
\item JINR project: The technology of superconducting coils manufacturing is based on a hollow high-current cable similar to the one used for the Nuclotron magnets or the one used in the ITER systems. The manufacturing technology of the hollow cable made of NbTi/Cu composite wires is well developed at LHEP JINR. The cooling system is supposed to use a single-phase cooling scheme with supercritical helium.
\end{enumerate}
At the meeting on 15.12.24 the SPD Technical Board discussed both options and unanimously adopted the project proposed by the Novosibirsk group.

\section{SPD superconductive solenoid}

\subsection{General performance requirements}

\subsubsection{Magnetic field}
The magnetic field along the solenoid axis should be at least 1.0 T.

\subsubsection{Main dimensions and parameters of the magnet}
The cryostat of the magnet with the coils, cold mass, and thermal shields is located inside the yoke. A distribution box called control dewar is located on the upper octant of the yoke.
The overall dimensions are driven by the area allocated  for the SPD subdetectors and by the magnet field parameters. Outside diameter of the cryostat is 3808 mm, and the gap between the yoke and the cryostat is about 20 mm. 
In the transverse direction, a free space with a diameter of 3308 mm is left for the inner SPD detectors. The length of the magnet is 4080 mm. The magnet should be installed symmetrically inside the yoke (see Fig.  \ref{lb_mag_1}). 

\begin{figure}[!ht]
    \center{\includegraphics[width=1.\linewidth]{mag1}}
  \caption{ The main dimensions of the cryostat and the yoke.
	}
\label{lb_mag_1}
\end{figure}

\subsection{Technical specification of components}
\subsubsection{Magnetic analysis}
The SPD solenoid is designed to provide a magnetic field of 1~T over a length of about 4 m in a bore of 3.2 m. 
In general, the uniformity of the field is not a critical factor. The field variation up to 20\% in the area of the tracking detectors ($|z|<1.4$~m, $r<0.9$~m) is acceptable.
To meet the above requirements, the cold mass design detailed in foresaw splitting of the solenoid in three inter-connected windings, featuring 300, 150 and 300 turns in the upstream, center and downstream coils, respectively.
Two options of the operating current of 4.4~kA and 5.2~kA are considered, which correspond to the value of the field in the center of the magnet 1~T and 1.2~T, respectively.

%The SPD solenoid is designed to provide a magnetic field of 1.0 T over a length of about 4 m in a bore of 3.2 m. 
%The field homogeneity constraints at the center of the solenoid -900 mm $\leq Z \leq $ 900 mm and radius 150 mm uniformity is better than $\pm$2\%. To meet the above requirements, the cold mass design detailed in foresaw splitting of the solenoid in three inter-connected windings, featuring 2$\times$300 and 1$\times$150 turns in the Upstream/Downstream and Center coils, respectively, and an operating current of 4.4 or 5.2 kA.
\begin{comment}
\begin{figure}[!ht]
    \center{\includegraphics[width=1.\linewidth]{mag_8}}
  \caption{ Solenoid layout.
	}
\label{lb_mag_6}
\end{figure}

\paragraph{2D Axially symmetric case}
We considered the following input data for solenoid simulation and optimization.
It was considered the original version with three identical coils of 250 turns each and a current of 6300 A. Arrangement for coils as 250--250--250.
As well as the same arrangement of the side coils was considered, but with half the number of turns in the central coil. That is the arrangement for coils as 250--125--250. 
The uniformity region for $B_z$ component and relation $B_r/B_z$ increases by about 2$\div$2.5 times for the scheme 250--125--250. 

The general solenoid layout is shown in Fig. \ref{lb_mag_6}. 
The uniformity region for $B_z$ component and relation $B_r/B_z$ increases by about 2$\div$2.5 times for the scheme 250--125--250. The uniformity for $B_z$ component within the range $\pm$ 2\% and $\pm$ 4\%  is shown in Fig.\ref{lb_mag_7} (a) and (b), respectively for two  arrangements of cols.  The radial integral is calculated according to the formula 
\begin{equation}
Int =\left\{\left|\int_{z}^{100}\frac{\left.\ Br(r,z\right)}{\left.\ Bz(r,z\right)}dz\right|\right\}\ 
\end{equation}
from the current $Z$ to 100 cm at different radii $r$. The uniformity for $B_r/B_z$  and for radial integrals  for two arrangements of cols: 250--125--250 and 250--250--250 are presented in Fig. \ref{lb_mag_8}.

With arrangement of coils as half turns in central coil (so-called 250--125--250) the uniformity regions had increased for 2$\div$2.5 times wider. As well maximum radial integral value had been reduced from 88 mm down to 30 mm for area 200 cm (Z) ? 100 cm (r). 
Meantime the central magnetic field value had been reduced from 1.16 T for arrangement 250--250--250 down to 0.96 T for arrangement 250--125--250.  
To ensure the value for central field higher than 1 T we have to increase the number of turns in side coils up to 300 and central coil as up to 150. For current 6300 A it comes to central magnetic field value as 1.12 T 
And in conclusion, reducing the number of ampere-turns in the central coil by half compared to the number of amper- turns in the side coils has a positive effect on the quality of magnetic field in terms of increasing the zone of uniformity of the field component $B_z$, the ratio $B_r/B_z$ and also minimizing the radial integral.
In this case, the decrease in the central field by 20\% should be compensated by an increase in the turns in all coils, also by 20\%, respectively, to provide the central field not less than 1.1 T. 
The above considerations were performed for 2D axially case. After analyzing the design of the coil, we came to a more technological version of it, which reflects all the considerations of this section.
This new version was considered in the 3D calculations of the next section.


\begin{figure}[!h]
  \begin{minipage}[ht]{0.53\linewidth}
    \center{\includegraphics[width=1\linewidth]{mag_9} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.47\linewidth}
    \center{\includegraphics[width=1\linewidth]{mag_10a} \\ (b)}
  \end{minipage} 
  \caption{Uniformity for $B_z$ component within the range $\pm$2\% (a) and $\pm$4\%   for two arrangements of cols (all three coils have the number of turns as 250 each and side coils are 250 turns with central one is for 125).
	}
\label{lb_mag_7}
\end{figure}


\begin{figure}[!h]
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{mag_13} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{mag_14} \\ (b)}
  \end{minipage} 
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{mag_15} \\ (c)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{mag_16} \\ (d)}
  \end{minipage} 
  \caption{ Uniformity for $B_r/B_z$ (a), (b) and for radial integrals (c), (d)  for two arrangements of cols: 250--125--250 (a), (c) and 250--250--250 (b), (d), respectively.
	}
\label{lb_mag_8}
\end{figure}
\end{comment}

\paragraph{3D simulation}
The following conditions were applied for the 3D simulation:
the configuration of the superconducting coil and magnetic design according to the latest STEP model with three coils. The coil arrangement is shown in Fig. \ref{fig:coils}.
The current of the coil is 5200 A. Conductor cross-section is 8 mm $\times$ 12 mm. Length of  the side coils is 2$\times$1260 mm, while length of the central coil is 630 mm. 
\begin{figure}[!h]
    \center{\includegraphics[width=1.\linewidth]{Magnet_Fig_5_2}}
  \caption{ %Arrangement of superconductive coils.
  Cross-sectional view of the magnet demonstrating the arrangement of superconducting coils for the basic option with three main coils and without correction coils.
	}
\label{fig:coils}
\end{figure}
\begin{figure}[!h]
    \center{\includegraphics[width=1.\linewidth]{m_coils2}}
  \caption{ %Placement of the correcting coils. 
  Schematic cross-section view of the yoke and coils for the configuration of the solenoid with correction coils.
	}
\label{fig:coils2}
\end{figure}
The calculations were carried out using the MASTAC software package.
Three options were considered:
\begin{enumerate}
\item the basic version with three coils;
\item the correction coils added to the basic version (see Table \ref{tab:coils1} );
\item the central coil is absent to increase the field uniformity.
\end{enumerate}
Figure \ref{fig:coils2} shows the identification of the supercondiucting coils. The ''A'' configuration is a basic three coils arrangement,
 ''B'' and ''C'' are the types of correction coils added. Table \ref{tab:coils2} shows the correction coil designs in terms of the number of layers and ampere-turns. 

\begin{table}[h!]
\caption{Design of the correction coils.}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
Configuration & Coil ''B'' & Coil ''C''   \\
\hline
1   &  2 layers of 60 turns & 2 layers of 60 turns \\
2   &  2 layers of 20 turns & 2 layers of 50 turns \\
3   &  2 layers of 50 turns & 2 layers of 50 turns \\
4   &  2 layers of 40 turns & 2 layers of 40 turns \\
\hline
\end{tabular}
\end{center}
\label{tab:coils1}
\end{table}%

\begin{table}[h!]
\caption{Maximum values of deviations of $B_z(z)$values from $B_z(0)$ in \% at different vertical Y positions.}
\begin{center}
\begin{tabular}{|c|c|c|c|}
 \hline
 & Y=0 m & Y= 0.5 m & Y=1.0 m \\
 \hline
 65$\times$2 & 12.2 & 10.8 & 3.7 \\
  60$\times$2  +   60$\times$2    &  5.7  & 2.9 & 13.7 \\
  20$\times$2  +   50$\times$2    &  9.7  & 8.0 & 3.9 \\                      
  50$\times$2  +   50$\times$2    &  6.6  & 4.2 & 10.1 \\
    40$\times$2  +   40$\times$2    &  8.3  & 6.3 & 5.8 \\
    80$\times$2  +   30$\times$2 +   30$\times$2    &  3.9  & 3.4 & 15.8 \\
\hline
\end{tabular}
\end{center}
\label{tab:coils2}
\end{table}%

\begin{figure}[!h]
  \begin{minipage}[ht]{0.6\linewidth}
    \center{\includegraphics[width=1\linewidth]{m_coils3} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.4\linewidth}
    \center{\includegraphics[width=1\linewidth]{m_coils4} \\ (b)}
  \end{minipage} 
  \caption{%Distribution of $B_z$ magnetic field component (a) and uniformity of this component (b) in the section YZ at X = 0 for coils 40$\times$2 + 40$\times$2. 
  Distribution of the axial component of the magnetic field $B_z$ along the $z$ axis for the magnet configuration with correction coils $40 \times 2 + 40 \times 2$ and the current of 5200~A. (a) shows the absolute value of $B_z$ and (b) shows $B_z$ normalized to its value at $z=0$. Three curves correspond to the displacements $y=0$~m, $y=0.5$~m, $y=1$~m at $x=0$~m.
	}
\label{fig:field_2}
\end{figure}

\begin{figure}[!h]
    \center{\includegraphics[width=1.\linewidth]{m_coils5}}
  \caption{ %$B_z$ component of the magnetic field in the YZ section at X = 0 for correcting coils configuration 40$\times$2 + 40$\times$2.
  Distribution of the $B_z$ component of the magnetic field in the YZ section at X = 0 for correcting coils configuration $40 \times 2 + 40 \times 2$.
	}
\label{fig:field_3}
\end{figure}

Table \ref{tab:coils2} presents the uniformity for simulation of cases described in Table \ref{tab:coils1}. From the data in Table \ref{tab:coils2}, it can be seen that for coils 40$\times$2 + 40$\times$2 the results are optimal. 
This field map can be considered as a reference for estimating the rate of reconstruction in a homogeneous field.

The distribution and uniformity of $B_z$ field component in the section YZ at X = 0 for coils 40$\times$2 + 40$\times$2 are shown in Fig. \ref{fig:field_2} (a) and (b), respectively. The color plot for $B_z$ component is presented in Fig. \ref{fig:field_3}. 

Switching off the central coil in order to reduce its contribution to the central region of the solenoid is considered a potential 
option for improving the field uniformity without the use of the additional correction SC coils. In this case, the uniformity improves up to 10\% (see Figs. \ref{fig:field_4} and \ref{fig:field_5}).
The disadvantage of this method of improving uniformity is the decrease in the solenoid field and, as a consequence, the need to increase the current from 5200 A to 6500 A to achieve 1.1 T at the center of the solenoid.
The distribution and uniformity of $B_z$ in the section YZ at x = 0 for central coil switch off are shown in Fig. \ref{fig:field_6} (a) and (b). The color plot for $B_z$ component for this case is presented in Fig. \ref{fig:field_6}. 

Therefore, the three coils version of Fig. \ref{fig:coils} is the basic variant. 
The distribution and uniformity of $B_z$ in the section YZ at x = 0 for basic version are shown in Fig. \ref{fig:field_6} (a) and (b).

\begin{figure}[!h]
    \center{\includegraphics[width=1.\linewidth]{m_coils6}\\ (a)~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~(b)}
  \caption{ %Distribution of $B_z$ magnetic field component (a) and uniformity of this component (b) in the section YZ at X = 0 for for the central coil switched off and current 6500 A.
  Distribution of the axial component of the magnetic field $B_z$ along the $z$ axis for the magnet configuration without the main central coil and the current of 6500~A. (a) shows the absolute value of $B_z$ and (b) shows $B_z$ normalized to its value at $z=0$. Three curves correspond to the displacements $y=0$~m, $y=0.5$~m, $y=1$~m at $x=0$~m.
	}
\label{fig:field_4}
\end{figure}
\begin{figure}[!h]
    \center{\includegraphics[width=1.\linewidth]{m_coils7}}
  \caption{ $B_z$ component of the magnetic field in the YZ section at X = 0 for the central coil switched off and current 6500 A.
	}
\label{fig:field_5}
\end{figure}
\begin{figure}[!h]
    \center{\includegraphics[width=1.\linewidth]{m_coils8}\\ (a)~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~(b)}
  \caption{ %Distribution of $B_z$ magnetic field component (a) and uniformity of this component (b) in the section YZ at X = 0 for for basic version of three coils and current 5200 A.
  Distribution of the axial component of the magnetic field $B_z$ along the $z$ axis for the basic magnet configuration with three main coils and a current of 5200~A. (a) shows the absolute value of $B_z$ and (b) shows $B_z$ normalized to its value at $z=0$. Three curves correspond to the displacements $y=0$~m, $y=0.5$~m, $y=1$~m at $x=0$~m.
	}
\label{fig:field_6}
\end{figure}


\paragraph{Magnetic forces}

Simulation of the magnetic forces was performed with the Maxwell tensor method from 3D magnetic field data. The results of simulation are shown in Table \ref{tab:mag_forces}. The elements on which the force acts are shown in Figure \ref{fig:field_9}.

Figure \ref{fig:field_10} shows a map of the distribution of magnetic forces acting on one of the door wings. The force values are calculated for the centers of the corresponding grid elements 0.1$\times$0.1 m and displayed in color ranges of 200 Newtons. The results of calculation for magnetic forces acting on the coils during their displacement are shown in Table \ref{tab:mag_forces2}. 

\begin{table}[h!]
\caption{Magnetic forces in kN acting on the elements of the solenoid (1 mm air gap before end-caps).
Calculations were performed for the basic configuration of the magnet with three coils.}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
 Force  com- & Barrel top sector & Barrel top  & End-caps & End- & Central coil (1/8 & Side coil (1.8   \\
ponent & (half along Z) &  sector   &  (half)  &  caps & of top sector)  & of top sector) \\
\hline
X & 0 & 0 & -12.4 & 0 & 0 & 0 \\
Y & -143.8 & -287.6 & 0 & 0 & 658.9 &1185.9 \\
Z & 67.5 & 0 & -694.1 & -1388.2 & 0 & -594.1 \\
\hline
\end{tabular}
\end{center}
\label{tab:mag_forces}
\end{table}%

\begin{figure}[!h]
    \center{\includegraphics[width=1.\linewidth]{m_coils9}}
  \caption{ Schematic view of contour surfaces for force calculation.
	}
\label{fig:field_9}
\end{figure}
\begin{figure}[!h]
    \center{\includegraphics[width=0.7\linewidth]{m_coils10}}
  \caption{ Magnetic forces map for one of the door wings.
	}
\label{fig:field_10}
\end{figure}

\begin{table}[h!]
\caption{Magnetic forces in kN acting on the displaced coils.}
\begin{center}
\begin{tabular}{|c|c|c|c|c|}
\hline
Displacement, mm & Force comp. & Left coil & Central coil & Right coil \\
\hline
\hline
0 & X & 0 & 0 & 0 \\
0 & Y & 0 & 0 & 0 \\
0 & Z & 4748.0 & 0 & -4748.0 \\
\hline
5 in Z & X & 0 & 0 & 0 \\
5 in Z & Y & 0 & 0 & 0 \\
5 in Z & Z & 4521.4 & -69.6 & -4743.4 \\
\hline
5 in Y & X & -2152.8 & -1065.1 & 2152.8\\
5 in Y & Y & 0 & 0 & 0 \\
5 in Y & Z & 4752.8 & -0.3 & -4753.3 \\
\hline
\end{tabular}
\end{center}
\label{tab:mag_forces2}
\end{table}%

\subsubsection{Cold mass with conductor and coil}
The SPD solenoid is designed to operate at a current of 4.4 kA, that is 24\% of the critical current at 4.5 K, and 2.05 T peak magnetic field in the coil and 1.0 T magnetic field in the axis of the solenoid. 

The conductor is a superconducting NbTi/Cu wire-based Rutherford cable, co-extruded with a high purity aluminum-stabilizing matrix. The insulated conductor dimensions at 4.5 K are 10.90 mm in width and 7.90 mm in height. The Rutherford cable is composed of 8 strands with a diameter of 1.40 mm and a Cu/SC ratio of 1.0. The critical current density of the superconductor at 4.2 K and 5 T shall be larger than 2800 A/mm$^2$ to ensure a temperature margin for a quench well above 2.0 K. The same type of the conductor is produced in Russia and used for the PANDA solenoid, FAIR, Darmstadt.

The SPD solenoid consists of three 2-layer coil modules to be wound on a collapsible mandrel. After curing, aluminum alloy support cylinders are placed over each module and the assemblies are epoxy bonded. The pre-assembled modules are then removed from the mandrel to be electrically connected and bolted together to form a single cold mass assembly before installation in the cryostat.

The magnet is indirectly cooled by a network of aluminum alloy cooling tubes, securely bonded to the outer surface of the aluminum alloy support cylinder, ensuring proper heat conduction. During normal operation, two-phase helium is circulated through the cooling tubes by natural convection.

The magnet quench protection system relies on the continuous monitoring of the coil's voltages and the extraction of the energy to an external dump resistor, once a quench is detected. The maximum coil winding temperature and electrical voltage across the coil terminals during a quench has to be limited to 100 K and 500 V, ensuring a robust and extremely low-risk operation, as appropriate for the unique particle detector magnets. Quench propagation across the coil winding is accelerated by using the quench-back effect of the support cylinder, as well as the aluminum heat drains.

The cold mass of the SPD solenoid consists of three epoxy resin impregnated coils, reinforced by shells made of structural aluminum. 

The upstream and downstream winding packs are identical and feature 2 layers of 150 turns. The center coil, instead, is smaller, featuring 2 layers of 75 turns. The conductor is wound around the aperture with a tension. The tension of the conductor is set with tensioning rollers weighing about 50 kg. The coils should be prepared and impregnated in vacuum according to the standard BINP technological scheme TTS4 STO 103-2011.

Figure \ref{lb_mag_2} shows the dimensions of the coil envelopes at room temperature, as computed taking into account thermal shrinkage, shrink fit, and the magnetic field. Note that the dimensions include both cable insulation and ground insulation. 

The cold mass components are shown in Fig. \ref{lb_mag_3}~(a).

\begin{figure}[!ht]
    \center{\includegraphics[width=1.\linewidth]{mag_2}}
  \caption{ Room temperature dimensions in mm of the coil envelopes, including cable and ground insulation.
	}
\label{lb_mag_2}
\end{figure}

\begin{figure}[!h]
  \begin{minipage}[ht]{0.65\linewidth}
    \center{\includegraphics[width=1\linewidth]{mag_3} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.35\linewidth}
    \center{\includegraphics[width=1\linewidth]{mag_4} \\ (b)}
  \end{minipage} 
  \caption{(a) Part of the cold mass cross-section, showing the layout at the end flange. (b)  Cross-section of the solenoid conductor, showing the 8 strands Rutherford cable enclosed by the Al matrix, including sizes and their tolerances.
	}
\label{lb_mag_3}
\end{figure}

\subsubsection{Conductor}
Al stabilized conductors for detector magnets are selected for the following reasons:
\begin{itemize}
\item simplicity of conduction cooling; affordable, since no dynamic operation is needed; quasistationary;
\item simplicity and reliability of electrical connection;
\item high-purity Al stabilized, the residual-resistance ratio (RRR)  $\geq$ 1000, maximum MPZ (m), much larger $\lambda/\rho$ than copper, where $\lambda$ is the mean free path of conduction electrons and $\rho$ is resistivity;
\item particle transparency for minimum particle scattering.
\end{itemize}
This type of conductors was used in production of larger detectors, such as CELLO, CDF, TOPAZ, VENUS, ALEPH, DELPHI, CLEO, SDC, BELLE, ATLAS CS, ATLAS ECTs, ATLAS BT, CMS, PANDA and Mu2e solenoids.
Exactly the same conductor, as was used for the PANDA solenoid is supposed to use in SPD. 
The solenoid conductor consists of three components: 
\begin{itemize}
\item superconducting NbTi/Cu multi-filamentary strand with 1.4 mm diameter;
\item Rutherford-type flat cable with 8 strands;
\item high purity aluminum stabilizer of 10.95 mm $\times$ 7.93 mm cross-section, clad by a co-extrusion or plating process (or another qualified process).
\end{itemize}

\begin{table}[]
\centering
\caption{NbTi/Cu strand mechanical and electrical specifications.}
\label{tab:ma_1}
\begin{tabular}{|l|c|c|c|}
\hline
Parameter                           & Unit  & Value  & Tolerance  \\
\hline
Diameter filament                   & $\mu$m    & $<20$   & --           \\
Diameter strand                     & mm    & 1.400  & $\pm$ 0.005     \\
Cu/SC ratio                         & --     & 1.00   & $\pm$ 0.05      \\
Surface coating                     & --     & none   & --           \\
NbTi Jc (at 4.2 K, 4.05 T)          & A/mm$^2$ & $>$ 2800 & --          \\
Critical current (at 4.2 K, 4.05 T) & A     & $>$ 2600 & --          \\
n-value (at 4.2 K, 4.05  T)         & --     & $>$ 30   & --           \\
Conductor RRR                       & --     & $>$ 100  & --           \\
Twist direction                     & --     & left   & --           \\
Twist pitch                         & mm    & 25     & $\pm$ 5        \\
\hline
\end{tabular}
\end{table}

\begin{table}[]
\centering
\caption{Rutherford cable mechanical and electrical specifications.}
\label{tab:ma_2}
\begin{tabular}{|l|c|c|c|}
\hline
Parameter                                                                                                       & Unit     & Value   & Tolerance \\
\hline
Number of strands                                                                                               & --        & 8       & --         \\
Cable width                                                                                                     & mm       & 5.3     & $\pm$ 0.1     \\
Cable thickness                                                                                                 & mm       & 2.60    & $\pm$ 0.05    \\
Transposition angle                                                                                             & degree   & 20.0    & $\pm$ 0.5     \\
Twist direction                                                                                                 & --       & right   & --         \\
Critical current (at 4.2 K, 4.05T)                                                                              & A        & $>$ 20800 & --         \\
\begin{tabular}[c]{@{}l@{}}Critical current degradation of\\   extracted strand (at 4.2 K, 4.05 T)\end{tabular} & \%        & $<$ 5     & --         \\
RRR of extracted strands                                                                                        & --        & $>$ 100   & --         \\
Residual twist on 1 m of cable                                                                                  & degree/m & $<$ 45    & -- \\        
\hline
\end{tabular}
\end{table}

\begin{table}[]
\centering
\caption{Solenoid conductor mechanical and electrical specifications.}
\label{tab:ma_3}
\begin{tabular}{|l|c|c|c|}
\hline
Parameter                                                           & Unit & Value        & Tolerance \\
\hline
Width (after cold work) at 300 K                                    & mm   & 10.95        & $\pm$ 0.03    \\
Thickness (after cold work) at 300 K                                & mm   & 7.93         & $\pm$ 0.03    \\
Width (after cold work) at 4.5 K                                    & mm   & 10.90        & $\pm$ 0.03    \\
Thickness (after cold work) at 4.5 K                                & mm   & 7.90         & $\pm$ 0.03    \\
Minimum Al layer thickness in height                                & mm   & $>$ 1.9        & --         \\
Minimum Al layer thickness in width                                 & mm   & $>$ 2.1        & --         \\
Surface roughness                                                   & --    & Ra $<$ 3.2     & --         \\
Critical current (at 4.2 K, 4.05  T)                                & A    & $>$ 20800      & --         \\
Critical current (at 4.5 K, 3.6 T)                                  & A    & $>$ 23400      & --         \\
Critical current degradation of extracted strand w.r.t. virgin wire & \%    & $<$ 15         & --         \\
Overall Al/Cu/superconductor ratio                                              & --    & 10.5/1.0/1.0 & --         \\
Extracted strand RRR                                                & --    & $>$ 100        & --         \\
Aluminum RRR (at 4.2 K, 0 T)                                        & --    & $>$ 600        & --         \\
Al 0.2\% yield strength at 300 K                                     & MPa  & $>$ 30         & --         \\
Al 0.2\% yield strength at 4.2 K                                     & MPa  & $>$ 40         & --         \\
Shear strength Al to strands                                        & MPa  & $>$ 20         & --         \\
Unit length for upstream \& downstream coils                         & m    & 2 $\times$ 3203     & --         \\
Unit length for center coil                                         & m    & 1604         & --         \\
Total length of conductor                                           & m    & 8010         & --         \\
Minimum bending radius during production and on spools              & mm   & $>$1000       &  --\\    
\hline   
\end{tabular}
\end{table}

Pure aluminum features a very high electrical and thermal conductivity at low temperatures, providing the best possible stability in terms of maximum MPZ (Minimum Propagation Zone), making the coil least sensitive to mechanical disturbances that can cause coil training during commissioning and quenching during normal detector operation. Furthermore, aluminum stabilized superconductors can be made by co-extrusion of several kilometers long. Precise rectangular conductor shapes can be obtained, allowing for high accuracy in the coil winding. The cross-section of the conductor is shown in Fig. \ref{lb_mag_4}~(b).

Tables \ref{tab:ma_1}, \ref{tab:ma_2}, and \ref{tab:ma_3} present a summary of the main mechanical and electrical properties of the strands, Rutherford cable, and Al-stabilized conductor. 
%The full technical specifications for manufacture, inspection, and test can be found in reference \red{[?????]}.

The conductor has a temperature margin of about 2,4 K. The shape of the conductor allows to easily wind the coil from both the wide and the narrow sides.
%The conductor has been its temperature margin about 2.4 K. The shape of the conductor makes possibilities to do ease coil winding as with using the wide side of the conductor so the narrow side. 

\subsubsection{Insulation}
The main requirement for coil insulation is to provide the required electrical strength in terms of break-down voltage, while maximizing heat conduction, in order to reduce the peak temperature in the conductor in the 2-layer windings.
The conductor insulation used in PANDA is proposed for the SPD solenoid. The insulation scheme relies on the use of fiberglass 3$\div$5 mm thick in the first and the last layers, and  a nominal conductor insulation between layers.
The nominal cable insulation thickness is 0.200 mm per side. It is made of two half-overlapped layers of 100 $\mu$m thick fiberglass tape. The tape is wrapped around the surface of the conductor. BINP technology of a vacuum impregnation provides a reliable electrical strength and a good resistance to coil winding imperfections, especially when using  two layers of the conductor, in the SPD case.

Ground insulation is added at the outer surface and sides of the coil modules. No ground insulation is applied at the inner diameter, where detector vacuum already provides the necessary dielectric strength. At the outer diameter (3$\div$5 mm thick), the first layer is wound, which is then machined, after curing of the coil module to obtain precise fitting to the supporting cylinder-to-coil interface. The precise thickness of ground insulation after machining depends on the control of the radial dimensions of the coil during winding. A minimum thickness of 2.0 mm is recommended. 

The envisaged thickness of ground insulation at the coil sides is 2.80 mm for the upstream and downstream coils and 1.50 mm for the central coil. The thickness of the axial ground insulation can be adjusted to correct winding tolerances, since dielectric strength is always ensured by the mylar layer, located at the sliding interface. At the side flange, used as the base for coil winding, the axial ground insulation is provided in the form of epoxy shims, precisely machined, in order to accommodate winding tolerances. At the opposite side, axial ground insulation is provided by filling the empty spaces between the winding pack and the flange with epoxy resin after the flange assembly.

\begin{figure}[!h]
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{mag_5} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{mag_6} \\ (b)}
  \end{minipage} 
  \caption{(a) Thermosyphon circuit. (b) Connection of the cooling tubes and aluminum strip on the outer surface of the aluminum alloy support cylinder. 
	}
\label{lb_mag_4}
\end{figure}


\subsubsection{Thermosyphon cooling circuit}
The cold mass of the SPD solenoid is indirectly cooled by circulating two-phase helium by natural convection. Homogenous model, used for the preliminary study for CMS \cite{Bredy:2006iy} and then BINP, is also used for cooling of the PANDA detector solenoid and the  CBM detector dipole magnet.

The main advantages of a thermosyphon system are its simplicity and reliability, as it does not require any moving parts, such as cold pumps and high pressure for piping of the coils. On top of this, thermosyphon cooling ensures constant and uniform temperature, since the helium flow automatically adjusts to the heat load distribution.

The thermosyphon circuit consists of two manifolds, at the top and bottom of the cold mass, connected by two sets of six syphon tubes, as illustrated in Fig. \ref{lb_mag_4}~(a).  

The SPD coils feature six cooling tubes with two tubes for each.

The material selected for the thermosyphon circuit is Al-1100 due to its high thermal conductivity. The extruded tubes have a diameter of 10 mm and are welded to the support cylinder -- a technically proven solution to ensure reliable thermal contact, as shown in Fig. \ref{lb_mag_4}~(b).

The thermosyphon circuit is assembled as two halves consisting of six cooling tubes, welded to the top and bottom manifolds. The division in two halves is on purpose, as then each half-circuit can be fully tested for leaks, prior to installation on the cold mass, including the bimetallic (steel-aluminum) joints at the connectors, interfacing the manifolds and the cryogenic lines to the cold box.

%The extruded tubes have a process diameter of 10 mm and are welded by intermittent seam welding to the support cylinder (Fig. \ref{lb_mag_4}(b)). During welding should be taken attention for the support cylinder temperature. The temperature must be smaller than 350 $^\circ$C.

\subsubsection{Sliding interface}
Due to the presence of NbTi/Cu strands in the Al-stabilized conductor, the thermal contraction of the coil is less than that of the aluminum alloy, used for the support cylinder and flanges. On top of this, small gaps tend to develop at the coil winding-to-flange interfaces under the bending action of the Lorentz force.

In order to prevent the risk of stress accumulation at the coil winding-to-flange interfaces that could result in cracks in the insulation, triggering magnet quenches, the coil is allowed to slide with low friction and, if needed, separate from the flange. Therefore, sliding interfaces are created between coil windings and flanges by placing a 0.1 mm Mylar foil and 0.4 mm of Kapton\textregistered.

\subsubsection{Support cylinder}
In order to limit coil deformation and stress, due to the Lorentz force, support cylinders are placed around the coil windings. The cylinders are made of graded aluminum alloy Al-5083-O, exhibiting good mechanical strength at cryogenic temperature. Being the main structural elements of the cold mass, the shells must be produced as single pieces with uniform material properties.

The assembly formed by coil winding and support cylinder is referred to as a coil module. The assembly operation is performed via shrink fit with interference in order to ensure radial pre-stress. The required radial interference between coil windings and shells is 0.70 mm at room temperature. For this purpose, the support cylinders are produced with oversized dimensions to allow for machining of the inner surface. The thickness of the cylinders after machining shall not be less than 20~mm.

The coils are permanently bonded to the support cylinders by means of epoxy resin or grease (for example Apiezon N), suitable for cryogenic applications. The shells are connected together using bolts passing through the flanges, as described in the next section.

\subsubsection{Flanges, bolts, spacers, and venting holes}
The flanges are disks made of aluminum alloy Al-5083-O that cover the coil winding ends (outer flanges) or separate the coil modules (inner flanges). Similar to the requirements for the support cylinders, the flanges have to be produced as single pieces. Joining several flange pieces by welding is not allowed. 

The bolt calculations assume a safety factor of 1.5 and are based on the Eurocode 3, which is the standard adopted at CERN/DESY/FAIR. 
All bolted interfaces should be designed to hold the weight of the cold mass in tension during assembly and for all operating conditions. 
All bolted interfaces should be designed to be slip-critical under any condition. As such, the friction force under each bolt shall be higher than the shear force. Therefore, the bolts need to be sufficiently pre-loaded during the assembly. The recommended pre-load at room temperature amounts to 60\% of the tensile strength of the bolt. Since the thermal contraction of the material SS A4 is lower than that of Al-5083-O, the pre-load will reduce to 35\% of the bolt tensile strength after a cool-down. Compressive forces during the magnet operation will also reduce the  bolt pre-tension  to some extent. 

Bolt tightening shall be performed in steps with a torque wrench, and each bolt pre-load should be measured using an ultrasonic stress meter. Bolts shall be tightened uniformly, with an acceptable pre-load variation of $\pm$10\%. It is recommended to re-measure the bolt pre-load, and adjust if necessary, prior to the installation of the cold mass in the cryostat to correct possible relaxation, due to a local yielding and creep in the material.

Gaps of 8 mm are envisaged between the inner flanges that are to be shimmed with aluminum spacers. The gap allows for adjusting the axial position of the coil modules, in order to compensate winding and assembly tolerances and obtain the correct magnetic field profile (Fig. \ref{lb_mag_5}). The axial dimensions of the spacers are to be determined after the dimensions of the coil modules have been precisely measured. 

\begin{figure}[!ht]
    \center{\includegraphics[width=1.\linewidth]{mag_7}}
  \caption{ Connections "inner flanges -- support cylinder" (left) and "inner flange -- inner flange" (right).
	}
\label{lb_mag_5}
\end{figure}

In order to reduce the work associated with shimming and not interfere with the thermal bridges, spacers will be placed only at the locations of the bolts. Shimming of the entire surface of the flange is not required: based on the maximum axial force on the coil modules, the Al 5083-O yield strength (145 MPa) and, assuming a sufficient safety factor, the minimum shim area is 0.04 m$^2$. The value is much smaller than the surface of the inner flanges ($\sim$1 m$^2$).

When the thermal bridges are placed in correspondence with the position of the bolts, and hence of the spacers, attention shall be paid to limit the stress on the soft aluminum, so that the thermal conduction of the strip is not degraded.

To reduce the air evacuation time of the cryostat during pumping, it is recommended that all closed volumes should have a hole to vent to the cryostat vacuum (minimum diameter  of 1 mm). 

Venting holes are recommended at the location of the bolt connections, although at present they are not included in the technical drawings of the cold mass. When the threaded hole is filled with epoxy, venting holes allow for an exit of excess resin, which can be regarded as an indicator of good bond quality. 

\subsubsection{	Cold mass thermalization}

The cryogenic scheme of the SPD solenoid relies on indirect cooling of the cold mass by circulating saturated helium at 4.5 K by natural convection. A thermosyphon circuit consists of a bottom and top manifold connected by 12 parallel syphon tubes, attached to the outer surface of the support cylinder, as in Fig. \ref{lb_mag_9}.

The cooling method chosen for the SPD magnet's superconducting coil is based on the natural convection of liquid helium flow. It is a self-regulating thermosyphon circulation flow system. Natural circulation loop works on the principle that a heat load on the channels of the heat exchanger produces a two-phase flow that is, on average, less dense than the liquid phase. 
\begin{figure}[!h]
    \center{\includegraphics[width=0.65\linewidth]{coldmass1}}
  \caption{ Design of the cooling cold mass circuit: 1 -- upper manifold; 2 -- lower manifold; 3 -- syphon tubes; 4 -- Al-SS bi-metal adapters; 5 -- vessel with liquid helium.
	}
\label{lb_mag_9}
\end{figure}

\begin{figure}[!h]
    \center{\includegraphics[width=1.\linewidth]{coldmass2}}
  \caption{ Thermosyphon circuit of the SPD solenoid showing the two-halves assembly of the cold mass, as well as the height of the chimney and position of the control dewar.
	}
\label{lb_mag_10}
\end{figure}
The liquid from the helium vessel of the control dewar will be fed through the front pipeline and manifolds at the bottom of the support cylinder. Then, the liquid will be heated in the tubes of the heat exchanger (a rib cage configuration) on the surface of the support cylinder. The two-phase helium from the top manifold will return back through the reverse pipeline to the upper part of the helium vessel.

The design of the thermosyphon cooling circuit includes the definition of the optimal size for the syphon tubes and their position on the cold mass support cylinder. PED and AD2000 pressure vessel rules have to be applied for the construction of the cryogenic system.

In order to verify the feasibility of thermosyphon cooling, the expected mass flow rate and vapor fraction have been assessed with the homogenous model, described in Ref. \cite{Dhanaraj_2015}. In the model, the required  quantities are determined by balancing the driving hydrostatic pressure difference, which results in the thermally induced density gradient between the hot and cold sides of the loop, with the fluid acceleration and friction pressure drops in the supply and return tubes. 
The reported diameters correspond to the inner diameters of the pipes. It must be noted that the current technical drawings may contain out-of-date values for the dimensions of the pipes of the thermosyphon circuit.

The model thus confirms that the height of the control dewar installed on the upper platform of the SPD yoke with respect to the bottom of the magnet is sufficient to guarantee the driving hydrostatic pressure. The thermosyphon tubes and supply/return lines are also properly dimensioned to guarantee minimal pressure drop along the cooling circuit (Fig. \ref{lb_mag_10}).
The main advantages of a thermosyphon system are its reliability, since it does not include any moving part, and its ability to maintain a uniform temperature, as the helium flow automatically adjusts to the heat load distribution and variations.

\begin{figure}[!ht]
    \center{\includegraphics[width=1.\linewidth]{coldmass3}}
  \caption{ General view of the SPD cryostat with the control dewar.
	}
\label{lb_mag_11}
\end{figure}

\subsubsection{	Cryostat and control dewar}

All materials and components used in the construction of the cryostat and control dewar must be suitable for the use for which they are intended, in particular for the use at low temperatures. The choice of materials has to be in line with the directive 2014/68/EU PED and must be made according to the regulation prescribed by the AD/AD2000 Technical Rules for Pressure Vessels. 
\begin{figure}[!h]
    \center{\includegraphics[width=0.9\linewidth]{process_flow1}}
  \caption{ Process flow diagram of the SPD cryogenic system.
	}
\label{lb_mag_1222}
\end{figure}
%The general view of the SPD cryostat with the control Dewar is presented on Fig.15. 
The general view of the SPD cryostat with the control dewar is presented in Fig. \ref{lb_mag_11}.
The cryostat comprises of the cold mass with the superconducting coil, surrounded by a thermal screen and suspended on low heat conduction triangle supports. The cryostat should be mounted on the supports connected to the magnet yoke. The design of the cryostat supports will be defined later.

The control dewar is a functional unit of the cryogenic system and is intended to maintain the required parameters of liquid and gaseous helium (flow rate, pressure, temperature) and to provide cooling of the current leads. In the process flow diagram of the SPD cryogenic system, it is located between the cryostat and the helium liquefier. 

Physically, the control dewar is located on the top of the yoke. The vessel for liquid helium, current leads, piping, control and relief valves, and temperature sensors are placed in the horizontal vacuum tank of the control dewar. 

Cryogenic and current supplies will be connected from the control dewar to the cryostat through the service chimney in a special slit at the backward end of the yoke barrel. In the bottom part of the chimney an interface box is located, which is intended to accommodate connections of the cryogenic pipelines and current bus bars from the cryostat and the control dewar.

Based on the experience of creating a similar superconducting magnet, when assessing the cyclic strength of the cryostat, it was estimated that the solenoid parts should allow for 1000 cooldown cycles from room temperature to the operating temperature and back to room temperature, and 2500 energization cycles to the nominal current or any fraction of it. 

The cryogenic system of the cryostat and the control dewar will be designed to handle the loads resulting from all operation scenarios. Design pressure for all pipelines and helium vessel is 19 bar absolute (bar-a).

Liquid helium that is used for cooling the cold mass is fed from the liquefier at 4.5 K. Thermal shields of the solenoid surround the cold internal parts and are cooled by gaseous helium, which passes through the pipes of the heat exchanger of serpentine type. The helium flow leaves the liquefier at a temperature level of 40 or 50 K and returns to the liquefier after passing the thermal shields at a temperature level of about 80 K.
The process flow diagram of the SPD cryogenic system has the same principle as for CMS solenoid (CERN) and PANDA (FAIR), and is shown in Fig \ref{lb_mag_1222}.

The main components of the cryogenic system are: 
\begin{enumerate}
\item the cryostat, which includes:
\begin{itemize}
\item the superconducting coil cooled indirectly via the thermal contact with the aluminum support cylinder,
\item thermal shields cooled by gaseous helium,
\item a vacuum vessel;
\end{itemize}
\item the control dewar, which includes:
\begin{itemize}
\item a vessel for liquid helium,
\item current leads,
\item thermal shields cooled by gaseous helium,
\item valves, gauges and other instrumentation,
\item a horizontal vacuum tank with pumping system;
\end{itemize}
\item a transfer line (chimney) connecting the vacuum shell of cryostat and the control dewar;
\item the helium liquefier;
\item the transfer lines for helium supply connecting refrigerator and the control dewar.
\end{enumerate}

\subsubsection{	Thermal loads of cryostat and control dewar}
Estimated thermal loads of the control dewar, cold mass, and thermal shields of the SPD solenoid are summarized in Table \ref{tab:mag_5}. %The loads will be recalculated for the Final Design Review.
\begin{table}[]
\centering
\caption{Heat loads of the control dewar, transfer line, and cryostat. }
\label{tab:mag_5}
\begin{tabular}{|l|c|c|c|}
\hline
T=4.5K                               & \multicolumn{3}{l}{Heat loads, W}                           \\
\hline
                                     & Normal condition & Without magnetic field & Current ramping \\
\hline                                   
\multicolumn{4}{l}{Cryostat}                                                                       \\
\hline  
radiation                            & 7.8              & 7.8                    & 7.8             \\
supports                             & 5*               & 5*                     & 5*              \\
eddy current loss in cold mass       & -                & -                      & 11.50**         \\
eddy current loss in conductor       & -                & -                      & 0.09**          \\
current leads, 6.5kA B=1.25T         & 15               & 9                      & 9               \\
\hline  
\multicolumn{4}{l}{Control dewar}                                                                  \\
\hline  
radiation                            & 0.45             & 0.45                   & 0.45            \\
supports                             & 0.26             & 0.26                   & 0.26            \\
cold valves                          & 1.05             & 1.05                   & 1.05            \\
safety relief valves                 & 3,22             & 3,22                   & 3,22            \\
vacuum barrier                       & 0.35             & 0.35                   & 0.35            \\
\hline  
\multicolumn{4}{l}{Transfer line}                                                                  \\
\hline  
radiation                            & 0.06             & 0.06                   & 0.06            \\
supports                             & 0.20             & 0.20                   & 0.20            \\
\hline  
Total                                & 33,39            & 27,39                  & 44,98           \\
\hline
\hline
T=60K                                & \multicolumn{3}{l}{Heat loads, W}                           \\
\hline
                                     & Normal condition & Without magnetic field & Current ramping \\
\hline
\multicolumn{4}{l}{Cryostat}                                                                       \\
\hline  
radiation                            & 160              & 160                    & 160             \\
supports thermal shields             & 12.00            & 12.00                  & 12.00           \\
eddy current loss in thermal shields & -                & -                      & 47.00**         \\
\hline  
\multicolumn{4}{l}{Control dewar}                                                                  \\
\hline  
radiation                            & 10.66            & 10.66                  & 10.66           \\
supports thermal shields             & 6.30             & 6.30                   & 6.30            \\
supports helium vessel               & 16.50            & 16.50                  & 16.50           \\
cold valves                          & 22.50            & 22.50                  & 22.50           \\
safety relief valves                 & 1.07             & 1.07                   & 1.07            \\
vacuum barrier                       & 1.18             & 1.18                   & 1.18            \\
\hline  
\multicolumn{4}{l}{Transfer line}                                                                  \\
\hline  
radiation                            & 0.99             & 0.99                   & 0.99            \\
supports                             & 2.00             & 2.00                   & 2.00            \\
Total                                & 233,2            & 233,2                  & 280.2           \\
\hline
\multicolumn{4}{l}{*ATLAS data;  ** PANDA data}                                                   
\end{tabular}
\end{table}

\subsubsection{Cryostat vacuum vessel}
The cryostat vacuum vessel is designed as two concentric shells with thick annular end plates, all made of stainless steel, according to AD2000 W10; its basic parameters are given in Table \ref{tab:mag_5}. A cross-section of the cryostat is shown in Fig. \ref{lb_mag_11}.

\begin{table}[]
\centering
\caption{Vacuum vessel dimensions and operating conditions.}
\label{tab:mag_6}
\begin{tabular}{|l|c|}
\hline
Envelope             &                  Dimension                                                                             \\
\hline
\begin{tabular}[c]{@{}l@{}}Inner radius
     \\ Outer radius
      \\ Length 
      \\ Inner cylinder thickness \\ Outer cylinder thickness \\ End plates thickness\end{tabular} & \begin{tabular}[c]{@{}l@{}}1604 mm\\ 1834 mm\\ 3800 mm
      \\ 8 mm
      \\ 12 mm
      \\ 45 mm\end{tabular} \\
Operating conditions                                                                                                                                           &                                                                                               \\
Operating pressure inside/outside                                                                                                                              & 0/1 bar-a                                                                                    \\
Designed inside overpressure against 1 bar-a                                                                                                                   & 1.45 bar-a      \\
\hline                                                                              
\end{tabular}
\end{table}
The nominal wall thickness is 12 mm for the outer cryostat shell and 16 mm for the inner shell. The thickness of the flanges is 45 mm. The thickness of the shells allows to minimize the displacement of the cold mass under the action of the magnetic forces, relative to its nominal position. The flanges are attached to the vacuum vessel shells by 96+96 stainless steel bolts, according to the State Standard 11738-84 (DIN912) M10$\times$1.5 (L = 60 mm).

The installation of the ECal, weighing 44 tons, requires the cryostat to be optimized, taking into account additional loads. It may be possible to increase the thickness of the inner shell. The calorimeter is proposed to be installed on two horizontal rails, welded to the inner shell.

%So as planned to install the ECal with total mass 44 tons into the cryostat, the cryostat should be optimized to take into account additional loads. There is a possibility to increase the thickness of the inner shell. It is supposed to install the calorimeter on two horizontal rails welded to the inner shell.
%So as planned to install the ECal with total mass 44 tons into the cryostat the cryostat should be recalculated take attention additional loads. It may be possible to increase the inner shell thickness. It is supposed to install the calorimeter on two horizontal rails welded to the inner shell.

The cryostat supports (to be designed later) will provide a high rigidity of the construction for all structural loads, including the action of the magnetic forces, and will take into account the minimal dimensions between the outer shell of the cryostat and the yoke (see Fig. \ref{lb_mag_111}). The 18 supports will be installed, 9 pieces for each side. The maximal load (about 64 tons) should be on the bottom octant of the yoke. To distribute this load, four supports are installed on the top plate of the octant next to the edges, whereas the biggest part of the load goes on the side plate of the octant. The mechanical stress analysis shows that the maximum dimensional deformation is 1.6 mm for the top octant plate and the maximum stress is about 140 MPa (Fig. \ref{lb_mag_112}). Also, these supports make it possible to align the solenoid axis with the beam axis.

\begin{figure}[!ht]
    \center{\includegraphics[width=1.\linewidth]{mag20_1}}
  \caption{ Cross-section of the cryostat.
	}
\label{lb_mag_11}
\end{figure}
\begin{figure}[!ht]
    \center{\includegraphics[width=1.\linewidth]{cryo25}}
  \caption{ Location of the cryostat in the yoke and arrangement of the cryostat supports.
	}
\label{lb_mag_111}
\end{figure}
\begin{figure}[!ht]
    \center{\includegraphics[width=1.\linewidth]{cryo26}}
  \caption{ Calculation of mechanical and magnetic loads on the bottom octant.
	}
\label{lb_mag_112}
\end{figure}

The axial and radial gaps between the cryostat vacuum shell and the thermal shield, as well as between the shield and the cold mass in warm and cold state, are indicated in Fig. \ref{lb_mag_11}. They are not sufficient for the cryostat assembly and for avoiding of thermal contacts between the shells after cooling. A certain amount of space is needed for adjusting the optimal mutual positions of the holes for the triangle supports in the support flanges on the inner cryostat shell and in the brackets or holes for connecting the triangle supports to the cold mass. 
There are 12 triangle supports on each side. The wide side of a triangle support is attached to a part of the vacuum shell by a special flange with two M16 bolts. The apex of the triangle is attached to the cold mass. The shape of the support takes into account the mechanical and thermal loads, as a compromise.
To compensate for the radial changes in lengths of the cold mass and the vacuum shell  (more than 12 mm), spherical washers are installed in all attachment points. To minimize the change in the position of the cold mass, we assume the pre-setting of the cold mass to be at + 5$\div$6 mm from the plane of the support flange, and after cooling down to 4.5 K -- at -5$\div$6 mm from the plane of the support flange. To compensate for the longitudinal changes in length (more than 12 mm), a slot is proposed in the cold mass, at the point of attachment of the triangle apex. The design of a triangle support is shown in Fig. \ref{lb_mag_113} and the mechanical analysis in Fig. \ref{lb_mag_114}. The estimated loads on the triangular supports are given in Table \ref{tab:load_to_support}. 
\begin{figure}[!ht]
    \center{\includegraphics[width=1.\linewidth]{cryo27}}
  \caption{ Design of the triangle support of the SPD cold mass.
	}
\label{lb_mag_113}
\end{figure}
\begin{figure}[!ht]
    \center{\includegraphics[width=1.\linewidth]{cryo28}}
  \caption{Calculated mechanical loads on the triangle support.
	}
\label{lb_mag_114}
\end{figure}
\begin{figure}[!ht]
    \center{\includegraphics[width=1.\linewidth]{cryo29}}
  \caption{Triangle support test device.
	}
\label{lb_mag_115}
\end{figure}

\begin{table}[htp]
\caption{Loads on the triangilar support.}
\begin{center}
\begin{tabular}{|l|c|c|}
\hline
Load conditions & Load, kN & Maximum load to support, kN \\
\hline
Cold mass weight & 42 & 4.0 \\
Decentering force (5 mm) & 47.5 & 4.47 \\
\hline
Total load  & 89.5 & 8.47 \\
\hline
\end{tabular}
\end{center}
\label{tab:load_to_support}
\end{table}%

As a material for the supports, it is proposed to use STEF1 or some type of carbon fiber. Mechanical calculations were made for a support with a thickness of 20 mm and a load of 10 kN (Fig. \ref{lb_mag_114}). Calculations indicate an acceptable stress level of 96 MPa, with Limit stress of STEF1 -- 132 MPa and with a maximal deformation of 0.9 mm.
Testing of the triangle supports at room and cryogenic temperatures is planned. The proposed scheme of the tests is shown in Fig. \ref{lb_mag_115}.

The exact location of the cold mass inside the cryostat after its assembly should be defined with maximum precision. This is necessary to determine an optimal position of the superconducting coil inside the yoke aperture. After the cryostat assembly, any correction of the cold mass position inside the cryostat is impossible. A correction of the coil position, relative to the yoke aperture, can only be provided by means of fitting spacers in the cryostat support legs. This correction can be implemented in accordance with the results of field measurements in the tracker area and measurements of forces in the suspension rods.

In the normal operative condition mode, the inner cryostat volume is evacuated, which leads to general membrane compressive stresses in the outer cryostat shell, due to the action of the outer atmospheric pressure. In the process of magnet operation, an emergency situation may happen, when an overpressure up to 0.05 MPa appears in the inner volume. This leads to general membrane compressive stresses in the inner cryostat shell.

The buckling analysis of the cryostat shells is based on an FE model. The considered load cases are the following:
\begin{itemize}
\item	 cryostat weight;
\item	 weight load of the cold mass and thermal screen octants, applied to the outer cryostat shell;
\item	weight loads of the thermal screen octants and of the inner detectors, applied to the inner cryostat shell;
\item	 outer overpressure of 0.1 MPa (first variant);
\item	 inner overpressure of 0.05 MPa (second variant).
\end{itemize}
According to computations, the stability of the cryostat shell under the action of an outer overpressure of 0.1 MPa is ensured with a safety margin of 8.5. The stability of the cryostat shell from the action of an inner overpressure of 0.05 MPa is ensured with a safety margin of 17 (Fig. \ref{lb_mag_12}).

\begin{figure}[!h]
    \center{\includegraphics[width=1.\linewidth]{mag_21}}
  \caption{ Calculations of the cryostat stresses and deviations. The load of the calorimeter is not included.
	}
\label{lb_mag_12}
\end{figure}

\subsubsection{Control dewar}
\paragraph{Vacuum vessel}
The outer vacuum housing of the control dewar encloses the stainless steel vessel for liquid helium, control valves, current leads, and process piping, surrounded by a thermal shield, located between the outer housing and the interior of the control dewar (Fig. \ref{lb_mag_13}). The vacuum vessel of the control dewar has a horizontal barrel shape and is made of stainless steel.

The thickness of the outer walls of the vessel is 8 mm and the weight of the assembled control dewar is about 1600 kg. The main dimensions of the control dewar are shown in Fig. \ref{lb_mag_13}. The diameter of the vacuum shell is 1500 mm, the height with valves is about 2500 mm, the width of the control dewar is 2780 mm and with the vacuum pump system -- 3425 mm. The flanges of the control dewar lids are tightened by 2$\times$48 studs M12.

The vapor-cooled current leads of the solenoid and the cryogenic relief valves are mounted on the top plate of the control dewar housing. 

Vacuum vessels, shells of transfer lines and the cryostat must handle the loads from all possible operating scenarios. Design pressure of all vacuum vessels is 0.45 bar(g).


\begin{figure}[!h]
    \center{\includegraphics[width=1.\linewidth]{dewar1}}
  \caption{ Layout of the control dewar. 
	}
\label{lb_mag_13}
\end{figure}

\paragraph{Valves of the control dewar}
Chosen types of the control dewar valves are listed in Table \ref{tab:mag_6}. The regimes of the flow through the heat exchangers of the cold mass and the thermal shield will be defined in detail later. The positions of valves of the control dewar for various magnet operation regimes are established in accordance with Table \ref{tab:mag_7}, where the positions of controlled valves are indicated for each regime.

\begin{table}[]
\centering
\caption{Control dewar valves.}
\label{tab:mag_6}
\begin{tabular}{|l|c|c|c|l|}
%\multicolumn{1}{c}{\textbf{Part}} & \multicolumn{1}{c}{\textbf{Nominal diameter, mm}} & \multicolumn{1}{c}{\textbf{Rated pressure, bar}} & \multicolumn{1}{c}{\textbf{Rated temperature, ë}} & \multicolumn{1}{c}{\textbf{Valve type}}                               \\
\hline
Part                                & Nominal       & Rated  & Rated & Valve type \\
                                       &diameter,  mm & pressure,  bar & temperature, K & \\
\hline
CV1 & 10                                                & 25                                               & 4.5$\div$300                                           & pneumatically-actuated control valve \\
        &   &   &   & with digital positioner (0...100\%)\\
CV2& 10                                                & 25                                               & 4.5$\div$300                                           & pneumatically-actuated control valve  \\
        &   &   &   & with digital positioner (0...100\%)\\
CV3& 25                                                & 25                                               & 4.5$\div$300                                           & pneumatically-actuated control valve  \\
        &   &   &   & with digital positioner (0...100\%)\\
CV4& 10                                                & 25                                               & 4.5$\div$300                                           & pneumatically-actuated control valve  \\
        &   &   &   & with digital positioner (0...100\%)\\
CV5& 10                                                & 25                                               & 4.5$\div$300                                           & pneumatically-actuated control valve \\
        &   &   &   & with digital positioner (0...100\%)\\
CV6& 8                                                 & 25                                               & 80$\div$300                                            & pneumatically-actuated control valve \\
        &   &   &   & with digital positioner (0...100\%)\\
CV7& 8                                                 & 25                                               & 80$\div$300                                            & pneumatically-actuated control valve  \\
        &   &   &   & with digital positioner (0...100\%)\\
CV8& 8                                                 & 25                                               & 40$\div$300                                            & pneumatically-actuated control valve  \\
        &   &   &   & with digital positioner (0...100\%)\\
CV9& 8                                                 & 25                                               & 40$\div$300                                            & pneumatically-actuated control valve  \\
        &   &   &   & with digital positioner (0...100\%)\\
SV1& 15                                                & 25                                               & 80$\div$300                                            & pneumatically-actuated shut-off valve                   \\
        &   &   &   &(open/closed)  \\
SV2& 20                                                & 25                                               & 80$\div$300                                            & pneumatically-actuated shut-off valve                \\
        &   &   &   &  (open/closed)    \\
RV1& 20                                                & 20                                               & 4.5$\div$300                                           & safety relief valve                                                   \\
RV2& 20                                                & 20                                               & 4.5$\div$300                                           & safety relief valve     \\                                             
\hline                                             
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Positions of the control dewar valves for various SPD magnet operation regimes. C: valve closed, O: valve open, R: valve regulated.}
\label{tab:mag_7}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
{\tiny Valve} & {\tiny  Initial } & {\tiny Cool down}  & { \tiny Steady-state} & {\tiny  Warm-up} & {\tiny  Cooling of }  & {\tiny  Emergency} & {\tiny  Cooling} & {\tiny Emergency} & {\tiny Emergency} & {\tiny Emergency}  & {\tiny Emergency}  \\
          &{\tiny  setting }& \tiny {from} &  &  &  { \tiny the thermal} & {\tiny (coil}  & {\tiny  after coil } & {\tiny (refrigerator}  & {\tiny (power}  & {\tiny (current lead} & {\tiny (loss of} \\
          &           & \tiny {300 to 4.5 K} &  &  & {\tiny shields} & {\tiny quenching)} & {\tiny quenching} &{\tiny failure)} & {\tiny failure)} &  {\tiny voltage rise above} &{\tiny vacuum)}\\
          &            &     & & & & & & & &{\tiny allowable level)} & \\
\hline
CV1                    & C               & R                                                               & C            & R       & C                              & C                          & R                            & C                                                                          & C                                                                   & R                                                                                                          & C                                                                    \\
CV2                    &   C            &     R                                                         &R            & C       & C                              & C                          &R                            & C                                                                          & C                                                                   & C                                                                                                          & C                                                                    \\
CV3                    & C               & C                                                              & O            & C       & C                              & C                          & C                            & O                                                                          & O                                                                   & C                                                                                                          & C                                                                    \\
CV4                    & C               & O                                                               & O            & R       & C                              & C                          & O                            & C                                                                          & C                                                                   & R                                                                                                          & C                                                                    \\
CV5                    & C               & C                                                               & C            & R       & C                              & O                          & R                            & R                                                                          & R                                                                   & R                                                                                                          & O                                                                    \\
CV6                    & C               & R                                                               & R            & R       & C                              & C                          & R                            & R                                                                          & R                                                                   & R                                                                                                          & C                                                                    \\
CV7                    & C               & R                                                               & R            & R       & C                              & C                          & R                            & R                                                                          & R                                                                   & R                                                                                                          & C                                                                    \\
CV8                    & C               & R                                                               & R            & R       & R                              & R                          & R                            & C                                                                          & C                                                                   & R                                                                                                          & C                                                                    \\
CV9                    & C               & O                                                               & O            & O       & O                              & O                          & O                            & C                                                                          & C                                                                   & O                                                                                                          & C                                                                    \\
SV1                    &C              &C                                                              & C            & O       & C                              & C                          & C                            & C                                                                          & C                                                                   & O                                                                                                          & C                                                                    \\
SV2                    &C             &O                                                           & O            & C       & C                              & O                          & O                            & O                                                                          & O                                                                   & C                                                                                                          & O            \\                                                       
\hline
\end{tabular}
\end{table}

\paragraph{Vessel for liquid helium }

A stainless steel vessel for liquid helium, required to maintain the operating conditions of the solenoid, is placed inside the control dewar. The hydraulic volume of the helium bath of the vessel is chosen to provide stable operation of the magnet with heat inflows to the control dewar and the superconducting coil during the period necessary for safe de-energizing the superconducting coil, when the liquefier is stopped. The heat flow into the vessel and to the superconducting coil, including heat losses in current leads, amounts to 50 W, which corresponds to a liquid helium flow rate of 71 l/h. Since it takes more than 60 minutes for safe de-energization of the coil, the volume of the helium vessel is chosen to be 300 liters, to have a sufficient safety margin. The outer surface of the vessel is covered by a multilayer screen-vacuum insulation to reduce heat inflows.

The volume and the outer surface area of the vessel for liquid helium is 300 l and 2.5 m$^2$, respectively. It is possible to increase 
the volume of the helium vessel,
because the space on the upper yoke platform allows a placement of the control dewar with bigger dimensions.
The helium vessel suspensions are made by combining a pipe and a rod (Fig. \ref{lb_mag_15}). The heat load on the suspension (0.09 W)  is calculated with the following parameters: the temperature of the shell -- 300 K, of the helium vessel -- 4.5 K, and of the thermal shields -- 60 K. The components of the suspension are:
\begin{itemize}
\item a stainless steel rod 217 mm long with a diameter of 40 mm;
\item a stainless steel  pipes with a diameter of 21.3, thickness of 2, and length of  588 mm;
\item a rod 200 mm long, stainless steel M12.
\end{itemize}
\begin{figure}[!h]
    \center{\includegraphics[width=1.\linewidth]{mag23_1}}
  \caption{ Arrangement of the helium vessel into the control dewar and a scetch of the suspension of the helium vessel.
	}
\label{lb_mag_15}
\end{figure}

Stability of the helium vessel, when it is exposed to external pressure of $-1$ bar(g) (vacuum inside the vessel), is provided with a sufficient safety margin. The conditions of static and cyclic strength and the stability condition will be fulfilled in this case as well. 

An electrical heater is installed in the helium bath to maintain the required level of liquid helium and to control the rate of the return helium flow to the helium liquefier (maintenance of thermal balance). The heater power of about 400 W corresponds to the maximum cooling capacity of the liquefier. This heater is also used for rapid evaporation of liquid helium from the bath. The power capacity of the heater may vary from zero to the maximum value, determined by the cooling power of the liquefier at a temperature level of 4.5 K. Two identical liquid helium level-meters (one active, one spare) will be installed in the helium vessel. 

It is also suggested to install a differential pressure sensor. The first point of pressure measurement is the upper part of the helium vessel with gas medium; the second capillary should be installed at the bottom of the helium vessel.  The value of the $\Delta P$ provides a measurement of the liquid helium level in the vessel. The control of the liquid helium level  in the vessel will be included in the control system of the magnet. 

\subsubsection{	Chimney and interface}
The vacuum pipe (chimney) connects the vacuum volumes of the cryostat and the control dewar. The outer diameter of the chimney is 219.1 mm, the wall thickness is 2 mm. It encloses the superconducting bus-bars, direct and return pipes for gaseous and liquid helium flows, measurement wiring, all of which are surrounded by a thermal shield (Fig. \ref{lb_mag_16}).  Its bottom part is supplied by a weld ring flange DN 250 ISO-K with rotatable bolt ring DN 250 ISO-K (both made of stainless steel 304/1.4301). This flange is tightened to the flange on top of the interface box by 12 bolts M10. The rotatable bolt ring facilitates the connection procedure of the flanges at the stage of the cryostat and control dewar assembly.

 
A decoupling spring bellow (made of stainless steel 1.4541), supplied with two flanges DN 250 ISO-K (made of stainless steel 304/ 1.4301), is placed at the top of the chimney, in order to compensate for mutual shifts of the control dewar and the cryostat during assembly, reloading of the magnet from stationary supports to roller skates and back, and during magnet movement along the rail track. The upper flange of the decoupling spring bellow is connected to the flange at the bottom of the control dewar. 
The main parts of the chimney are shown in Figure \ref{lb_mag_17}.

\begin{figure}[!t]
    \center{\includegraphics[width=1.\linewidth]{chim1}}
  \caption{ Section of the chimney with the control dewar.
	}
\label{lb_mag_16}
\end{figure}
\begin{figure}[!b]
    \center{\includegraphics[width=1.\linewidth]{chim2}}
  \caption{ The main dimension of the chimney. 1 -- bellows; 2 -- G10 spacer; 3 -- thermal shield; 4 -- bus-bar.
	}
\label{lb_mag_17}
\end{figure}
\begin{figure}[!h]
    \center{\includegraphics[width=1.\linewidth]{chim3}}
  \caption{ Views of the chimney's thermal shield with thermal bridges and a cross-section of the chimney.
	}
\label{lb_mag_18}
\end{figure}

The current leads and process piping surrounded by a thermal shield are located between the outer shell and cold part with temperature 4.5 $\div$ 50 K. The 80-K return pipe should be fixed to the chimney thermal shield and have the copper thermal bridges installed every 350$\div$400 mm. To fix the location of the thermal shield in the vacuum shell, a few ball supports are installed (see Fig. \ref{lb_mag_18}). Also, these supports allow the movement of the thermal shield, relateive to the vacuum shell, after cooling and shrinkage of the thermal shield. The material of the thermal shield is stainless steel 304/ 1.4301. One edge of the copper thermal bridges is brazed to the stainless steel 80-K return pipe, and another edge is connected to the thermal shield by screw rivets. Apiezon N grease provides a reliable heat contact of the connection.

The positions of the 4.5-K forward and return pipes, the 50-K forward pipe, and bus-bars into the chimney are fixed by two G10 spacers. The spacers will be equipped with two or three G10 wheels, to compensate for the changing dimensions of this assembly, relative to the thermal shield during all operating conditions. The 50-K return pipe has a rigid fixation to the spacers, while other pipes and bus-bars have a slippery fixation. To avoid any risk of heating the bus-bars and high risk of quenching or even overheating of the superconductor, the bus-bars are connected to an assembly with a 4.5-K return pipe (Fig. \ref{lb_mag_19}).
\begin{figure}[!h]
    \center{\includegraphics[width=0.8\linewidth]{mag_27}}
  \caption{ Cross-section of a bus-bar assembly.
	}
\label{lb_mag_19}
\end{figure}
\paragraph{Interface box}
The interface box is located in the bottom part of the chimney and is fixed on the flange of the cryostat. The box accommodates connections of the pipelines, as well as joints of the superconducting bus-bars of the cryostat and the control dewar. The flanges with connectors for sensors are located on the side cover of the interface box.
Testing of the solenoid welds of superconducting cables in the interface box will be performed using extensions of the bus-bars (Fig. \ref{lb_mag_20}). The joints will be made by edge welding of Al to Al stabilizer, up to three times. These extensions can be cut to allow dismounting of the solenoid a few times.

\begin{figure}[!h]
    \center{\includegraphics[width=0.8\linewidth]{mag28_1}}
  \caption{ Connecting bus-bars and process pipes into the Interface box. 
	}
\label{lb_mag_20}
\end{figure}
\begin{figure}[!h]
    \center{\includegraphics[width=1.\linewidth]{mag29_1}}
  \caption{ Cryostat thermal shield.  
	}
\label{lb_mag_21}
\end{figure}

\paragraph{Thermal shields}
Thermal shields of the solenoid surround the cold internal parts and are cooled by gaseous helium, which flows through the pipes of the heat exchangers. The design of the cooling circuit of the screen provides its cooling independently from the cold mass cooling. The helium flow leaves the liquefier at temperature of 50 K and passes the heat exchangers of the thermal shields of the cryostat, chimney and control dewar successively. After that it returns to the liquefier at temperature of 80 K. Heat gains to the thermal shields of the cryostat, chimney and control dewar, as well as the temperature of the cooling gas at inlet and outlet of the heat exchangers of each circuit element in the steady-state regime, are indicated in the flow scheme. The total length of the cooling tube of the heat exchangers is about 76.3 m (cryostat, control dewar, and chimney).

\subsubsection{Thermal shield of the cryostat }
The cryostat thermal shield surrounds the cold mass with the coil. It consists of two cylindrical sectors and two flanges. The heat exchanger of the cryostat thermal screen consists of Al alloy pipes with a diameter of 12 and thickness of 2 mm fixed on the outer and inner shells of the quadrants and connected by intermittent welding. The cooling pipes were optimized for 50 K helium gas, but it is possible also to use liquid nitrogen.

The shield envelope is split up into electrically separated parts (quadrants) (Fig. \ref{lb_mag_21}), to avoid damage and deformations of the screen, when the coil undergoes an emergency discharge. The quadrant shells are separated by gaps of about 14 mm, covered by sheets of insulating material G10. In addition, there are radial flange cuts of 10 mm. As can be seen from these pictures, there are four different types of quadrant configuration (depending on the shape of the heat exchanger tube and on the positions of the attachments for the temperature interceptions of the cold mass suspension). 

The inner and outer shells of the octants are supported by the stiffening ribs (angled profile 30 $\times$ 20 mm) and interconnected by the flanges at the ends. Shells, flanges and stiffening ribs of the octants are made of aluminum alloy AL 5083 (AMg5). The thickness of the sheets of the shells and flanges is 4 mm. The mass of the outer shell of a quadrant is about 60 kg, the mass of the inner shell is about 52 kg. These masses are convenient for assembling. The total area of the screen surface of the cryostat is 78 m$^2$. The total mass of the cryostat screen is 880 kg.

The shield is positioned into the cryostat with the help of the  ball support units with a G10 ring. On the outer and inner surface of the shield  30 layers of superinsulation will be placed. The total heat inflow through the shield supports is about 15 W. 
Appropriately oriented slots, made in the octant shells, are intended to reduce the lateral loads applied to the studs, caused by thermal shrinkage of the shield material.

\subsection{Electrical systems}
\subsubsection{	Electrical connections of the coils}
The SPD solenoid relies on the following electrical joints:
\begin{itemize}
\item two layer-to-layer joints in the upstream and downstream coil modules;
\item two coil-to-coil joints connecting the center coil module to the upstream and downstream coil modules;
\item two terminal joints connecting the solenoid to the bus-bars.
\end{itemize}

The routing of the coil-to-coil joints and terminal joints on the cold mass is displayed in Fig. \ref{lb_mag_24}. The joints are aligned with the magnetic field lines to avoid forces. The joints are clamped and glued to the cold mass, resulting in good thermal contact with the cold surface of the support cylinder. No thermalization of the joints to the cooling circuit is envisaged in this reference design, due to the expected low heat generation. A support bracket, shown in Fig. \ref{lb_mag_25}~(a), holds the weight of the bus-bars at the upstream end of the cold mass. The bracket is designed to sustain a total weight of 800 N, while the expected weight of the bus-bars is about 300 N.

Although the current routing of the bus-bars and joints is such as not to interfere with the other components installed on the cold mass, it is advisable to further optimize the layout of the upstream end of the cold mass. The present design of the area is crowded, due to the necessity to route both the electrical and cooling lines through the cryogenic chimney.

In Fig. \ref{lb_mag_25}~(a) it is possible to distinguish the grooves in the inner flanges, allowing routing of the conductor from the coil to the outer surface of the cold mass. The cross-section of the coil conductors is 8$\times$11 mm$^2$.
% and connection between downstream, central and upstream coils. 

The area is crowded due to the presence of the radial rod supports and cooling line manifold, connecting the thermosyphon circuit to the cold box.

The design of the joints between the SPD solenoid conductors is essentially the same as applied in the ATLAS magnets. The configuration of the layer-to-layer and coil-to-coil joints is shown in Fig. \ref{lb_mag_25}~(b) left.  Terminal joints are instead illustrated in Fig. \ref{lb_mag_25}~(b) right. The use of the left-over conductor, developed for the ATLAS end-cap toroids, is intended in this reference design for the bus-bars of the SPD solenoid.

All conductor joints inside the cryostat are made without removing the aluminum stabilizer. The joints are made by TIG welding of the adjoining cables. Al-1050 is recommended as the filler material, as used for the conductor in the ATLAS toroids. The use of different aluminum alloys is also possible, depending on the expertise of the firm, building the SPD solenoid. After welding and cleaning, the conductor insulation is applied around the layer-to-layer joints. Ground insulation, instead, has to be wrapped around the coil-to-coil and terminal joints.

\begin{figure}[!h]
    \center{\includegraphics[width=0.8\linewidth]{mag_33}}
  \caption{ Position of coil-to-coil and terminal joints on the PANDA solenoid cold mass as an example.
	}
\label{lb_mag_24}
\end{figure}

\begin{figure}[!h]
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{mag_34} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{mag_35} \\ (b)}
  \end{minipage} 
  \caption{(a) Upstream end of the cold mass showing the bus-bars and their support bracket. (b) Layer-to-layer and coil-to-coil (left) and terminal (right) joint layouts. }
\label{lb_mag_25}
\end{figure}

The electrical resistance of the joint shall not exceed 1.0 n$\Ohm$ at 4.2 K and 3 T. The joint length resulting in the envisaged resistance is determined experimentally by welding and testing the conductor samples. In this reference design a minimum joint length of 700 mm is assumed for all joints (note that some joints in the drawings of this document may have erroneously a shorter length). Cooling and interruption of welding must be applied to the joints during welding, in order to limit the duration of the superconducting cables inside the conductors at temperatures above 600 K, to avoid critical current degradation. The critical current degradation in the superconducting cables due to the joint welding shall not exceed 5\%.

\subsubsection{Power converter}
The magnet is powered by a DC power supply, providing an operational current 4.4 (5.2) kA. 
It is possible to increase the value of the current by  installing additional power converters, when the planned field at the solenoid axis is 1.5 T.
 The bus-bars connecting to the power supply are equipped with the circuit breakers. The bus-bars resistance is negligible, compared to the circuit resistance during slow and fast dumps.
The slow discharge of the magnet is achieved by opening the circuit breakers, to disconnect the magnet from the power supply. The current is discharged via the slow dump unit, composed of several diodes in series. A series of four diodes is assumed, featuring a total resistance of 3 m$\Ohm$, which results in a discharge time of 2000 s.
Block scheme of the electrical racks is shown in Figure \ref{lb_mag_26}~(a).

The power convertor assembly design is shown In Fig. \ref{lb_mag_26}~(b). It is proposed to use the TDK-Lambda type current source. One current source has a value of the current up to 1000 A. Seven or eight current sources are connected in parallel. 

\subsubsection{Quench protection}
The quench protection system is designed to limit the peak temperature on the coil windings to 80 K and the peak voltage to ground to 500 V during any normally protected quench. The system relies on the monitoring of the resistive voltages, associated with the normal zone spread, and the quench development via the voltage taps, installed on the coil modules, as well as on the joints and bus-bars. A schematic view of the magnet electrical circuit is shown in Fig. \ref{lb_mag_27}~(a).
\begin{figure}[!h]
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{mag_36} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{mag_37} \\ (b)}
  \end{minipage} 
  \caption{(a) Cabling diagram of the power supply scheme. (b) General design of five paralleled current sources controlled by ACU.}
\label{lb_mag_26}
\end{figure}
\begin{figure}[!h]
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{mag_38} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{mag_39} \\ (b)}
  \end{minipage} 
  \caption{(a) Electrical quench protection scheme of the PANDA solenoid. (b) Main parameters of the electromechanical breaker.
}
\label{lb_mag_27}
\end{figure}

The quench protection system (QPS) continuously monitors the magnet voltage during operation. In case a resistive voltage exceeding the threshold of 0.5 V is detected, the QPS waits for 1 s to eliminate false signals and gives the magnet a chance to recover, if the perturbation energy was below the minimum quench energy. If a quench recovery does not occur, the QPS activates the circuit breakers (Fig. \ref{lb_mag_27}~(b)) to disconnect the power supply from the magnet, and the current is discharged in the fast dump resistor. The value of the resistor is set to 62.5 m$\Ohm$, to limit the voltage to ground. The grounding circuit is designed to symmetrically divide the voltage across the magnet terminals. Quench protection, in the case of a fast dump, is helped by the quench-back effect of the support cylinder, which improves quench propagation, thereby reducing the temperature increase of the coils.

To assess the quench performance of the SPD solenoid, quenches have been initiated at different locations in each of the three sub-coils (i.e. across the two layers, as well as at the edges and the center of the winding packs). The quench is initiated by rising the temperature of the selected turn above the critical value.

During a fast dump, independently from the location of origin of the quench, the current in the coils decays with a time constant of 9.5 s. The maximum voltage drop is 360 V, well below the maximum design limit of 500 V (Fig. \ref{lb_mag_28}). The hot spot temperature is limited to a very safe value of 60 K.
\begin{figure}[!h]
    \center{\includegraphics[width=0.8\linewidth]{mag_40}}
  \caption{ Electromechanical breaker and help of snubber against the arc.
	}
\label{lb_mag_28}
\end{figure}

The total stored energy E is:
\begin{equation}
E=\frac{1}{2\mu_0} B_0^2\times V = 19.3 ~MJ.
\end{equation}

With the present layout of the quench protection system, 58\% of the initial magnetic field energy is dissipated in the dump resistor, 26\% as eddy current loss in the coils and casing, and the remaining 16\% in the diode unit.

The results of the quench analysis show that proper operation of the QPS limits the peak coil temperature and voltage well below the threshold values. The maximum temperature reached by the coils is here re-assessed in the case of failure of the QPS, which results in the entire stored energy being dissipated in the winding. Under the assumption that the quench-back effect of the support cylinder causes a rapid propagation of the normal zone to the entire coil without extracting energy from the system, the magnet would heat up to 80 K. Even in the unrealistic case that the energy is entirely dumped in only one of the sub-coils, the temperature would reach 112 K and 161 K for the upstream/downstream and center coils, respectively. Although unwanted from the cooling point of view, these temperature values do not pose risks for the integrity of the solenoid.

\subsection{Vacuum system of the SPD magnet}
The control dewar, chimney, and cryostat with superconducting coil have a common vacuum volume. A pumping station with rotary and turbo-molecular pumps performs the vacuum pumping. The pressure to be obtained by vacuum pumping before cooling and cryostatic temperature regulation is 10$^{-5}$ mbar. Further pumping will be performed in the process of cooling by cryogenic panels, mounted on the outer surface of the support cylinder. The vacuum system is shown in Fig. \ref{lb_mag_29}~(a). The pumping station is placed on the upper platform of the magnet. Two pressure sensors are fitted on the vacuum casing of the control dewar to check the pressure. 
\begin{figure}[!h]
  \begin{minipage}[ht]{0.45\linewidth}
    \center{\includegraphics[width=1\linewidth]{mag_41} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.55\linewidth}
    \center{\includegraphics[width=1\linewidth]{mag_42} \\ (b)}
  \end{minipage} 
  \caption{(a) Vacuum equipment. (b) Distribution of the pressure inside of the vacuum system.
}
\label{lb_mag_29}
\end{figure}
For pumping of the vacuum volumes of the control dewar, chimney, and superconducting coil cryostat up to $10^{-1}$ mbar with a safety factor of 2, a rotary pump could be employed with a pumping speed of 15$\div$18 l/s. For pumping down to 10$^{-5}$ mbar, a turbo pump with a pumping speed of 500$\div$680 l/s can be chosen. Distribution of the pressure inside the vacuum system is presented in Figure \ref{lb_mag_29}~(b). Calculation was done by software ''MOLFLOW+ 2.6.62''.  

The cryostat and control dewar of the SPD solenoid will be built according to AD2000. The worst-case scenario concerning the safety of the cryostat would arise, if a leak evolved in the part of the liquid helium (LHe) cooling circuit that runs through the vacuum vessel. Only in this case the pressures balance could actually be reversed, and the pressure inside the cryostat could exceed the atmospheric pressure.

The cryostat vacuum vessel, control dewar, and all connections have to be verified to resist up to a pressure of 1.50 bar (absolute pressure) from the inside. This provides a good safety margin, as the coolant circuit will be working at an absolute pressure of 1.30 bar, and we foresee safety flange DN250. For the outer cryostat shell, the stability against a pressure reverse is easily guaranteed, since it is designed to work with 1.0 bar from the outside. This is naturally different for the inner wall of the cryostat, which is designed to keep, under normal operation, the atmospheric pressure from inside. However, the inner wall of the cryostat is designed to keep safely the full load of the detector, mainly the weight of the ECal with minimum deformation. The extra thickness needed to fulfill this requirement is more than enough to guarantee  against buckling of the inner wall of the cryostat in case of a pressure reversal, due to a leak in the helium circuit. 

A system of safety valves has been foreseen to prevent an excessive pressure rise in the vacuum vessel of the cryostat, control dewar, and chimney. A relief flange opening at 0.3 bar is foreseen. In case of LHe vaporization, the relief valve would open, venting the helium gas to the atmosphere and preventing damages to the cryostat vessel. 
\begin{table}[]
\centering
\caption{Sensor instrumentation summary for the cold mass of the SPD solenoid.}
\label{tab:mag_8}
\begin{tabular}{|l|c|c|c|c|}
\hline
\multicolumn{1}{c}{\textbf{Function}} & \multicolumn{1}{c}{\textbf{Location}} & \multicolumn{1}{c}{\textbf{Quantity}} & \multicolumn{1}{c}{\textbf{Sensor type}} & \multicolumn{1}{c}{\textbf{Notes}} \\
\hline
\multirow{6}{*}{Quench detection}     & Coil  modules                         & 6                                     &                                          & 3 Primary/Redundant pairs          \\
                                      & Coil-to-coil joints                   & 4                                     &                                          & 2 Primary/Redundant pairs          \\
                                      & Terminal joints                       & 4                                     & Voltage                                  & 2 Primary/Redundant pairs          \\
                                      & Bus-bar joints                        & 4                                     & taps                                     & 2 Primary/Redundant pairs          \\
                                      & Vertical bus-bars                     & 4                                     &                                          & 2 Primary/Redundant pairs          \\
                                      & Current leads                         & 4                                     &                                          & 2 Primary/Redundant pairs          \\
\hline                                      
\multirow{3}{*}{Cryogenic monitoring} & Coil modules                          & 6                                     & Cryogenic                                & 1 Top/Bottom                       \\
                                      & Bus-bars                              & 4                                     & temperature                              & 2 Primary/Redundant sensors        \\
                                      & Cryogenic lines                       & 2                                     & sensor                                   & 1 Supply/Return line   \\
\hline                                                 
\end{tabular}
\end{table}
\begin{table}[]
\centering
\caption{List of purchasing equipment for control dewar cryogenic system.}
\label{tab:mag_9}
\begin{tabular}{|c|l|l|}
\hline
\multicolumn{1}{c}{No.} & \multicolumn{1}{c}{Type device/ instrument} & \multicolumn{1}{c}{Producer}                                                       \\
\hline
1                       & Cold Valves                                 & \begin{tabular}[c]{@{}l@{}}Velan\\ Weka\\ Stoehr\\ Flowserve\end{tabular}          \\
2                       & Relief valves                               & Leser                                                                              \\
3                       & Warm valves                                 & \begin{tabular}[c]{@{}l@{}}Velan\\ Weka\\ Stoehr\\ Flowserve\end{tabular}          \\
4                       & Pressure transmitters                       & Emerson/ Siemens/ WIKA                                                             \\
5                       & Pressure indicators                         & Swegelok                                                                           \\
6                       & T platinum sensors                          & Heraeus                                                                            \\
7                       & Low-temperature thermometers                       & \begin{tabular}[c]{@{}l@{}}Business Logistix Ltd\\ OXFORD/ JINR/ BINP\end{tabular} \\
8                       & Warm flow meters                            & BROOKS Smart series/ BRONKHORST                                                    \\
9                       & Heaters                                     & many companies                                                                     \\
10                      & Level meters                                & AMI                                                                                \\
11                      & Connectors, 2 bars                          & Fischer                                                                            \\
12                      & Connectors, 2 bars for heaters              & Fischer                                                                            \\
13                      & Connectors, 40 bars                         & Serie\_Hermetique\_Jager                                                             \\
14                      & Pumps, preliminary and TMP                  & Edwards/ Laybold or equal                                                          \\
15                      & Gate valve DN150                            & VAT                                                                                \\
16                      & Vacuum angle valves                         & many companies                                                                     \\
17                      & Fittings                                    & Swegelok                                                                           \\
18                      & MLI                                         & Groupe HUTCHINSON ex- JEHIER/ RUAG                                                 \\
19                      & Ball supports                               & Bosch Rexroth            \\                                                         
\hline
\end{tabular}
\end{table}

\subsection{Cryogenics safety}
The different parts composing the cryostat should be designed, fabricated, and inspected according to the intent of the 
%AD2000 norm,
actual norms including corresponding documentation, certificates, and used standards. 

The choice of indirect cooling of the solenoid will greatly reduce the amount of liquid helium in the cryogenic system. The pipes, guaranteeing the coil refrigeration, will contain $\sim$10 l of refrigerant. This includes the two manifolds placed on the top and on the bottom of the cold mass for the thermosyphon circulation. Another  $\sim$300 l of liquid helium will be stored in the helium vessel, housed in the control dewar.

The operating pressure of the SPD coil cryogenic system will be 130 kPa (absolute pressure), corresponding to a coolant temperature of 4.5 K during cooldown and warmup. The two phases of liquid helium, used by the cooling system, will be fed to the helium vessel of the control dewar through a transfer line from the helium liquefier during normal operation. Liquid helium from this vessel will give the coil cryogenic system the capability to operate for up to 60 min. for safe de-energization of the coil.

The transfer line will decouple the refrigerator from the solenoid cryogenics, in case of refrigerator failure. In the worst case, the gas would be transferred into the helium vessel at the full pressure of the running compressor of the liquefier ($\sim$16 bar). In this case, it would be vented to the air through the relief valve and safety flange DN250. Furthermore, it will help that the liquefier and the control dewar will be connected through a long transfer line. This line will hydraulically decouple them in the scenario of a liquefier failure with the 16 bar helium gas, at the temperature of the last heat exchanger, transferred into the system.

As an additional safety measure, all the cooling loops and distribution lines inside the cryostat (including the intermediate radiation shields) are designed for a nominal operating pressure of 16 bar. The helium vessel of the control dewar, operating at 1.3 bar, is designed for an overpressure of 19 bar and will be equipped with a relief valve, venting the vessel into the atmosphere for the pressure p = 1.8 bar in case of helium boiling off, due to a quench or vacuum failure.

\subsection{Cold mass instrumentation}
The instrumentation of the cold mass of the SPD solenoid, taken as an example, falls under two groups: quench protection and cryogenic monitoring. Table \ref{tab:mag_8} provides a summary of the sensors to be installed.

The quench protection system monitors the coil modules and superconducting bus-bars for resistance growth, and provides a trigger for the current breaker to isolate the power converter from the solenoid, in order to limit the rise of conductor temperature, due to Joule heating. The quench detection system relies on voltage taps. Voltage taps are critical sensors and, therefore, must have redundancy. The voltage taps, installed on the joints, also provide the capability to monitor the joint resistance. Similarly, voltage taps are installed on the current leads to monitor the lead resistance.

Cryogenic monitoring is based on temperature sensors to control cooldown, warmup, steady state operation, and changes in response to a heat load, such as a quench. Temperature sensors are installed on the cold mass and bus-bars, as well as on the supply and return cryogenic lines.


Appropriate instruments and tools are required to control cryogenic processes. There are cryogenic cold and warm control valves with transmitters and actuators, flowmeters, pressure transmitters and manometers, thermosensors, level meters and related accessories. The minimal list of needed instruments and tools is presented in Table \ref{tab:mag_9}.

\begin{comment}
\subsection{Cost estimate}
An estimate of the cost of the magnetic system is presented in the Table \ref{Mag_cost}. To the 6780 kEuro or 7700 k\$ indicated there, we must add the cost of the system of detailed measurement and control of the magnetic field of 500 k\$.

\begin{table}[htp]
\caption{Cost estimate}
\begin{center}
\begin{tabular}{|c|c|c|}
\hline
Milestone & Description                 &           Cost, kEuro                \\
\hline
1 & Project management and testing  &  1870 \\
	& Technical project                      &    800 \\
	& 	Plan review                         &    170 \\
	& 	Preliminary design review  &    250 \\
	& 	SAT full solenoid                &     650 \\
\hline
2	& Conductor                                                    & 1650 \\
	& 	Contract conductor with ext. firm           &    360 \\
	& 	FDR conductor                                        &   160 \\
	& 	Start of conductor production at ext. firm&   870 \\ 
	& 	FAT conductor                                         &   260 \\
\hline
3	& 	Cryostat and cold mass      &  1060 \\
	& 	Cryostat design                   &   140 \\
	& 	FDR cryostat                      &   140 \\
	& 	Procurement  components  &   250 \\
	& 	FAT cryostat                        &   420 \\
	& 	SAT cryostat                       &    110 \\
\hline	
4	& 	Control dewar and prox. cryogenics  & 740 \\
	& 	Control dewar design                         & 100 \\
	& 	Control dewar vacuum equipment     &  150 \\
	& 	FDR control dewar                            &  170 \\
	& 	FAT control dewar                             &  220 \\
	& 	SAT control dewar                             &  100 \\
\hline
5	& 	Electrical components               &  760 \\
	& 	Contract el. components           &  120 \\
	& 	FDR el. components                  &  180 \\
	& 	Procurement of el. components&  340 \\
	& 	FAT el. components                   &  120 \\
\hline	
6	& 	Magnet alarm safety system	              &  120 \\
	& 	FDR safety system                                 &   40 \\
	& 	Tender of components for safety system&   60 \\
	& 	FAT safety system                                  &   20 \\
\hline	
7	& 	Coil winding                                    &  580 \\
	& 	Design coil winding                        &    40 \\
	& 	Tooling design                                &    30 \\
	& 	FDR coil                                         &    60 \\
	& 	Procurement of coil components   &   180 \\
	& 	FAT coil winding                             &   220 \\
	& 	Cold mass integration                    &    50 \\
\hline
	& 	Total  (with installation and commissioning) &  6780 \\
\hline

\end{tabular}
\end{center}
\label{Mag_cost}
\end{table}%

\end{comment}

%\input{TDR_magnet_JINR.tex}

\section{Cost estimate}
An estimate of the cost of each of the two magnetic system options is presented in the Table \ref{Mag_cost}. To the indicated  values, we must add the cost of the system of detailed measurement and control of the magnetic field of 500 k\$. 

\begin{table}[htp]
\caption{Cost estimate (kEuro).}
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
Milestone & Description                 &   Novosibirsk option & JINR option   \\
\hline
1 & Project management and testing  &  \bf{1870} & \bf{1220} \\
	& Technical project                      &    800 &  500\\
	& 	Plan review                         &    170  &  120\\
	& 	Preliminary design review  &    250   & 200\\
	& 	SAT full solenoid                &     650   & 400\\
\hline
2	& Conductor                                                    &  \bf{1650} &  \bf{850}  \\
	& 	Contract conductor with ext. firm           &    360         & \\
	&      Production conductor material and Cu inserts at ext. firm &   & 400 \\
	&      Production conductor at LHEP               &            &  200 \\
	& 	FDR conductor                                        &   160   & 100\\
	& 	Start of conductor production at ext. firm&   870   & \\ 
	& 	FAT conductor                                         &   260  &  150\\
\hline
3	& 	Cryostat and cold mass      &  \bf{1060} & \bf{640} \\
	& 	Cryostat design                   &   140 &   100\\
	& 	FDR cryostat                      &   140 &   70\\
	& 	Procurement  components  &   250 & 150\\
	& 	FAT cryostat                        &   420 &  250\\
	& 	SAT cryostat                       &    110 &   70\\
\hline	
4	& 	Cryogenics                            & \bf{740} &  \bf{1840}\\
	& 	Control dewar design                         & 100 &\\
	& 	Control dewar vacuum equipment     &  150 &\\
	&      Feed box design    && 100 \\
	&     Helium refrigerator  && 1100 \\
	&     Vacuum equipment  &&  150 \\
	& 	FDR                           &  170 &  170\\
	& 	FAT                             &  220 &  220\\
	& 	SAT                           &  100 &    100\\
\hline
5	& 	Electrical components               &  \bf{760} & \bf{760} \\
	& 	Contract el. components           &  120 & 120\\
	& 	FDR el. components                  &  180 &180\\
	& 	Procurement of el. components&  340 & 340\\
	& 	FAT el. components                   &  120 & 120\\
\hline	
6	& 	Magnet alarm safety system	              &   \bf{120} &  \bf{120} \\
	& 	FDR safety system                                 &   40 &  40\\
	& 	Tender of components for safety system&   60 &  60\\
	& 	FAT safety system                                  &   20 &  20\\
\hline	
7	& 	Coil winding                                    &   \bf{580} &  \bf{490} \\
	& 	Design coil winding                        &    40 & 40\\
	& 	Tooling design                                &    30 & 30\\
	& 	FDR coil                                         &    60 & 60\\
	& 	Procurement of coil components   &   180 & 150\\
	& 	FAT coil winding                             &   220 & 160\\
	& 	Cold mass integration                    &    50 &  50\\
\hline
	& 	Total  (with installation and commissioning) &   \bf{6780} & \bf{5920}\\
\hline

\end{tabular}
\end{center}
\label{Mag_cost}
\end{table}%


\section{Cryogenic system}
The magnetic field is formed by a superconducting (SC) coil. The NbTi superconductor, which has an operating temperature of 4.5 to 9.0 K, has been selected for the SC coil of the detector SPD. Keeping the SC coil in the SC state implies the use of a non-standard cryogenic system operating at 4.5 K. The working substance being gas/liquid helium.
For the SPD magnetic system project, two fundamentally different variants of structures and technical solutions of SC coils are being developed.  One concept is based on the application of a tubular SC cable of the Nuclotron type; this variant is proposed by the JINR LHEP working group (the first variant). To cool the proposed SC coil, supercritical helium is required, which requires the use of a refrigerator-type cryogenic plant.  The second concept implies the use of a Rutherford SC cable and for this SC coil a thermosiphon cooling method is used, which means the use of a liquefier type of cryogenic plant, this variant was proposed by the INP working group (second variant).
The cryogenic helium plant with the input cryostat will be placed on a technical platform, which is moved together with the SPD detector.  The   cryogenic system consists of three main subsystems: helium and nitrogen systems, as well as auxiliary systems. The helium system includes the cryogenic plant, high- and low-pressure helium flow pipelines, and cryogenic flexible pipeline for liquid and vapor helium.  Nitrogen system:  two cryogenic tanks for liquid nitrogen storage, cryogenic pipeline, pipeline for nitrogen vapor. Auxiliary systems: vacuum, measuring, cryogenic monitoring and control system, order gas system and water-cooling system. 
The cryogenic systems for both variants of SC coils will differ in the type of cryogenic plant and the design of the input cryostat.

\subsection{Helium cryogenic system  \label{sec:Cryogenic_He_system}}
\subsubsection{Cryogenic plant for the JINR variant of the SPD magnet}
The concept of the first version of the SC coil requires the use of a cryogenic helium plant of refrigeration type. It has the ability to work with supercritical helium flow and allows slow cooling of the SC coil by helium vapor, at a rate of about 4 K/h, as well as step-by-step cooling of the heat shields. The main operating parameters of the cryogenic plant are given in Table \ref{tab:cryo_1}.

\begin{table}[]
\centering
\caption{Main operating parameters of the cryogenic plant for the JINR option of the magnet.}
\label{tab:cryo_1}
\begin{tabular}{|c|l|c|}
\hline
p. & Operating parameters                            & Unit                                                                \\
\hline
1  & Cooling capacity                                & 100 W \@ 4.5K                                                        \\
2  & Temperature of outlet flow from the SPD         & 4.8 K (2.5 bar)                                                     \\
3  & Temperature of inlet flow from the SPD          & 4.8 K (3.0 bar)                                                     \\
4  & Hydraulic resistance of the SC coil             & 0.5 bar                                                             \\
5  & Cold weight                                     & 7865 kg                                                             \\
6  & Maximum pressure in coil                        & 5 MPa                                                               \\
7  & Mass flow rate                                  & $\leq$16 g/s                                                            \\
8  & Equipment Requirement                           & Maximum reliability,  \\
    & & energy efficiency, \\
    &  & compactness, automatic mode \\
9  & Interval of repair/regulatory work of the plant & Not more than once a year      \\
\hline                                    
\end{tabular}
\end{table}

The plant must have an additional outlet of liquid nitrogen from the nitrogen vessel to provide cooling of the SC coil heat shields, as well as meet all modern solutions in the cryogenic technology. 

The plant includes flexible lines to connect to the input cryostat for transportation of liquid and gaseous helium and nitrogen flows. Maximum heat load for flexible lines: for helium communications is 3 W/m; for nitrogen communications is 5 W/m.  All cryogenic flexible lines and pipelines are vacuum insulated, condensate formation on external surfaces of communications is not allowed. 

The power consumption of the cryogenic plant is 2 kW.

\subsubsection{Cryogenic plant for the Novosibirsk option of the SPD magnet}

The concept of the second variant of the SC coil requires the use of a cryogenic helium liquefaction plant, which allows to cool the SC coil and heat shields with helium vapor, the maximum cooling rate is 1 K/h. This variant uses the thermosiphon method of SC coil cooling. A similar cooling principle and SC coil design is used in such projects of MPD, PANDA, etc. detectors.

\begin{table}[]
\centering
\caption{Main operating parameters of the cryogenic plant for the Novosibirsk option of the magnet.}
\label{tab:cryo_2}
\begin{tabular}{|c|l|c|}
\hline 
p. & Operating parameters                            & Unit                                                                \\
\hline 
1  & Cooling capacity                                & 140 l/h                                                             \\
2  & Temperature of outlet flow from the SPD         & 4.3 K (1.05 bar)                                                    \\
3  & Temperature of inlet flow from the SPD &          4.5 K (1.15 bar)                                     \\
4  & Hydraulic resistance of the SC coil             & 0.1 bar                                                             \\
5  & Cold weight                                     & 3800 kg                                                             \\
6  & Maximum pressure in coil                        & 5 MPa                                                               \\
7  & Maximum heat load                               & 45 W                                                                \\
 8  & Equipment Requirement                           & Maximum reliability,  \\
    & & energy efficiency, \\
    &  & compactness, automatic mode \\
9  & Interval of repair/regulatory work of the plant & Not more than once a year      \\         
\hline                    
\end{tabular}
\end{table}

The plant must have an additional outlet of 50 K helium flow with a smooth adjustable temperature from 297 K to 50 K, to cool the heat shield of the detector SC coil. 
The plant includes flexible lines to connect to the input cryostat for transportation of liquid and gaseous helium flows. The maximum heat load for flexible lines of helium communications is 3 W/m. All cryogenic flexible lines and pipelines are vacuum insulated, condensate formation on external surfaces of communications is not allowed. 
The power consumption of the cryogenic plant is 2 kW.

\subsubsection{Helium pipelines}

The cryogenic system requires pipeline installation along the route from the central cryogenic station to the location of the SPD detector. Figure \ref{lb_cryo_1} shows the routing of the high- and low-pressure helium flows. The total length of the traces is about 220 meters. Pipelines of high-pressure helium flow have a 60 mm diameter and low-pressure helium flow has a 100 mm diameter. The material of the pipelines is stainless steel 12X18H10T or analog. Tracing has the following route. From the room 177 the route goes piping with other communications in one route to room 109/1 (about 120 meters of traces). From the room 109/1 the route goes to the courtyard of building 17 and on the ramp comes to the room 140/2.

The pipelines section from the entrance to room 140/2 to the cryogenic plant is made of flexible lines. Figure \ref{lb_cryo_1} shows the location of the cryogenic equipment on the technical platform and the flexible line. The pipelines have a system of safety devices, to provide safe operation.

\begin{figure}[!ht]
    \center{\includegraphics[width=1.\linewidth]{cryo_1}}
  \caption{ Tracing pipelines of high- and low-pressure helium flows.
	}
\label{lb_cryo_1}
\end{figure}

\begin{figure}[!h]
  \begin{minipage}[ht]{1.\linewidth}
    \center{\includegraphics[width=1\linewidth]{cryo_2} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{1.\linewidth}
    \center{\includegraphics[width=1\linewidth]{cryo_3} \\ (b)}
  \end{minipage} 
  \caption{Flexible lines in the room 140/2 when  SPD is in the ''beam'' (a) and ''servise'' (b) position.
	}
\label{lb_cryo_2}
\end{figure}

\subsection{	Nitrogen system \label{sec:Cryogenic_N2_system}}
To provide operation of the cryogenic helium plant it is necessary to create a nitrogen system. The nitrogen system includes the following main elements: two cryogenic storage tanks for liquid nitrogen, cryogenic pipeline and flexible line. 
The system uses two cryogenic tanks each with a capacity of 20 m$^3$, the main technical parameters are presented in Table \ref{tab:cryo_3}.

The cryogenic storage tanks are located on a special foundation to the Building 17 on the side of the room 140/1. 
Liquid nitrogen is supplied through a cryogenic pipeline by raising the pressure to 4.0 bar in the cryogenic storage tank. When the minimum liquid nitrogen level in the first cryogenic storage tank is reached, the control system automatically switches the liquid nitrogen supply from the first cryogenic storage tank to the second cryogenic storage tank.  The cryogenic pipeline is vacuum insulated and condensate formation on external surfaces of communications is not allowed. Total length of the route is about 120 meters. The pipeline is made on a tube-in-tube type, the inner pipeline is 30 mm in diameter, the outer pipeline is 70 mm in diameter. The material of the pipeline is stainless steel 12X18H10T or analog. The route has the following (Figure \ref{lb_cryo_3} shows a preliminary route): from the tanks the pipeline rises to a height of 6 meters for the passage over the road, then along the wall of the building 17, room 140/1, enter the room and bring it to the cryogenic plant. The route has a system of safety devices, to ensure safe operation. 

The discharge of gaseous nitrogen is carried out according to the principle of the shortest route with exit to the atmosphere. The discharge pipelines?s diameter is 70 mm.  Energy consumption of the system is 2 kW.
\begin{table}[]
\centering
\caption{Main technical parameters of the cryogenic storage tank.}
\label{tab:cryo_3}
\begin{tabular}{|c|l|c|}
\hline
p. & Operating parameters                                                                       & Value                        \\
\hline
1  & Overall volume                                                                             & 20 000 l                    \\
2  & Maximum daily evaporation rate depending & 0.17 \%                      \\
    & on pressure 100 kPa and ambient temperature15 $^{\circ}$ C       & \\
3  & Maximum outlet flow rate (nitrogen)                                                        & 600 Nm$^3$ / h                 \\
4  & Maximum operating pressure                                                                 & 1.8 MPa                     \\
5  & Operating pressure range                                                                   & From 1.2 bar to 4.0 bar     \\
6  & Minimum permissible wall temperature (inner vessel)  & 77 K \\
7  & Maximum pressure in vacuum space at T=293 K & 10 Pa \\
8  & Interval of repair / regulatory work of the plant & Not more than once a 7 years. \\
\hline
\end{tabular}
\end{table}%


\begin{figure}[!ht]
    \center{\includegraphics[width=1.\linewidth]{cryo_4}}
  \caption{ Tracing cryogenic pipelines of nitrogen flow.
	}
\label{lb_cryo_3}
\end{figure}

\subsection{Auxiliary systems}

Vacuum subsystem provides maintenance of discharged medium in isolation volumes of the cryogenic plant, input cryostat and SC coil cryostat. Maximum pressure value in the isolation volumes at 293 K (before start of cooling) is $1\times10^0$ Pa, maximum pressure value at 4.5 K (after cooling) for the cryogenic plant is $1\times10^{-3}$ Pa, for inlet cryostat and SC coil cryostat is $1\times10^{-5}$ Pa.

The subsystem includes several types of vacuum pumps: rotary vane pumps, Roots pumps, diffusion vapor pumps and turbomolecular pumps. The subsystem equipment is located on the technological platform of the detector SPD. The total power consumption of the subsystem is 14 kW.

Pneumatic valves and valves are used to control technological processes of the cryogenic system, their stable operation is ensured by the ordering of gas. The ordered gas subsystem has the following characteristics: working pressure 6 bar, working gas -- dry air. The system includes: air screw compressor, receiver, moisture separator and various fittings (valves and reducers). Power consumption of the subsystem is 3 kW.

The cryogenic system is controlled by means of data acquisition from all related subsystems (cryogenic unit, helium pipelines, nitrogen system, pneumatic system, vacuum system and data from SC coil control system). Figure \ref{lb_cryo_4} presents a block diagram of cryogenic control system. The control system has automatic circuits with which the following steps are carried out: preparation, cooling of the SC coil, cryostatting at workloads, and heating.
\begin{figure}[!ht]
    \center{\includegraphics[width=0.8\linewidth]{cryo_5}}
  \caption{ Tracing cryogenic pipelines of nitrogen flow.
	}
\label{lb_cryo_4}
\end{figure}

\subsection{Cost estimate}
The cost of the equipment described above and the required capacity are presented in Tab. \ref{tab:cryo_4}.

\begin{table}[]
\centering
\caption{Costs and required equipment capacity}
\label{tab:cryo_4}
\begin{tabular}{|c|l|c|c|}
\hline
p.  & Name of system                           & Cost, k\$ & Power consumption, kW \\
\hline
1.1 & Cryogenic plant (JINR option)  & 3 000     & 2         \\
1.2 & Cryogenic plant (Novosibirsk option) & 3 330     & 2         \\
2   & Helium pipeline                          & 500       & -         \\
3   & Nitrogen system                          & 1 500     & 2         \\
4   & Vacuum subsystem                         & 500       & 14        \\
5   & Pneumatic subsystem                      & 50        & 3         \\
6   & Cryogenic system control                 & 500       & 2         \\
\hline
    & Total (JINR option)                  & 6 050     & 23        \\
\hline
    & Total (Novosibirsk option)                 & 6 380     & 23      \\ 
\hline
\end{tabular}
\end{table}







==> tex/TDR_Straw.tex <==
\chapter{Straw Tracker}
 The purpose of the Straw Tracker (ST)  is to reconstruct  tracks of  primary and secondary particles with high efficiency, 
  to measure their momenta with high precision, based on a track curvature in a magnetic field, and to contribute to a particle identification via energy deposition ($dE/dx$) measurements. 
 A spatial resolution of ST is required to be about 150\,\textmu{}m. It has to be achieved when operating in a magnetic field of \mbox{about 1\,T}.
 
  The detector is planned to be built of low-mass straw tubes, similar to those used in many modern experiments, such as NA62 \cite{Sergi:2012twa}, COMET \cite{Nishiguchi:2017gei}, SHiP \cite{Anelli:2015pba}, Mu2e \cite{Lee:2016sdb}, COMPASS \cite{Bychkov:2002xw,Platzer:2005jp}, NA64 \cite{Volkov:2019qhb}, and others. 
  
 The tracker will consist of the barrel part and two end-caps. Two different kinds of straw tubes are considered to be used for them.

\section{Barrel part}
\subsection{Welded straw tubes}
\subsubsection{Material}


The detector is assembled from about 26\,000 straw tubes. 
A single straw tube is manufactured from a thin polyethylene terephthalate (PET) foil, 
which is welded longitudinally by ultrasonic welding to form a tube. 
The straw has an active length from 10~cm to 2.7~m and a nominal inner diameter of 9.8~mm.
Its inner surface has a metal coating (Cu/Au) to provide electrical conductance on the cathode, 
while the electrons, produced in ionization processes, will drift towards the central wire anode.

The choice of the straw material is a compromise between many different requirements, i.e.~radiation length, permeation of gases, mechanical properties, adhesion to metal coating, bonding with epoxy and the ability to be ultrasonically welded into a tube. A summary of the specifications is given in Table \ref{st_bar_t1}.
\begin{table}[htp]
\caption{Summary of coated material specifications.}
\begin{center}
\begin{tabular}{|c|c|}
\hline
Description  & Specifications \\
\hline
PET film  &  polyethylene terephthalate \\
                & type Hostaphan RNK 2600 of \\
                &(36 $\pm$ 2) $\mu$m thickness\\
Density    &  1.4 g/cm$^3$ \\
Copper layer thickness &   50 nm \\
Gold layer thickness     &   20 nm \\
Resistivity of straw tube (2.1 m) & $\sim$70 $\Ohm$ \\
Permeation of naked film,   & 6 for He, 0.06 for Ar, 1 for CO$_2$ \\
($10^{-12}$ Torr$\times$l$\times$cm/s$\times$cm$^2$$\times$Torr) & \\
\hline
\end{tabular}
\end{center}
\label{st_bar_t1}
\end{table}%


The straw tubes for the tracking detector in the SPD experiment are manufactured from a biaxially oriented coextruded film made of PET. 
One side of the film is chemically pre-treated to improve adhesion.
This side was chosen for the epoxy bonding between the straw tube and the polyetherimide (PEI)  straw fixation plug. 
The nontreated side is coated by a conductive layer of 50 nm of Copper (Cu) followed by a protective layer of 20 nm of gold (Au). 
Once the production of the tube is completed, the conductive layer is on the inside of the tube, while the outside remains uncoated and pre-treated chemically for bonding.
The thickness of the film is 36 $\mu$m.

\subsubsection{Long-term tests}
Long-term tests were carried out with the straws mounted under tension with a load of 15 N applied before the extremities of the tubes are bonded to the PEI supporting parts. The sag and the tension of the tubes were measured during a long-term test lasting 18 months. 
The values are recorded with  the straws under pressure and compared to a reference straw at the atmospheric pressure.
The results are shown in Fig.\,\ref{st_ba_fig1}.

\begin{figure}[!ht]
  \begin{minipage}[ht]{0.45\linewidth}
    \center{\includegraphics[width=1\linewidth]{st_ba_1} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{st_ba_2} \\ (b)}
  \end{minipage} 
  \caption{(a) View of the long-term test setup. 
  (b) Straw tension as a function of time (blue curve) plotted together with humidity (red curve).
}
\label{st_ba_fig1}
\end{figure}


\subsubsection{Tensile test of PET samples}

The base material for the straw tubes was tested in CERN using the Instron tensile test apparatus. 
A close-up view of the apparatus with a tested film sample is shown in Fig.~\ref{st_ba_fig2}~(a).
The values observed for welded samples are typically 25\% lower than those of the coated unwelded PET. 
Unwelded PET has a tensile strength close to 130~MPa, whereas welded and coated samples fail at $\sim$100~MPa. 
The stress in the straws due to the pressure difference of 1\,bar is 13\,MPa, which gives sufficient safety margin.


\begin{figure}[!h]
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{st_ba_3} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{st_ba_4} \\ (b)}
  \end{minipage} 
  \caption{(a) Close-up view of the tensile test apparatus with a tested film sample (the weld is in the center). (b) Typical view of a coated PET with a magnification of 20\,000 (RNK 2600).
	}
\label{st_ba_fig2}
\end{figure}

\begin{figure}[!ht]
    \center{\includegraphics[width=0.9\linewidth]{st_ba_5}}
  \caption{ Cross-section of a welded seam where the two sides of the strip are fused.
	}
\label{st_ba_fig3}
\end{figure}


\subsubsection{Coating and permeation}

The metal coating is accomplished by a sputtering process.
The metallisation provides electrical conductivity, as well as an improvement in the permeation properties of the PET substrate. 
Measured values of the permeation through a 50 nm Cu coated membrane show a barrier improvement factor of 8.5 for He (helium), 9 for CO$_2$  and 5 for Ar (argon). The quality of the sputtered coating is measured by a peel test using adhesive tape.


\subsubsection{Studies using a scanning electron microscope}

The coated PET was examined using the Scanning Electron Microscope (SEM) in order to determine the quality of the coating and sputtering on the substrate. The SEM was also used to verify the metal coating thickness, not as a direct measurement, but by using the energy-dispersive X-ray spectroscopy facility and a third party software.
The metal coating and weld quality of the seam were checked using both the SEM and the traditional optical microscopy, as shown in Fig.~\ref{st_ba_fig2}\,(b) and Fig.~\ref{st_ba_fig3}.


\subsubsection{Glue bonding test}

The adhesion between the outer side of the straw tube and the PEI straw support is critical. 
The chosen epoxy resin for this operation was TRA-BOND 2115,  fabricated by Tra-Con Inc.,~whose outgassing properties and radiation hardness were studied at CERN. This epoxy has a good resistance to stress and temperature cycles. Its pot life is close to two hours and curing in 24 hours. Samples of PET were peel tested after being bonded to an aluminium plate. The bond of the selected candidate was better than the natural resistance of the material. The selected material was also analysed by the X-ray photoelectron spectroscopy. This allowed us to better understand the chemical treatment made by the PET suppliers and its effects on bonding.


\subsubsection{ Straw manufacturing and welding}

A dedicated machine for the straw production has been designed and constructed to manufacture   
8000 straws for the NA62 experiment (diameter 10~mm, thickness 36~$\mu$m), 
2000 straws for the COMET experiment (diameter 10~mm, thickness 20~$\mu$m), and
100 straws for the SHiP experiment (diameter 20~mm, thickness 36~$\mu$m). 
Straw sets are currently being produced for prototypes intended for the NA62 upgrade and 
the straw tracker for DUNE (diameter 5~mm, thickness 20~$\mu$m). 
An ultrasound head with a movable fixation at the frame and an anvil for the straw welding are shown in Fig.~\ref{st_ba_fig6}.
They were designed and 
constructed to obtain a good quality of the welding seam (see Fig.~\ref{st_ba_fig5}) and 
to minimize differences in the straw diameter down to $\sim$10~$\mu$m. 
The distribution of the straw seam widths and tube diameters, obtained during the production of a large set of straws, are shown in  Fig.~\ref{st_ba_fig7}. 
After manufacturing, each straw is equipped with the glued end-plugs and tested for leaks. 
All measurements are individually recorded in a logbook where all straw characteristics are stored, i.e.~material, manufacturing date, inner diameter, etc. 
A unique serial number is allocated to every straw tube.
%a complete feedback is readable 
Using this number one can access the straw information 
at any moment of the detector assembly.

A few straws with a diameter of 10 mm were used for the dedicated mechanical tests. They were cut in 20 segments of about 25~cm long and tested under overpressure until the breaking point. The other straws were cut to 5.3~m and the cut ends were preserved for further analysis. The breaking pressure was found to be 9~bar on average; and not one sample broke under 8.5~bar. The quality control procedure was the same as for NA62 straws. During the ultrasonic welding process,  the seam quality was verified by a digital microscope and recorded to file for each straw. Furthermore, the seam quality was checked by an operator in real time. 


Several measurements and tests are performed post-fabrication. The seam width and straw inner diameter are measured by an optical method. The cathode electrical DC resistance is measured. The elongation and breaking force are measured on the test samples (cut straw ends). The straws undergo a long-term overpressure test with temporary end-plugs glued into both ends of each straw. An overpressure test to $\Delta P\approx  2$ bar is performed for a period of about 1~hour. Subsequently, the straw is subjected to a long-term overpressure test at  $\Delta P\approx  2$ for a period of at least 30~days. A gas leak estimation is obtained by measuring the loss of pressure over time. The local straw deformation is measured under an applied weight of 300~g, and the pressure is derived from the calibrated relation between loss of pressure and deformation. The design of an individual straw tube is shown in Fig.~\ref{st_ba_fig4}.

\begin{figure}[!h]
    \center{\includegraphics[width=0.6\linewidth]{Straw3}}
  \caption{A single straw tube for the  SPD barrel.
	}
\label{st_ba_fig4}
\end{figure}

\begin{figure}[!h]
    \center{\includegraphics[width=0.9\linewidth]{st_ba_6}}
  \caption{ Quality of the welding seams of 0.4 mm (left) and 0.85 mm (right) at $\times60$ magnification.
	}
\label{st_ba_fig5}
\end{figure}


\subsubsection{Straw conditioning}

Once the ultrasonic welding apparatus produces the straws, they need to be carefully stored, prior to installation into the detector. 
The straws need to be stored during a period of time that varies from several weeks to several months. 
The tube storage has several constraints that need to be addressed.
Namely, the inner diameter of the tube must remain free of dust and of foreign particles. The tube must also have the ability to be manipulated by technicians without buckling. With the above constraints in mind, it was decided that the optimal way to store the tubes would be under pressure. 
%This would also have the added value that the changes of pressure in a tube with respect to time could be observed. 
This would also have the added value of being able to observe changes in pressure in the pipe over time.
Straws that show gas leakage and have poor weld quality can be removed. 
Taking into account further quality control tests that are performed on the tubes before installation, and the manipulation of the tube itself during its installation into the detector, a dedicated system was developed, in the form of valves.
% as shown in Figure 26. 
For storage, the straws are gas-filled with an approximate overpressure of 1~bar. 
The pressure loss over time is measured indirectly by measuring the local deformation of a straw under a 300~g weight and comparing it to the day it was first subjected to pressure.
The first valve must have the ability to let gas into the straw, then act as a non-return valve, thus keeping the straw under pressure. The valve design is loosely based on the ''Dunlop'' / ''Woods'' valve design, with an additional feature. To prevent leakage through the non-return system, an O ring and  a threaded screw have been added. This is also used to fit the gas connector.

The second valve used at the other end of the straw tube is a simplified version without a non-return mechanism.
To run a leak test, we simply connect the test system to an M4 thread inside the valve and pressurize the straw. 
%To simplify Sagitta measurements of the simply supported tube both valves are of the same weight. 
To simplify measurements of the sagitta of a freely supported tube, both valves have the same weight.
In addition, the ends have the ability to be connected to the standard M4 threads. Furthermore, both valves have an outer diameter smaller than the straw tube outer diameter, which allow the installation of a straw tube under pressure.
%This facilitates the manipulation of the straws and limits the risk of buckling the straw wall and the welding seam.
This facilitates handling of the straws and reduces the risk of buckling  the straw wall and the welding seam.

\begin{figure}[!h]
    \center{\includegraphics[width=0.7\linewidth]{st_ba_7}}
  \caption{The straw production setup with an ultrasound head with movable fixation at the frame.
	}
\label{st_ba_fig6}
\end{figure}

\begin{figure}[!h]
  \begin{minipage}[ht]{0.52\linewidth}
    \center{\includegraphics[width=1\linewidth]{st_ba_9} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.48\linewidth}
    \center{\includegraphics[width=1\linewidth]{st_ba_8} \\ (b)}
  \end{minipage} 
  \caption{Welding seam width (a) and straw diameter (b) distributions.
	}
\label{st_ba_fig7}
\end{figure}

\begin{figure}[!h]
    \center{\includegraphics[width=0.7\linewidth]{st_ba_10}}
  \caption{Setup for the measurement of the straw sag and frequency as a function of different pre-tension and pressure. The computer is connected to an IR emitter and receiver (OPB732) to measure the frequency of the vibrating straw.
	}
\label{st_ba_fig8}
\end{figure}


\subsubsection{Mechanical properties and pre-tension of the straw}

In order to determine the necessary straw pretension, a dedicated setup was developed to measure the straw sag and the vibration frequency of the straws as a function of pressure, as shown in Fig.~\ref{st_ba_fig8}. 
%In order to simulate the effect of the vacuum, 
The straw was connected to a gas bottle, and the absolute pressure inside the straws was set to 2 bar. Four straws were glued horizontally into two plates. One straw was equipped with a sliding fixation on one end to allow for a variable straw pre-tension. 
%However, 
The sliding end of the straw was blocked (clamed ends) before measuring the deformation (sag) and frequency. 
The results of the measurements are shown in Fig.~\ref{st_ba_fig9}~(a). 
%The increase of the sag, as the pressure inside the straws increases, is clearly shown.
The increase in sag is clearly visible as the pressure inside the straw decreases.


\subsubsection{ Pressure influence}

A study of the straw sag as a function of overpressure at different pre-tension was carried out to determine the required straw tension. The results are shown in Fig.~\ref{st_ba_fig9}~(b). 
A minimum tension of 10 N is necessary to obtain an acceptable straw straightness. We have decided to apply a force of 15 N during installation,  in order to allow for some loss of tension over time.

\begin{figure}[!h]
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{st_ba_11} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{st_ba_12} \\ (b)}
  \end{minipage}
  \caption{(a) Measured sag and frequency of the straw as a function of pre-tension at different over-pressures. 
  (b) Straightness as a function of pressure for a 1.85~m long horizontal straw for different values on the pre-tension.
	}
\label{st_ba_fig9}
\end{figure}


\subsubsection {Wire centering and wire offset}

%Due to the length of the straw and the high voltage on the wire, a calculation of the effect from the electrostatic forces on the wire offset was carried out. 
In order to evaluate the effect of electrostatic forces on the wire, the dependence of the wire displacement on the straw length and high voltage was calculated.
%The displacement was calculated using the formula
The following formula was applied:
\begin{equation}
y=\frac{C}{k^2}(\frac{1}{\cos (kL/2)} -1),
\end{equation}
where $C=\rho g \sigma$ and $k$ is calculated using the expression
\begin{equation}
k^{2}=2\pi \epsilon_0 E_0^2(b)/T.
\end{equation}
Here $\rho$ is the density of the wire material, $\sigma$ is the cross-section of the wire, $T$ is the straw tension, $E_0$ is the field strength at the straw wall, $L$ is the length of the straw tube, and $\epsilon_0$ is the vacuum permittivity constant.

\begin{figure}[!h]
    \center{\includegraphics[width=0.7\linewidth]{st_ba_13}}
  \caption{The wire deflection for a 2.1~m long straw  with (blue dashed line) and without (red solid line)
  	electrostatic deflection at 2.5~kV.
	}
\label{st_ba_fig10}
\end{figure}


%\subsubsection{ Straw Signal}

%The results plotted in Figure~\ref{st_ba_fig10} shows an amplification of the wire sag of $\sim$27\%, due to the electrostatic forces. 
The results are presented in Fig.~\ref{st_ba_fig10}.
In the case when the voltage was set to 2.5~kV (slow gas) and the tension in the wire was set to 90~g,
the increase in wire sag due to electrostatic forces is about 27\% with respect to the case without electric field.
For the fast gas with a high voltage of 1.8~kV, the corresponding increase in the wire sag is 9\%.


\subsection{Detector response simulation}

\subsubsection{Choice of the gas mixture and high voltage operating point}

The initial choice of the gas mixture and high voltage settings was based on experience of the NA62 experiment \cite{NA62:2017rwk}, where the straw tracker consists of  the straw tubes of identical design. 
Its performance requirements are similar to those of the SPD straw tracker. 
The $Ar(70\%)+CO_2(30\%)$ gas mixture was demonstrated to provide the stable straw operation, sufficient spatial resolution and high detection efficiency. 
Moreover, it does not contain any flammable or non-ecological components. 
The optimal operation voltage was chosen to be 1750 V, which corresponds to a gas gain of about $4.5\times10^4$. In the case of  the NA62 experiment readout electronics,  based on the CARIOCA chip \cite{Moraes:2003rga}, 
such voltage allows for efficient operation with a spatial resolution better than 120 $\mu$m.

The straw spatial resolution and detection efficiency has been studied with the GARFIELD simulation software \cite{Veenhof:1993hz,Veenhof:1998tt} for the NA62 readout electronics models. 
The results as functions of the high voltage and signal discriminator thresholds are presented in Ref.\,\cite{Hahn:1404985} and are also  shown in Fig.~\ref{st_gar_0} . 
The considered discriminator thresholds correspond to 4, 10 and 15 fC of the charge induced on an anode wire. The results are shown for charged tracks crossing the straw at the distance of 3 mm from the anode wire. 
\begin{figure}[!h]
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{st_gar_01} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{st_gar_02} \\ (b)}
  \end{minipage} 
  \caption{GARFIELD simulation results for the straw spatial resolution (a) and detection efficiency (b) as functions of the high voltage and discriminator thresholds for a charged track crossing a straw at the distance of 3 mm from the anode wire \cite{Hahn:1404985}.
	}
\label{st_gar_0}
\end{figure}


\subsubsection{ GARFIELD simulation of the straw tube response}

Detailed studies of a straw tube response are ongoing for the SPD straw tracker operation environment. To evaluate influence of the SPD magnetic field on the tracker performance, GARFIELD simulation of the intrinsic straw response to a 1 GeV muon has been performed for two extreme cases of 0\,T and 1.5~T field, aligned with the straw longitudinal axis. Muon tracks are generated to be normal to the anode wire at the distance of 3~mm. 
Drift trajectories of the electrons produced in clusters of primary ionization for 0\,T and 1.5~T magnetic fields
are compared in Fig.~\ref{st_gar_1} (a) and (b), respectively. 

\begin{figure}[!h]
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{garfield_1} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{garfield_2} \\ (b)}
  \end{minipage} 
  \caption{Muon track (red), primary ionization clusters (green), and electron drift trajectories (yellow), simulated with GARFIELD for 0 T (a) and 1.5 T (b) magnetic field, aligned with the straw longitudinal axis.
	}
\label{st_gar_1}
\end{figure}

The relative coordinate of the primary ionizing particle is reconstructed from the measured electron drift time and is affected by its fluctuations, which, in turn, depend on fluctuations in the primary ionization cluster distribution,  together with longitudinal diffusion as well as on characteristics of the readout electronics. To evaluate intrinsic performance of the straw tubes, the drift time of the first and second ionization clusters arriving at the anode is studied as a function of the distance between the muon track and anode wire. No transformation of the straw signal by the readout electronics is implemented at that stage. Examples of the obtained time distributions for the first and second arriving clusters,  produced by a muon passing at a distance of 4 mm from the anode wire, are shown in Fig.~\ref{st_gar_2} for a magnetic field of 0\,T  and 1.5~T. Simulation is performed with the old Fortran version of GARFIELD and with the new GARFIELD++ package. A reasobable agreement between the two predictions was observed for both values of the magnetic field.

The width of obtained distributions does not exceed 0.3 ns even for the magnetic field of 1.5 T. This points to a negligible contribution of the cluster distribution fluctuations and electron diffusion to the straw time resolution. The influence of the magnetic field on the most probable arrival time is clearly noticeable, while the time distribution widths are not affected by the magnetic field aligned with the anode wire. The dominating influence of the readout electronics on the straw tube time resolution will be demonstrated later in Section \ref{RER}.

\begin{figure}[!h]
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{First_cluster_arrived_B0T} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{Second_cluster_arrived_B0T} \\ (b)}
  \end{minipage} 
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{First_cluster_arrived_B1_5T} \\ (c)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{Second_cluster_arrived_B1_5T} \\ (d)}
  \end{minipage} 
  \caption{ Examples of the obtained drift time distributions for the first (left) and second (right) arriving ionization clusters for a track passing at 4 mm from the anode wire for 0 T (top) and 1.5 T (bottom) magnetic field. To compare the most probable values (MPV) and the distribution widths (RMS), the GARFIELD (blue) and GARFIELD++ (black) predictions are fitted to a Landau distribution (green and red, correspondingly).	}
\label{st_gar_2}
\end{figure}

The most probable values (MPV) of the arrival time distributions, obtained for  field-free simulations using GARFIELD  and GARFIELD++ \cite{GARFIELDpp} packages as functions of a distance between the muon track and anode wire, are shown in Fig.~\ref{st_gar_3}~(a). 
The measurements performed at the NA62 experiment with the nominal tracker readout electronics are shown for comparison as a two-dimensional histogram. 
The simulation results are shifted by a constant delay to compensate for the time delays introduced by the readout chain in real measurements. 
Comparison of the MPV  obtained in the simulation  for a magnetic field of 0\,T and 1.5~T is presented in Fig.~\ref{st_gar_3}~(b).

\begin{figure}[!h]
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{Compare_Garfields} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{FitTimeResolution1} \\ (b)}
  \end{minipage} 
  \caption{The most probable drift time of the first arriving cluster simulated with GARFIELD and GARFIELD++. (a) Values obtained with GARFIELD (magenta points) and GARFIELD++ (cyan points) delayed with a constant value compared to the experimental results, obtained for an NA62 tracker straw (2D histogram)  and the most probable value of the experimental data (yellow). (b) Most probable values of the first cluster arrival time for 0 T and 1.5 T magnetic field. The simulation results are fitted to a quadratic function.
	}
\label{st_gar_3}
\end{figure}


\subsubsection{ Influence of realistic electronics readout on the straw time resolution \label{RER}}

Influence of the readout electronics on the straw spatial resolution is studied using a combination of GARFIELD and LTSpice \cite{LTspice} electronics simulation package. Individual straw signals simulated with GARFIELD are processed with LTSpice for a given electronics chain model. One of the possible SPD ST front-end electronics options, based on a VMM3a ASIC[REF], is considered in the study, and the corresponding model provided by the RD51 Collaboration (CERN) is used. Details of the readout electronics are described in Section~\ref{VMM3a_section}. 
%No magnetic field and electronics noise is accounted for at this stage.
At this stage, electronic noise and the influence of the magnetic field are not taken into account.

\begin{figure}[!h]
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{garf_signals_collection} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{signals_collection_spice} \\ (b)}
  \end{minipage} 
  \caption{(a) Signals induced at the straw anode due to an avalanche development as generated by GARFIELD for 1500 muons crossing a straw at the distance of 3~mm from the anode wire. (b) Corresponding electronics responses emulated with LTSpice.
	}
\label{st_gar_4}
\end{figure}

A current induced at the straw anode due to an avalanche development upon a muon crossing the tube at the distance of 3 mm from the anode wire as generated with GARFIELD is shown in Fig.~\ref{st_gar_4}~(a). 
1500~individual signals are shown together with the average trend. The corresponding readout electronics signals, emulated with LTSpice, are shown in Fig.~\ref{st_gar_4}~(b). The electronics chain model is set to describe the VMM3a operation mode with the shortest signal peaking time of 25 ns. A 10 mV signal discrimination threshold is chosen to correspond to 3~fC of the input charge. The time distributions of the first arriving cluster and the discriminator threshold crossing are shown in Fig.~\ref{st_gar_5} (a) and (b), respectively. In the case of realistic electronics, the time distribution is significantly wider. For the chosen electronics parameters, the time resolution was found to be 3.6~ns. 
The corresponding distribution, obtained with an NA62 straw readout with the original electronics, is shown  Fig.~\ref{st_gar_5}~(c). 
The time of the discriminator threshold crossing, measured for the relative muon track distances of $3.05\pm0.05$~mm, was obtained from the NA62 results shown in Fig.~\ref{st_gar_3}~(a).

\begin{figure}[!h]
  \begin{minipage}[ht]{0.32\linewidth}
    \center{\includegraphics[width=1\linewidth]{Fig6_left} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.32\linewidth}
    \center{\includegraphics[width=1\linewidth]{3mm_electronics_simulation} \\ (b)}
  \end{minipage} 
  \hfill
  \begin{minipage}[ht]{0.32\linewidth}
    \center{\includegraphics[width=1\linewidth]{3mm_NA62_projection} \\ (c)}
  \end{minipage} 
  \caption{Drift time distribution, obtained for first arriving clusters as simulated with GARFIELD together with a Landau fit (a), and the time distribution of the VMM3a-based readout electronics response, modeled for the corresponding signal sample with LTSpice for 25 ns peaking time and 10 mV discriminator threshold together with a Gaussian fit (b). (c) Corresponding distribution obtained with an NA62 straw readout with the original electronics. The time of the discriminator threshold crossing is measured for the relative muon track distances of $3.05\pm0.05$~mm.
	}
\label{st_gar_5}
\end{figure}



\subsection{Chamber design, construction and installation}

\subsubsection{Detector geometry and layout}

The mechanical construction proposed for  the SPD ST is based on engineering solutions, which were already efficiently applied in the ATLAS and PANDA experiments. The straw tracker consists of three parts: a barrel part and two end-caps. The barrel has inner and outer radii of 270 and 867 mm, respectively. It is subdivided azimuthally into 8 modules, with 31 double layers of straw tubes each, as shown in Fig.~\ref{fig:st_4_1}. The layout of a single module with the supporting frame are shown in Fig.~\ref{fig:st_4_2} and  Fig.~\ref{fig:st_4_3}.

\begin{figure}[!h]
    \center{\includegraphics[width=1.\linewidth]{st_4_1.png}}
  \caption{General layout of the barrel part of ST, which shows 8 modules (octants).
  Each module contains 31 double layers of straw tubes encased in a composite-polymer capsule.
  %Straws of adjacent double layers oriented perpendicular to each other.
	}
\label{fig:st_4_1}
\end{figure}

\begin{figure}[!h]
  \begin{minipage}[ht]{0.57\linewidth}
    \center{\includegraphics[width=1\linewidth]{st_4_2} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.35\linewidth}
    %\center{\includegraphics[width=1\linewidth]{st_4_2_1} \\ (b)}
    \center{\includegraphics[width=1\linewidth]{st_4_2_1_v2} \\ (b)}
  \end{minipage} 
  \caption{(a) Power frame of a single octant. (b) The barrel supporting frame for eight ST octants.
	}
\label{fig:st_4_2}
\end{figure}
\begin{figure}[!h]
    \center{\includegraphics[width=0.9\linewidth]{st_4_3.png}}
  \caption{Sketch of one module (octant) of the barrel part of the straw tracker.
	}
\label{fig:st_4_3}
\end{figure}


\begin{comment}
\begin{table}[htp]
\caption{Straw tubes in different layers of one octant of the ST barrel part.}
\begin{center}
\begin{tabular}{|c|cccccccccc|}
\hline
Layer &1&2&3&4&5&6&7&8&9&10\\
\hline
Angle, deg & 0&5.27&-5.65&0&6.43&-6.82&0&7.59&-7.97&0\\
Straws, pcs.&41&79&87&49&99&103&59&115&119&67\\
Total length, m&92.7&95.5&102.7&110.7&116.7&123.5&133.3&137.5&144.3&151.4\\
\hline
\hline
Layer & 11&12&13&14&15&16&17&18&19&20\\
\hline
Angle, deg&8.74&-9.12&0&9.88&-10.26&0&11.02&-11.4&0&12.15\\
Straws, pcs.&131&139&77&149&155&87&167&171&95&183\\
Total length, m&158.3&165.5&174&179.3&186.3&196.6&200.4&207.2&214.7&221.2\\
\hline
\hline
Layer  & 21&22&23&24&25&26&27&28&29&\\
\hline
Angle, deg &-12.52&0&13.27&-13.64&0&14.39&-14.74&0&10.61&\\
Straws, pcs.&186&105 &199&203&115&215&219&107&80&\\
Total length, m&228&237.3&242.1&248.9&259.9&263&269.8&241.8&200.4&\\
\hline
\end{tabular}
\end{center}
\label{tab:layers}
\end{table}
\end{comment}

\begin{table}[htp]
\caption{Straw tubes in different layers of one octant of the ST barrel part.}
\begin{center}
\begin{tabular}{|c|cccccccccccc|}
\hline
Layer           &1&2&3&4&5&6&7&8&9&10&11&12\\
\hline
Angle, deg  &  0&+5& -5&  0& +5&-5& 0& +5&  -5&  0 & +5 &-5 \\
Straws, pcs.&45&83&85&53&91&95&61&99&103&73 & 111&111 \\
\hline
\hline
Layer          &13&14&15&16&17&18&19&20&21&22&23&24\\
\hline
Angle, deg  &   0&+5&-5&0&+5&-5&0&+5&-5&0&+5&-5\\
Straws, pcs.& 81&119 & 123& 89& 127& 131& 99&139&139&109&147&151 \\
\hline
\hline
Layer          &25&26&27&28&29&30& \multicolumn{1}{c|}{31}  &  \multicolumn{1}{c|}{} &   \multicolumn{4}{c|}{Total} \\
\cline{1-8}
\cline{10-13}
Angle, deg  & 0&+5&-5& 0&0&0& \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{} & 0 & +5 & -5 & \multicolumn{1}{|c|}{0,$\pm$5} \\
Straws, pcs. &117&155&158&123&103&79&\multicolumn{1}{c|}{39} &  \multicolumn{1}{c|}{} & 1071&1071 & 1096& \multicolumn{1}{|c|}{3238} \\
\cline{1-8}
\cline{10-13}
\end{tabular}
\end{center}
\label{tab:layers}
\end{table}



The main axes of the straw direction are $Z$, $U$, $V$. The $Z$ axis is along the beam axis. 
The angle between the $U$, $V$ and $Z$ axes is $\pm5$~degree. The value of the angles by layers is shown in Table \ref{tab:layers}.
Each tube has a diameter of 9.8 mm. 
 %Eight modules are fixed together by a carbon fiber frame, thus forming a pair of independent semi-cylinders.
 %This design provides a possibility to assemble and disassemble ST in the presence of the beam pipe. 
Each module is enclosed in a 400~$\mu$m thick carbon fiber mesh capsule. 
The capsule provides the positioning of the individual straw tubes with a 50 $\mu$m accuracy. One side and two ends of the capsule have 5 mm holes, where straw end-plugs will be fixed. The FE electronic boards, which will be connected to these plugs, will additionally serve as the capsule covers, thereby isolating the inner volume from the external environment. 

The straw tubes will only be read out from one side. 
Each octant contains about 1100 tubes with parallel and about 2200 tubes with oblique angles to the beam direction. 
The total number of electronic channels per octant is 3238. 
Thus, the total number of channels in the barrel part of ST is $3238 \times 8 = 25904$. 
The rigidity of the structure is assured by the low overpressure of gas inside the tubes and their fixation inside the capsule volume. The anode wire positioning accuracy is achieved by the wire fixation in the carbon fiber covers. 
The capsule also serves to thermally stabilize the gas, circulating inside the detector volume, and to protect the straw surface from humidity. 
The sketch of one octant is shown in Fig.~\ref{fig:st_4_3}. 
One meter of straw tube has a weight of 1.15 g. %Only about 8000 m of straw. 
Thus, the weight of all the tubes in one octant with the glued end-caps is about 17~kg.


\subsubsection{Assembling the straw tracker}

Prior to the octant assembly, the straws of a proper length have to be prepared with the end-plugs glued to both ends of the straw. 
Layers $Z$, $U$, and $V$ will be installed one by one, forming the octant. 
Each straw of the stereo-layers $U$ or $V$ will have one end positioned at one of the octant ends, 
while the opposite end of the straw will be located at the octant side and will be connected to the gas pipes during the assembly.  

%To assemble the octant, one needs to prepare straw tubes of the required length for each layer. Then the end-plag should be glued into them at both edges. After that, layers Z, U, V should be put one by one and fill the octant in this way. The edges of layers U and V should be connected to the side of the octant with gas tubes.
A frame with precise holes for the straw end-plugs will be glued into the octant ends, maintaining the straw alignment. Then the anode wires are inserted into the straws, and their crimp tubes are connected to the flexible webs, as was implemented in the NA62 Straw Tracker and is shown in Fig.~\ref{fig:st_4_4}.  

At each end of the octant,  four front-end covers (one per an octant quarter) will be installed,  sealing the gas volume. A 50 $\mu$m thick mylar foil, plated with 50 nm of aluminum,  will be glued over the octant sides. Finally, carbon fibers will be glued onto the foil.

The ST installation procedure is demonstrated in Fig.~\ref{fig:st_4_5}.
Two separate halves of the carbon fiber frame are inserted into the inner volume of the SPD detector prior to mounting the  octants.
%, as shown in Fig.~\ref{fig:st_4_2}.
After that, the octants are installed into the frames one by one. 

\begin{figure}[!h]
    \center{\includegraphics[width=1.\linewidth]{straw_ass}}
  \caption{Picture of the straw end connectivity and gas manifold. A rigid-flex circuit board (web) connects high voltage to the signal wires and transmits the signal to the front-end cover. The cover also houses the high-voltage connector and feedthrough for the gas. 
	}
\label{fig:st_4_4}
\end{figure}

\begin{figure}[!h]
    \center{\includegraphics[width=1.\linewidth]{straw_ass_2}}
  \caption{Straw tracker installation procedure. Left: installation of the carbon frame. Right: installation of the pre-assembled ST octants. 
	}
\label{fig:st_4_5}
\end{figure}

\subsection{Detector components and assembly principles}
\subsubsection{Active web and wire connection}
A cross-section of the octant end mechanical structure holding the straws is shown in Fig.~\ref{fig:st_4_6}~(a). 
A carbon frame has holes for precise positioning of the straws and wires. 
The modularity in terms of HV, gas supply, and a readout system is represented by four sections containing about an equal number of straws. 
Removable partitions for the gas manifold and a dedicated polyurethane joint for gas tightness were developed. The partitions also serve as supports for the so-called cover, which contains the front-end electronics, high-voltage and gas connections.
%Between the straws and the frame are glued insulating sockets in polyetherimide (PET).
Polyetherimide insulating sockets are glued between the straws and the frame.


High voltage is transfered to the wire by an active web, which also transmits the signal back to the front-end electronics.
The  web is a multi-layer rigid-flex printed circuit board
%The active web is a multi-layer flex-rigid printed circuit board, which carries the high voltage to the wire and transmits the signal back to the front-end electronics. 
having two connectors per straw, namely one for HV and one for the signals. 
%The web connects to the backside of the cover, which is shown in Fig. \ref{fig:st_4_6}~(b). 
The web has a connector to be plugged  to the backside of the cover, as shown in Fig.~\ref{fig:st_4_6}~(b). 
The cover does not only provide the leak tightness of the manifold, it also comprises the front-end electronics, high-voltage and gas connections.

\begin{figure}[!h]
  \begin{minipage}[ht]{0.3\linewidth}
    \center{\includegraphics[width=1\linewidth]{st_ba_gas} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.7\linewidth}
    \center{\includegraphics[width=1\linewidth]{st_as_1} \\ (b)}
  \end{minipage} 
  \caption{(a) Four gas volumes of an octant. (b) Detail of the rigid-flex circuits board (web) that connects to the straws (ground) and the wire (high voltage and signal).
	}
\label{fig:st_4_6}
\end{figure}

The wire is tensioned and positioned using a copper tube inserted in the so-called connection, shown in Fig.~\ref{fig:st_4_7}. 
The copper tube connects to the second layer of the web, which brings high voltage to the wire and the signal back to the front-end electronics. 


\subsubsection{Measurement of the straw straightness}

Once the straws are fixed at both ends in the detector frame, their straightness is measured layer by layer with two light sources and a CCD camera/microscope. The two laser diodes illuminate the straw and the camera/microscope takes a photograph of the straw section. The system is calibrated using a wire stretched from top to bottom, parallel to the straws. A stepper motor moves the camera, and a picture is taken at 10 equidistant positions along the straw. A dedicated LabVIEW\textregistered~program transforms the pictures into a black and white image and finds the two straw edges automatically. The program then calculates the position of the straw center (straightness) in the $XY$-plane and the diameter of the straw.

\begin{figure}[!h]
  \begin{minipage}[ht]{0.32\linewidth}
    \center{\includegraphics[width=1\linewidth]{st_plugs} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.68\linewidth}
    \center{\includegraphics[width=1\linewidth]{st_tension} \\ (b)}
  \end{minipage} 
  \caption{(a) Connection plugs.	(b) Schematic view of the wire tension measurement device.}
\label{fig:st_4_7}
\end{figure}


\subsubsection{Wiring}

A gold-plated tungsten wire from Toshiba with a diameter of 30 $\mu$m is chosen for anode. The limit of elastic deformation has been measured up to 150 g and the rupture occurs around 220 g. The nominal wire tension is set to 90 g. The detector is placed in a horizontal position and the straw resistivity is measured. All straw diameters are measured and recorded in the logbook. The webs are then installed and the ground circuit is fixed to the inside of the straw with the help of the connection plug, which is shown in Fig.~\ref{fig:st_4_7}~(a). A tight fit is necessary to ensure a good electrical contact. The ground petals are formed with a special tool to facilitate the insertion of the PET plugs. 
A wire with a diameter of 0.1~mm (''needle'' wire) is blown through the straw.
The 30 $\mu$m wire is fastened to the needle wire and kept under a small tension at all times during installation to avoid kinks. The wire is gently pulled through the straw. From both sides, the 30 $\mu$m wire is inserted in the copper tubes and the copper tubes are then inserted through the electronic circuit into the contact plugs. Once the wire is fixed to the web side, a 90~g weight is suspended to the wire on the opposite side and fixed. The electrical continuity between the two pins is checked, as well as insulation between wire and straw (broken wire). After wiring one layer, the wire tension is measured and a HV test is performed to measure the leak current, which should not exceed 1~or~2~nA per high voltage group at 1600~V.


\subsubsection{Measurement of wire tension}

The full straw tracker contains a total of about 26000 anode wires, and the wire tension need to be verified during and after installation. The wire resonance frequency is close to 50 Hz for a tension of 80~g and a wire length of 2200 mm. 
Since 50 Hz is close to the frequency of the 220 V voltage supply, in order to avoid this frequency, the nominal wire tension was set to 90 g. The acceptable values of wire tension during the module production are between 85 and 95 g. The upper limit of 95 g is considered to be comfortably below the elastic limit of 150 g, while the lower limit is high enough to allow good operation of the straw. Electrical instability of the wire was found for tensions below 35 g. 
Therefore, to minimize electrostatic deflections on the wire, the lower limit is set to 85 g. 

%The wire tension measurement principle is shown in Fig. \ref{fig:st_4_7}(b): 
The principle of measuring wire tension is presented in Fig.~\ref{fig:st_4_7}~(b).
Namely, the wire oscillations are stimulated in an external magnetic field with the help of a current generator, 
and the resonant frequency of the wire is measured. The current induced on the wires will be amplified with a high-input impedance amplifiers and an input signal threshold (typically of about 1.5 mV). Signals will be digitized by a PC based A/D board and the measured frequency will be translated into applied wire tension $T$ (in grams), following the formula:
\begin{equation}
T=\frac{4\mu L^2 \nu^2}{a},
\end{equation}
where $L$ is the free wire length in cm, $\nu$ is frequency in Hz, $\mu$ is the mass per unit length in g/cm and $a$ is the gravitational acceleration. Uncertainties in the measured tension arise from variations in the wire diameter and the length of the vibrating wire. The minimum uncertainty can be estimated to be of about 1\%. The readout electronics, connected to a cell of 16 straws, measures the main resonance vibration frequency of each wire. The magnetic field near the tested wire must be at least 100 G. The operator can modify the parameters of the pulse generator and Fourier analysis on the Labview-based computer panel. The tension of the wires will be measured during the stringing process itself, and a final global wire-tension measurement of all wires in the module will be carried out before the next assembly step. The results of the measurement will be written to the production database. Loss of wire tension can happen between module assembly at the assembly hall and arrival at the SPD hall, so the wire tension will be measured again after delivery to the nominal position. Major attention will be paid to wires, which show a tension loss of more than 10 g. These wires will be investigated carefully and replaced if necessary.


\subsubsection{Gas tightness tests}

The next stage will be to verify the  joints glued between the straws and the frame. It is important to perform this test at this stage because the straws and their  joints  are still easily accessible and repairable in case of a problem. A dedicated gas-tightness setup is to be used to verify the quality of about 8000  joints (per octant), glued between the straws and their end-plugs, and 
between the end-plugs and the straw support frame. The system contains a temperature sensor, pressure gauges, vacuum stand and a system of valves and pipes. Straws and gas manifolds will be filled with Ar from a bottle with a pressure of 100~mbar above atmospheric pressure.
%a bottle with 100 mbar over atmosphere pressure. 
The  volume of the octant to be tested is about 1\,m$^3$. 
The leak rate (mbar$\times$ l/sec) will be evaluated by measuring the pressure drop inside the straws as a function of time, once the pump has been stopped. A module will be approved for subsequent assembly, whenever the measured leak rate does not exceed $10^{-2}$ mbar$\times$l/sec. Nevertheless, every effort will be made to get the leak value as low as possible.




% old place of FE (VMM) section



\subsection{Gas system}

The gas system consists of two parts. First, the mixer system which delivers quantity, mixing ratio and pressure conditioning to downstream elements. Second, the distribution system, which delivers the gas in well defined quantities to the individual detector components.

\subsubsection{ Gas system requirements}

The total gas flow chosen corresponds to a normal gas flow rate of ~2$\div$4 cm$^3$/min per straw. The gas modularity is optimized in order to minimize the number of lines between the detector and the distribution racks, and, on the other hand, to minimize the loss of performance in the case of an accidental leak in any module.

\subsubsection{	 Mixer}

The detector shall be supplied with a constant gas mixture of Ar:CO$_2$=70:30 with a precision better than 1\%. The total flow of the mixer will be 1500 l/h. Each primary gas line is equipped with a Digital Mass Flow controller to measure the component flow with appropriate accuracy. An output pressure regulator adjusts the downstream pressure from 0.2 to 2 bar. The control system provides a flow an independent mixing ratio and adequate error handling. The mixer has to automatically follow the demands of the distribution system. 

\subsubsection{	Gas distribution}

The gas from the mixer is distributed to the eight gas distribution racks, one for each octant. The major design criteria of the distribution system is the uniform gas supply to each cell with adequate separation capabilities, in case of pressure loss,  due to a leaking straw. Each octant is divided into four gas volumes, as  it is shown in Fig. \ref{fig:st_4_6}.

\subsection{Aging studies}

In order to validate the different components and materials  in the detector, a dedicated prototype was built. The prototype contains two straws: one with aluminium coating and another with copper/gold. The straw end-pieces were made from ULTEM, and the connection to the straws was made with a section of the web. The wire is the 30 $\mu$m gold-plated Tungsten from Toshiba,  foreseen for the chamber production. Final crimp tubes were used for electrical and mechanical connections of the wire to the web. The prototype was mounted in the CERN aging test facility. A gas mixture of 70\% argon and 30\% CO$_2$ was used. The parameters during the aging test are summarized in Table \ref{tab_aging_test}.
\begin{table}[htp]
\caption{Parameters of setup for aging testing.}
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Gas mixture & Gas flow & Current & Total charge & Irradiation  & High voltage & Fe-55 scan  \\
                    &                 &              &                     & area          &                       &  slit size \\
\hline
Ar (70\%)+ & 0.5 cm$^3$/min & 280 nA& 0.27 C/cm & 10 mm &1700 V & 1 mm  \\
 CO$_2$ (30\%)&                    &            & (500 hours) & & & \\
\hline
\end{tabular}
\end{center}
\label{tab_aging_test}
\end{table}%


A scan with a Fe-55 source is made at intermediate irradiation levels 
%over the window 
along the straw length
from 10~mm to 75~mm. The results are shown in Fig.~\ref{st_ba_fig13}. No change in amplitude can be seen up to a total  charge of 0.27 C/cm. The estimated accumulated charge for the hottest straws in the experiment is 0.04~C/cm. After the initial run with Ar/CO$_2$, it was decided to dismount the prototype and investigate the wire and the inner surface of the straw  around the irradiated region.
\begin{figure}[!h]
    \center{\includegraphics[width=0.9\linewidth]{st_ba_17}}
  \caption{ Straw prototype for material validation (left), mounted in the setup (right).
	}
\label{st_ba_fig12}
\end{figure}
\begin{figure}[!h]
    \center{\includegraphics[width=0.9\linewidth]{st_ba_18}}
  \caption{Scan of signal amplitude along the straw length for straws with  two types of coatings Cu/Au (left) and Aluminium (right). % , respectively. 
  Different graphs correspond to different accumulated charge.
	}
\label{st_ba_fig13}
\end{figure}


% old place for the ST cost estimate


%========================

\section{End-cap part of ST}

%The Endcap design of the internal SPD tracker has two features. 
The design of the ST end-cap has to satisfy the following criteria.
The detector must have the shape of a disk, have a relatively small central hole, %internal diameter, 
which is defined by a vacuum beam pipe, and have a small amount of matter in the sensitive region of the detector. 
The detection layers should be thin, and the number of layers should be sufficient to identify particles via $dE/dx$ measurement.

For efficient registration of interactions with a large multiplicity, a detector with 
%an octagonal arrangement of drift tubes array at 45 degrees, which 
drift tubes, arranged so that they form an $X$, $Y$, $U$, $V$ coordinate system, is proposed. 
Each coordinate plane consists of two halves separated by a distance for installation on a vacuum tube, as shown in Fig.~\ref{SEC_1}. 
All coordinate planes are mounted sequentially on a solid base that can be attached to other power element of the SPD detector.

\begin{figure}[!ht]
    \center{\includegraphics[width=0.7\linewidth]{EC_1.pdf}}
  \caption{General layout of the ST end-cap detector with drift tubes.
	}
\label{SEC_1}
\end{figure}
\begin{figure}[!ht]
  \begin{minipage}[ht]{0.25\linewidth}
    \center{\includegraphics[width=1\linewidth]{EC_2} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.377\linewidth}
    \center{\includegraphics[width=1\linewidth]{EC_3} \\ (b)}
  \end{minipage} 
  \begin{minipage}[ht]{0.32\linewidth}
    \center{\includegraphics[width=1\linewidth]{EC_4} \\ (c)}
  \end{minipage} 
  \caption{(a) Twisted structure of the straw tube. The picture illustrates a winding on a precision rod. The end-plug (b) and the crimping pin (c) are used to fix the anode signal wire.
	}
\label{SEC_2}
\end{figure}

It is possible to implement such a detector on the basis of thin-walled drift tubes, made by winding two "kapton" tapes, as shown in Fig.~\ref{SEC_2}~(a). The technology of manufacturing such detectors is being successfully developed in LHEP JINR. Over two decades, the straw chambers have been created for several large experiments, such as SVD-2 and Thermalisation at Protvino, ATLAS, COMPASS, and NA64 at CERN, CBM in Darmstadt, etc.

It is supposed to use straw tubes with a diameter of 9.56 mm, made of two layers of polyimide film.
The outer layer of the straw tube consists of a polyimide tape with a thickness of 25 microns. A copper coating with a thickness of 100 nm is applied on one side. The surface resistance is $1 \pm 0.1~\Ohm$/square. Polyurethane hot-glue coating with a thickness of 4 $\pm$ 1 $\mu$m is applied on the other side.
The inner layer of the straw tube consists of a similar polyimide tape. The layer of hot glue is applied to one side, and on the other  side - a layer of aluminum 0.2 $\mu$m thick. Graphite with a thickness of 6 $\pm$ 2 $\mu$m is applied on aluminum. The resistivity of this surface is about 10 $\Ohm$/square. The outer and inner tapes are glued together on a calibrated rod, as shown in Fig. \ref{SEC_2}~(a), heated to 170 $^{\circ}$C.


\subsection{Elements of technology for assembling twisted straw tubes}

Before assembling the detector or its parts, each straw tube is filled with precision steel balls with a diameter of $6.010\pm0.003$~mm or $9.525\pm0.003$~mm for the straw tubes of the corresponding diameter. Filling with balls occurs automatically. It takes about 1 minute to fill a 1.8\,m long straw tube. Tubes with balls are assembled into the size of a detector on a precision table and glued together to form a single straw array. Araldite 2011, VK-9, and ALK-5.8 are used for gluing planes and other structural elements. The amount of glue used does not exceed 60\% of the weight of the straw tubes. After removing the straw balls, the tubes are installed in a common plane on a large precision table.

\begin{figure}[!ht]
  \center{\includegraphics[width=0.7\linewidth]{EC_5}}
  \caption{Technical drawing (left) and photo (right) of the internal backing of the signal spacer wire.
	}
\label{SEC_3}
\end{figure}
\begin{figure}[!ht]
    \center{\includegraphics[width=0.9\linewidth]{EC_6}}
  \caption{Example of carbon fiber strips used as external  support for the straw tubes.
	}
\label{SEC_4}
\end{figure}

The end-plug and crimp pins, located at both ends of the straw, are used for the installation and positioning of the anode signal wire. The end-plug and the crimping pin are shown in Fig.~\ref{SEC_2}~(b) and (c), respectively. The positioning accuracy of the signal wire is not worse than 100 $\mu$m. The end-plug has a bronze spring contact that connects the inner conductive layer to the ground. It also has two longitudinal grooved channels for supplying a gas mixture.

Internal supports of the signal wire (spacers) are installed inside the tubes and serve to prevent sagging of the signal wires. 
Spacers are pre-glued to the signal wire in the tubes with a length of more than 800~mm. The drawing and appearance of the spacer are shown in Fig.~\ref{SEC_3}.

External supports serve to reduce the sagging of the straw tubes.
The support elements are made of thin carbon fiber plates, glued to the tubes.
An example of such elements is shown in Fig.~\ref{SEC_4}.
Transverse T-shaped strips of $0.5 \times 9$~mm$^2$ are used to increase the geometric stability of the transverse dimensions of the straw array, which are glued in the direction perpendicular to the straw axis of the tubes.

The positioning accuracy of each signal wire in the straw tubes is determined by the accuracy of the straw manufacturing and 
the accuracy of the plastic end-bushings and pins. 
The general positioning of the tubes in the detector plane is carried out on a precision table using precise rulers, 
as a result of which the accuracy does not exceed 0.1~mm.


\subsection{The main characteristics of  twisted straw  tubes}

The main characteristics of the drift detectors are given in Table \ref{EC_tab1}.
\begin{table}[htp]
\caption{Main characteristics of  the drift straw tubes.}
\begin{center}
\begin{tabular}{|l|c|}
\hline
Drift tube diameter & 6 $\div$10 mm\\
Gas amplification at 1800 V & $2.5\times10^4$ \\
 Operating voltage range &  200 V \\
Electron collection time for $B=0$\,T & 0 $\div$100 ns \\
Electron collection time for $B=2$\,T & +20\% \\
Registration threshold  &  2$\div$3 fC\\
Resolution when measuring drift time &  100$\div$200 $\mu$m \\
Registration efficiency for a two-layer detector at 1 MHz  & 99.7\% \\ 
Gas mixture & Ar:CO$_2$ = 70:30 \\
\hline
\end{tabular}
\end{center}
\label{EC_tab1}
\end{table}%


\subsection{Radiation properties of twisted straw tubes}

Properties of the materials that are usually used for  the straw production are given in Table \ref{EC_tab2}.

Figures  \ref{SEC_6} -  \ref{SEC_7} illustrate the results of calculating the radiation thickness of a straw detector consisting of two layers shifted by half the diameter of  the tubes. The tubes in each layer are glued together without gaps into a single coordinate plane.
\begin{table}[htp]
\caption{Characteristics of the materials used in the construction of the straw tubes.}
\begin{center}
\begin{tabular}{|l|c|c|c|}
\hline
Material & Density, g/cm$^3$ & Rad. length, g/cm$^2$ &  Rad. length, cm \\
\hline 
Tungsten, W     & 19.3          &    6.76   &  0.35  \\
Graphite, C      &    2.2          &   42.70 &  19.4 \\
Polycarbon Lex&   1.2           &   41.50  &   34.6 \\
Kapton             &   1.4           &   39.95  &   28.5 \\
%\red{CO$_2$}            &   1.84        &  36.2  &   19.7 \\
Acrylic (PMMA) &  1.19         &    40.55 &   34.1 \\
Polystyrene      &   1.06        &     43.79 &   41.3 \\
\hline
\end{tabular}
\end{center}
\label{EC_tab2}
\end{table}%

\begin{figure}[!h]
    \center{\includegraphics[width=0.5\linewidth]{EC_7}}
  \caption{%Typical arrangement of tubes in a two-layer detector with the second layer shifted by half the diameter.
  A typical arrangement of tubes in a two-layer detector, where the layers are shifted relative to each other by half the diameter.
	}
\label{SEC_5}
\end{figure}
\begin{figure}[!h]
    \center{\includegraphics[width=0.9\linewidth]{EC_8}}
  \caption{ Dependence of the thickness of the two-layer straw detectors in radiation units $x/X_0$ on the place of passage of the particle through the two layers of tubes for two diameters of a straw.
	}
\label{SEC_6}
\end{figure}
\begin{figure}[!h]
    \center{\includegraphics[width=0.9\linewidth]{EC_9}}
  \caption{ A more detailed picture for particles passing between tubes of the same layer. The figure on the left takes into account the adhesive layer between the tubes of the first layer and the substance of the signal wire 30 $\mu$m in the second layer. On the right, only the substance of the tube walls in two layers without signal wire and glue is taken into account.
	}
\label{SEC_7}
\end{figure}


\subsection{Coulomb scattering in the straw material}

A charged particle passing through the medium is deflected repeatedly on the nuclei of the medium. Most of this deviation is due to Coulomb scattering on the nuclei. For many applications, it is sufficient to use the Gaussian approximation for the projection of the angular distribution with a width of $\theta_0$, for the scattering medium in units of radiation length 
$10^{-3}< x/X_0 <100$:
\begin{equation}
\theta_0 = \frac{13.6~MeV}{p\beta c} z \sqrt{x/X_0} \times (1+ 0.038 ln(x/X_0).
\end{equation}

For 8 double-layer single-coordinate chambers with a diameter of straw 10 mm and a radiation
thickness $x/X_0=9\times 10^{-4}$ and for a single-charged particle with a momentum p = 1 GeV/$c$  the multiple scattering angle $\theta_0$ is $9.4\times 10^{-5}$ that corresponds to a deviation at a 1\,m baseline of 0.094 mm. For the straw tubes of 6 mm ($x/X_0=1.64\times 10^{-3}$) the corresponding numbers are $1.3\times 10^{-4}$ and 0.13 mm. For the detector frame material made of aluminum 0.8 cm, radiation thickness ($x/X_0 = 0.1$) the values $\theta_0$ and spatial deviation are  $3.7\times 10^{-4}$ and 0.37 mm, respectively.


\subsection{Humidity and ambient temperature. Influence on the parameters of the tubes}

The straw tubes are made  by winding of kapton tapes on a rod, followed by sintering. It is known that the walls of the tubes change their size depending on the temperature and humidity of the environment. During the development of straw detectors for the COMPASS experiment in 2002, estimates of the elongation value depending on humidity were carried out. 
The elongation of the straw tubes depending on humidity is shown in Figures \ref{SEC_8} and \ref{SEC_9}.
The test showed that the length of the straw tubes is preserved after they are dried with dry air, i.e.~the tubes have a range of elastic deformation.

The same study was carried out when creating straw detectors with copper-coated tubes for the NA64 experiment in 2019. 
As a result, the elongation value of the straw tubes was found to be $1.4 \pm 0.2$~mm/m for copper-coated tubes with diameters of 6~mm and 10 mm for a change in relative humidity from 50\% to 80\%.

\begin{figure}[!h]
    \center{\includegraphics[width=0.7\linewidth]{EC_10}}
  \caption{Dependence of the elongation of single tubes $\varnothing$6~mm and $\varnothing$10~mm with a length of 3.2~m employed in the COMPASS experiment \cite{Bychkov:2006xr}. 
A large spread of data is observed for different tube materials.
	}
\label{SEC_8}
\end{figure}
\begin{figure}[!h]
    \center{\includegraphics[width=0.85\linewidth]{EC_11}}
  \caption{ Effect of humidity on the elongation of tubes with a diameter of 10 mm and carbon/kapton coating.
	}
\label{SEC_9}
\end{figure}


The temperature coefficient of expansion of the straw tubes $25.2 \times 10^{-6}$ K$^{-1}$ is mainly determined by the material of the tube walls and does not depend much on the diameter and type of coating. Changing the temperature by 28 degrees elongates the straw tube by 0.7 mm. Elongating the tubes from humidity by 0.7 mm/m is equivalent to changing the temperature of the straw detector from 20 to 48 degrees. In our case, the detectors are in normal conditions at a temperature that will vary within 5$\div$10 $^\circ$C. This may cause a change in the length of the tubes by 0.1 $\div$ 0.2 mm/m. This temperature dependence must be taken into account when developing detectors. For comparison, the coefficients of thermal expansion of some materials that can be used for construction are (in units of 10$^{-6}$ K$^{-1}$): 23 for kapton, 18 for aluminium, and 27 for mylar.

The presented results show that it is advisable to install straw planes in the frame of the chamber at a temperature not higher than the operating temperature of the chamber and humidity not lowers than the corresponding
elongation %, mm/m
will be in the future. 
The effect of different operating and assembling temperature/humidity can be compensated by applying additional compressive forces to the frame elements during the assembling procedure, or by stretching the frame after installing the straw tubes, compensating for the influence of climatic factors.


\subsection{Mechanical properties of the straw tubes}

Mechanical tests were carried out for the straw tubes with a diameter of 6~mm and 10~mm. 
The tubes were subjected to stretching.
The test results are shown in Fig.~\ref{SEC_10}~(a), from which it can be seen that in order to compensate for the influence of humidity, it is enough to stretch the frame of the detector by 0.7~mm per meter of straw length. At the same time, it was shown that the tensile force applied to the tube of about 5.5~N does not cause plastic deformations of the tube for a long period. Measurements were carried out for about 2~years. When the twisted tube is stretched, twisting may occur. The study of this effect was done at high gas pressure inside the tubes. The practical absence of twisting was shown, see Fig.~\ref{SEC_10}~(b). The pressure of 2~atm stretches the tube with a force of 5.5 N (570~g of force).

\begin{figure}[!ht]
  \begin{minipage}[ht]{0.55\linewidth}
    \center{\includegraphics[width=1\linewidth]{EC_12} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.4\linewidth}
    \center{\includegraphics[width=1\linewidth]{EC_13} \\ (b)}
  \end{minipage} 
  \caption{(a) Elongation of straw tubes depending on the applied force. Round dots are for tubes with a diameter of 10 mm, while square dots for 6 mm tubes. (b) %The twisting angle of the straw under stretches by action of a pressure inside 6 mm straw tube. 
The twisting angle of a straw tube with a diameter of 6 mm when stretched under pressure. 
Angle is 1.1 degrees for 1 m long tube and tensile force of 5.5 N directed along the tube.
	}
\label{SEC_10}
\end{figure}

The tensile force can be created by excessive pressure inside the tubes when gluing the tubes into the frame. 
%However, the excess pressure inside the tube 
This pressure changes not only the tube length, but also its diameter. 
Thus, at an excessive pressure of 0.5~atmospheres, there is an increase in the diameter of the tube by 0.5~$\mu$m, which leads to a change in the positions of tubes and an increase in the width of the array of 288 tubes by 0.14~mm.


\subsection{End-cap design based on a two-layer array of twisted tubes}

End-cap is proposed with an octagonal arrangement of the drift coordinate planes at an angle of 45~degrees, which form an $X$, $Y$, $U$, $V$ coordinate system, see Fig.~\ref{SEC_11}~(a). In total, 8 coordinate planes are supposed to be used in one end-cap. Each coordinate plane consists of two halves of a disk with an interval for installing a vacuum tube. The thickness of one coordinate plane is 30 mm. Eight coordinate planes are mounted together, forming a rigid block, 240 mm thick. A free octagonal zone 150~mm wide is formed in the center of the block, in which a vacuum pipe of accelerator with a diameter of up to 100~mm is located. The assembled end-cap must be put on the vacuum tube and, together with the rest of the internal detectors, attached to the external part of the SPD installation. The common view of the end-cap is presented in Fig.~\ref{SEC_11}~(b).

\begin{figure}[!ht]
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{EC_14} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.48\linewidth}
    \center{\includegraphics[width=1\linewidth]{EC_15} \\ (b)}
  \end{minipage} 
  \caption{(a) ST end-cap consisting of 8 coordinate planes assembled together. (b) Common view and main dimensions.
	}
\label{SEC_11}
\end{figure}

\begin{figure}[!h]
    \center{\includegraphics[width=0.7\linewidth]{EC_16}}
  \caption{ %Eight coordinate planes with an interval for installing a vacuum tube are depicted.
	Four double-layer planes with a central gap for a vacuum tube are depicted.
	}
\label{SEC_12}
\end{figure}


As mentioned above, the tubes in the detector layers must be pre-stretched before gluing into the detector frame. For this purpose, a special technological frame is made, into which all the tubes of the array are glued before installation of  the signal wires. 
Frame size is $2 \times 2$~m$^2$, see Fig.~\ref{SEC_13}. Then the frame is stretched by mechanical screws together with an array of tubes to the required compensating size. The compensating elongation of the array of tubes should be $0.7 \times 2 = 1.4$~mm for  the tubes 2 meters long. An array of tubes is glued in a stretched state on a precision table into the detectors frame, and each tube is cut along the contour of the frame.
The second array is also glued to the technological frame with a half-shift in the diameter of the tubes, stretched and glued to the chamber frame from the reverse side. Frame thickness is 2 mm of carbon fiber, width is 50 mm.

\begin{figure}[!h]
    \center{\includegraphics[width=0.7\linewidth]{EC_17}}
  \caption{ Pre-tensioning device for straw arrays.
	}
\label{SEC_13}
\end{figure}

\begin{figure}[!ht]
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{EC_18} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{EC_19} \\ (b)}
  \end{minipage} 
  \caption{(a) Technological equipment for assembly. (b) Octagonal rotary platform and a portable honeycomb board for assembling are shown. The diameter of the portable board is 2300 mm, the thickness is 50 mm.
	}
\label{SEC_14}
\end{figure}


Each half of the array consists of 72$\times$2 = 144 straw tubes with a diameter of 9.56~mm. The width of the array is 688.3~mm.
There is a total of 288 tubes in  the two layers of one chamber, which must be pre-stretched with a force of 
5N$\times$288 = 1440~N (14.6~kg load). Calculations carried out in the Inventor program show that the deformation of the chamber's frame does not exceed 50~$\mu$m.
Further installation of the signal wires, gas supplies, and matching electronic circuits (motherboards) is carried out according to the proven standard technology.  The straw planes are assembled on a rigid portable honeycomb board on a rotatable octagonal frame shown in Fig. \ref{SEC_14}.

\begin{figure}[!h]
    \center{\includegraphics[width=0.7\linewidth]{EC_20}}
  \caption{One of eight coordinate planes with a central gap for the installation of a vacuum tube.
  A technological honeycomb portable board is also shown.
	}
\label{SEC_15}
\end{figure}


\subsection{Readout electronics placement}

The electronics, which are located directly on the chambers, perform the function of matching, amplifying and integrating straw charge signals, as well as providing high voltage to the signal wires of the detector. One straw layer consists of 288 registration channels. 9 ''motherboards'' and 9 amplifiers for 32 channels will be required to read information from one layer. The diagram of the 32-channel motherboard is shown in Fig.~\ref{SEC_16}. In total, for two end-caps with 16 coordinate layers of 4608 registration channels, 144 motherboards and 144 amplifiers will be required. Subsequent recording electronics are being developed and will be described in Section \ref{VMM3a_section}.
\begin{figure}[!h]
    \center{\includegraphics[width=0.8\linewidth]{EC_21}}
  \caption{The scheme of reading signals from one group of 32 straw channels -- ''motherboard''.
	}
\label{SEC_16}
\end{figure}


\subsection{End-cap design option with annular cylindrical frame}

 An end-cap will consist of eight ring straw chambers, deployed relative to each other. Each chamber consists of two layers of straw mounted in an annular carbon fiber frame with an outer diameter of 1510~mm and a thickness of 5~mm. Total thickness of  one end-cap is 400 mm. The straw layers are shifted relative to each other by the value of the straw radius, see Fig. \ref{SEC_17}. The rows are arranged along the chords of the frame. The working length of the rows in the chamber varies from 360~mm to 1500~mm, depending on the location of the rows. 
A section of the frame with holes, in which straw tubes are installed, is shown in Fig.~\ref{SEC_18}.

\begin{figure}[!h]
    \center{\includegraphics[width=1.0\linewidth]{EC_22}}
  \caption{Cross-section view of one chamber indicating possible layout of the readout electronics and gas manifolds.
	}
\label{SEC_17}
\end{figure}
\begin{figure}[!h]
    \center{\includegraphics[width=0.7\linewidth]{EC_24}}
  \caption{ Section of the frame with holes in which straw tubes are installed.
	}
\label{SEC_18}
\end{figure}
The straw tubes are glued individually into the frames under a tension of 500~g each, to avoid sagging of the straw tubes, possible due to high humidity. Also, to avoid sagging of the straw tubes in the chamber, 4 carbon fiber supports are used, shown in Fig.~\ref{SEC_17}, two on each side of the chamber. Each row layer contains 256 rows, 128 on each side relative to the center of the chamber.
After sealing the tubes, anode wires are installed in them under a load of 90 g each. As calculations have shown, the deflection of the frame after that will not exceed 30~$\mu$m.
Motherboards are glued from the end of the frame after installing the anode wires. Motherboards are designed to supply high voltage to the straws and connect the signal from them to the amplifiers. The boards are made in such a way that there are no gaps between the boards after being glued to the frame.
The ground contacts of all lines, as well as the signal pins are soldered using short insulated wires to the corresponding contacts on the board.
Then, a second carbon fiber ring with a thickness of 5 mm is glued to the boards with an outer diameter of 1570 mm. Gas connectors are installed in the ring to supply the working gas mixture to the straw tubes.

The resulting $\Pi$-shaped box is divided into 4 separate sections to ensure the decoupling of gas flows.
The box is hermetically sealed from above with fiberglass plates.






%\subsection{Front-end electronics}
\section{Front-end electronics}
\label{VMM3a_section}

%\subsubsection{Signal parameters, processing and straw properties}
\subsection{Signal parameters and processing}

%The basic detecting element is a straw drift tube of $\sim$10 mm diameter, 2.1 meter long. 
When registering electrons produced in the ionization process, the straw tube itself serves as a cathode, and the wire located in the center of the tube serves as an anode.
The cathode is formed by a very thin layer of copper and gold, few hundred atomic layers thick, so the electrical properties are determined by the surface effects (one does not need to consider the skin effect). Indeed, the measured DC resistivity of the cathode is $\sim$70~$\Ohm$, entirely determined by the surface effects. 
%The anode is 30 $\mu$m diameter gold plated tungsten wire. 
The anode is a gold-plated tungsten wire with a diameter of 30~$\mu$m.
The straw can be considered as a very lossy transmission line, and the termination effects on both ends should be evaluated. With the gas mixture Ar:CO$_2$=70:30, the electron's total drift time is about 150~ns.
As a response to each cluster of primary and secondary electrons, created by the passage of particle, the straw outputs a current signal with an approximately hyperbolical shape and few microamperes amplitude. The shape differs from a hyperbolical curve for the first few ns, due to the variable ion mobility. Also, when the selected gas would contain electronegative components, like CO$_2$, the signal becomes distorted and of smaller amplitude, due to an electron attachment. The leading edge of the signal is quite short, of the order of 1~ns, the trailing edge time depends on a number of factors like geometry, gas and voltage applied. 
The ion tail lasts up to several 100~$\mu$s. % of microseconds. 
The electrical properties of the straws are the following:

\begin{itemize}
\item characteristic impedance of 350~$\Ohm$ (calculated) at 20~MHz and 1000~$\Ohm$ at 1~MHz;
\item capacitance of 23~pF;
\item attenuation of 2.3 at 20~MHz;
\end{itemize}

%To achieve excellent coordinate, timing, and energy deposit resolution, the ST has the following requirements for the straw-tube readout electronics:
In order to achieve excellent resolution in terms of coordinates, time and energy deposit, the following requirements are imposed on the ST for the readout electronics of the straw tubes:
\begin{itemize}
\item possibility to measure both time and deposited charge;
\item  time resolution not worse than 1~ns;
\item low threshold to identify charge from a single cluster;
\item dynamic range better than 1000 for charge measurement;
\item low power consumption to reduce heating.
\end{itemize}

To address these requirements we propose a front-end electronics readout based on the VMM3a custom
Application Specific Integrated Circuit (ASIC). 
This ASIC will be connected to the straw anodes, providing precise charge and time measurements. 
Each  chip can read out 64 individual channels, making it appropriate for compact electronic boards, where high-channel density is useful. The low power consumption ($<$15\,mW/ch)  and cost per channel  ($\sim$0.9 \$/ch) are equally useful for a compact detector readout.
%Each channel on VMM3a chip is containing a fast programable gain preamplifier, semi-gaussian shaper, a tail cancellation circuitry, baseline restorer and a single threshold discriminator. 
A fast programable gain preamplifier, semi-gaussian shaper, a tail cancellation circuitry, baseline restorer, and a single threshold discriminator are integrated into each channel of the VMM3a chip.
Input impedance of the preamplifier  is a compromise between good straw impedance matching and a small crosstalk. The lower value is advantageous, as it guarantees lower crosstalk and signal enhancement due to current increase during signal reflection on low termination impedance. 
The reflected signal, which returns after traveling to the far end of the straw and being reflected backwards, is already strongly attenuated and does not contribute significantly to the output. 
The shaping time should be short enough, in order to get a response from the first primary cluster and, thus, better time resolution, 
but should be long enough to integrate all the clusters, so that there is only a single charge measurement per particle crossing the straw (150$\div$200~ns).


%\subsubsection{Employment of VMM3a ASIC for straw tubes readout}
\subsection{Employment of VMM3a ASIC for straw tubes readout}

For a conventional gaseous tube readout design, each channel generally has a double threshold discriminator (low/high) and a start/stop time digitizer. The rising edge of the signal (start) above the lower threshold is used for precise drift time measurement, and the track to wire distance is obtained from it with a known $r-t$ calibration. The trailing edge of the signal (end) is simultaneous for all straws crossed by the same charged particle, see Fig.~\ref{st_fee_1}. It is generally used for time measurement validation or even as a crude time measurement. It is also ideal for building a fast hardware trigger or veto for multiple charged tracks. The second higher threshold is used for the stray gamma detection and/or rejection. 
\begin{figure}[!h]
    \center{\includegraphics[width=0.9\linewidth]{st_ffe_1}}
  \caption{ The trailing edge of  signals is almost the same for all straws crossed by a single charged particle.
	}
\label{st_fee_1}
\end{figure}
VMM3a measures Time of Threshold with a built-in Time to Amplitude Converters, as shown in Fig.~\ref{st_fee_2}. It has different TAC slopes which can be set to 60/150/350/650\,ns. The preamplifier shaping circuit can be configured to use one of four different peaking times (25, 50, 100, and 200 ns) and eight gain settings (0.5, 1, 3, 4.5, 6, 9, 12, 16 mV/fC). A channel-specific discriminator is triggered on input signals above a configurable threshold to initiate digitization of the amplified pulse with a 10-bit Analogue to Digital Converter (ADC) and timing information with an 8-bit ADC.
\begin{figure}[!h]
    \center{\includegraphics[width=0.9\linewidth]{st_ffe_2}}
  \caption{ 
   Block diagram of one of the VMM3a channels with
   a timing diagram demonstrating the conversion of time to amplitude.
}
\label{st_fee_2}
\end{figure}
To sum up, VMM3a channel can measure time interval from threshold crossing to the falling edge of the reference clock pulse next after the peak of the integrated charge is found. For the collider application, VMM3a reference clock is set to a bunch-crossing clock. Thus, a time interval between the collision and the first cluster's arrival at the tube wire can be measured with a VMM3a chip.

VMM3a has no inner circuitry for trailing edge digitization, but it has 64 direct-time outputs that can be programmed to generate pulses for external use as time reference, veto signal, trigger, etc. Such a design requires an extra multichannel TDC, which would increase cost per channel.
Also, VMM3a provides an integrated charge measurement, which can be used for the gamma rejection in place of the second higher threshold.


%\subsubsection{ Noise and internal crosstalk, straw termination}
\subsection{Noise and internal crosstalk, straw termination}

The threshold setting is a compromise between time resolution and the rate of noise hits. 
The lower the threshold, the better the time resolution and efficiency should be, notwithstanding the higher rate of noise hits.
%As the straw detector also provides multiple charged particles veto signal, the noise must be as small as possible. 
The chip discriminator thresholds are adjusted in VMM3a by a global 10-bit Digital to Analogue Converter (DAC) with additional channel-specific 5-bit trimming DACs. 
%Combined these features allow the VMM3a to satisfy the STT requirement of the lowest threshold level for time measurements with low noise level at the same time.
These features enable VMM3a to meet the ST requirements of the lowest threshold level for time measurements,  while keeping noise at low level.



Scans of equivalent noise charge (ENC) of VMM3a  as a function of the input capacitance  for  various shaping time settings 
are shown in Fig.~\ref{st_fee_3}~(a). 
As can be seen, ENC of better than 1000 e- can generally be achieved 
with input capacitance less than 100~pF. 
Based on this information, we can assume that  VMM3a can likely meet the ST low charge threshold requirement, if the straw tube gain is greater than 10$^4$ with input capacitance lower than 100 pF. 
\begin{figure}[!h]
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{st_ffe_3} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.45\linewidth}
    \center{\includegraphics[width=1\linewidth]{st_ffe_4} \\ (b)}
  \end{minipage} 
  \caption{(a) Equivalent noise charge (ENC) of VMM3a as a function of the input capacitance for various shaping time settings.
   (b) ENC as a function of gain.
	}
\label{st_fee_3}
\end{figure}
Crosstalk can also cause fake hits, so multiple measures have been taken to reduce it as low as possible. For conductive crosstalk, the return paths of  the straw signals are separated already at the level of the web connection and kept until  the front-end board input connector. The capacitive coupling effect can be mitigated by lowering input impedance of the readout electronics and eventually by individual shielding of the straw cathodes. Input impedance is the sum of preamplifier input impedance and input discharge protection resistor. The input impedance of the VMM is about 50~$\Ohm$ at the working frequencies; the value of the protection resistor is of the order of 50 $\Ohm$, too. Thus, the total load impedance for straw is $\sim$100 $\Ohm$, to be compared with the 350 $\Ohm$ straw's characteristic impedance. The lower load impedance will cause signal reflections, but in a useful manner: it will increase the input current, thus enhancing the input signal. As the straw is a transmission line with very high loss, the signal which returns after reflecting from the far end of the straw is already negligible. The other possibility, considered for lowering capacitive crosstalk, is covering the straws from the outside by a very thin metallic layer, connected separately to the ground of the front-end board.
The straw's far end is left open. This should enable collecting as much charge as possible, as the straw has a very high attenuation (2.3) at working frequency.


%\subsubsection{External crosstalk, grounding and shielding}
\subsection{External crosstalk, grounding and shielding}

Electrically active objects surrounding the detector, such as a crane, a magnet, power supplies of other detectors, wireless connections, etc., can create interference, hereinafter referred to as external crosstalk. Another possible source of problems for the detector electronics is the mismatch in the voltage levels used in front- and back-end electronics. Therefore, it is necessary to ensure that all conductive parts are connected to a safety ground. The proposed grounding and shielding scheme for the ST detector is shown in Fig.~\ref{st_fee_4}. This scheme ensures that signals received from the cathode of the straws are separated and connected close to preamplifier inputs at the front-end board. This scheme was implemented in the 64-straw prototype. 
%External crosstalk is an interference with external objects surrounding the detector, like cranes, magnets, power supplies, wireless connections, etc. Another source can be caused by voltage potential difference between front and back end. One must also ensure connection of all conductive parts to safety ground. The proposed grounding and shielding scheme, shown in Fig.~\ref{st_fee_4}, ensures that the straw signal returns are separated and connected close to preamplifier inputs at frontend board level. This scheme was implemented in the 64-straw prototype.

The ground of the front-end board is connected along its perimeter to a metal case that  surrounds the whole detector, thus forming a tight electromagnetic shield. The conductive layer of the straw tubes is grounded only on one end to prevent external currents flowing through the cathodes. All cable shields are connected on both ends: one side directly to the front-end board, back-end side through damping impedance. 
%The ground of the frontend board is connected around its perimeter to metal case, which is surrounding the whole detector, thus forming tight electromagnetic shield. Straws are connected to signal returns only on one end to prevent external currents flowing through the cathodes. All cable shields should be connected on both ends; one side directly to frontend board, backend side through damping impedance. If there are metallic pipes servicing gas or cooling, they should be electrically connected to metal frame as well.
\begin{figure}[!h]
    \center{\includegraphics[width=0.65\linewidth]{st_ffe_5_v2}}
  \caption{Grounding and shielding scheme of ST.
	}
\label{st_fee_4}
\end{figure}
All metallic pipes for gas supply or cooling of the ST detector will also be electrically connected to the metal frame. The metal case of the station should be connected to safety ground at one point. The back-end electronics (VME crates) must be connected to the same ground, thus providing both required safety connection and eliminating potential difference between front-end and back-end electronics. 
%The metal case of the station should be connected to safety earth at one point. The backend electronics (VME crates) must be connected to the same earth, thus providing both required safety connection and eliminates potential difference between frontend and backend electronics.

High channel density of VMM3a leads to small front-end PCB outlines, allowing digitizers to be set up directly inside the shielded metal case, resulting in even lower ambient noise levels.

%High channel density of VMM3a leads to small front-end PCB outlines, allowing to set up digitizers directly inside the shielded metal case resulting with even better external noise levels.


%\subsubsection{Studies with a prototype straw readout based on VMM3a and SRS system}




\section{DCS}
\subsection{ DCS architecture}
The Detector Control System (DCS) provides control and monitoring of the detector hardware. In addition, it will perform archiving of the hardware parameters to the database to provide access to this information during the offline data analysis. It has been decided to use the common DCS system, now under development at CERN, which is based on the PVSS II SCADA toolkit and the JCOP framework. The Straw Tracker controlled and monitored equipment includes the following items:
\begin{itemize}
\item low voltage power supplies;
\item high voltage power supplies;
\item gas mixing and distributing systems;
\item low voltage and temperature monitoring system.
\end{itemize}

\subsection{ Low voltage system}
The LV system provides power to the front-end (FE) boards placed on the four straw tracker chambers. Each chamber contains four views and each view contains 30 FE boards. In the present design, one FE board consumes ~ 1 A at 5 volts and, therefore, one module requires the LV power supply to provide a current of about 30A at 5 V. These requirements could be fulfilled by eight Wiener power supplies MPV8008, which have eight channels of 10 A output current each. One view requires four channels and, therefore, two power supplies will provide the required power for one chamber. The MPV8008 could be controlled in a similar  solution used in the LHC experiments. It includes a CAN-bus interface card and the OPC-server providing the interface to PVSS. A second possibility to control the MPV8008 is to use the TCP/IP protocol together with the corresponding TCP/IP PVSS driver, which is part of the PVSS driver package. %The final choice of the FE electronics and corresponding LV power supplies will be made once the results from the 2010 test beam with the 64-straw prototype are known.

\subsection{ High voltage system}
The Straw Tracker requires a high-voltage (HV) source with voltage below 2 kV and low current. The present design assumes two HV channels per view, with 32 channels in total. The CAEN HV power supply board A1535, containing 24 channels with 3.5KV/3mA output, should be sufficient. To have 32 HV channels, two boards of this type, housed in CAEN SY2527LC mainframe, are needed. The mainframe should be controlled via Ethernet line with TCP/IP protocol and corresponding CAEN OPC server. The JCOP framework is suitable for the board A1535 and is already available, having been developed for the CMS ME1/1 muon chambers.
	
\subsection{ Gas system controls}
The gas system for the straw tracker should provide and distribute Ar/CO$_2$. Due to the fact that the straws are placed in the inner layers of the detector, the gas system should rapidly close the gas line to a cell, in case of a leak in a straw. Pressure sensors will detect a sudden drop in pressure on the supply lines. In this case, the gas system should also send a signal to the Straw Tracker DCS to switch off the corresponding HV channels or the whole HV system. 
%gas mixture to individual straw cells. 
The plan is to use the CERN standard gas mixing/distribution system based on PVSS, with the possibility to control and monitor the gas mixing and gas flow values from the DCS PC. For this purpose, PVSS distribution manager will be used. Both software and hardware interlock signals to prevent HV turning on, if the gas flow is missing or an incorrect gas mixture is distributed.

\subsection{ Thermometry and FE monitoring}
In order to get information about the cover (front-end) temperature at the straw group inlet, one thermo-sensor per FE cover will be mounted. Two voltages (one for the FE boards and  one for the current consumed by a board) will be measured using Embedded Local Monitoring Boards (ELMBs). A chamber view has 30 boards, and four thermo-sensors will be mounted directly on the mechanics structure. In total, one view needs to measure 34 temperature values and 90 voltages. Therefore, to read out all monitoring information from one chamber, 10 ELMBs are needed. The readout should be performed via CAN-bus and OPC server, which is similar to monitoring the LV power supply. It seems reasonable to have one CAN-bus branch per chamber, which gives four CAN-bus branches in total. In case the LV power supplies control protocol is compatible with the ELMB control protocol, the LV power supplies will be connected to the chamber CAN-bus branches. The final decision depends on the final choice of the FE electronics.

\subsection{ Logical trees in DCS and FSM}
To get a convenient way of navigation through the detector elements, the DCS logical tree will have a structure including both tracker nodes and gas system nodes. Due to the fact that the detector has only a few LV and HV channels, the bottom node of the tree will be linked to the corresponding channel of the LV or HV power supply in the hardware tree. The FSM tree should correspond to the Straw Tracker logical tree. The states of FSM should correspond to the states of the whole detector.

\subsection{ 	 DCS development and maintenance}
The plan is to use our own DCS PC running tracker PVSS system and  DCS OPC servers for all detectors on one Windows-based computer. This PC should have CAN-bus adapter cards installed. After the development is finished and to simplify the maintenance of the detector DCS, the plan is to create a JCOP FW component containing all tracker PVSS panels and scripts, and to port it to the SPD central DCS computer. A copy of this component should be stored in the SPD DCS repository. The ST DCS PC should be used to run the DCS servers and to house the CAN-bus adapters. 
To simplify the control of the detector during further hardware development, debugging and maintenance, the PC to access PVSS panes located at the central DCS PC, will be used. 
For this purpose, the DCS PC will be equipped with a PVSS User Interface software installed.

\section{Cost estimate}
\subsection{ST barrel}

The configuration for the proposed ST is based upon 8 octant in the barrel part. Each octant contains about 3200 straws. 
%Assuming a single readout at one end of the straws
Assuming one-end reading for each straw, the total number of electronic channels is about 26\,000. 
The core cost is estimated for the construction of the complete ST, using a mixture of updated quotes from vendors, costs of the similar detector components used in different experiments. 
The risk associated with the project is relatively small. The ST design is based upon well established technology, using low mass straws, successfully developed for various modern projects. This does not require serious research and development in the field of detectors.

The corresponding costs for the various items of the ST barrel are summarized in Table \ref{cost_barrel}.
%
\begin{table}[htp]
\caption{Cost estimate for the barrel part of ST.}
\begin{center}
\begin{tabular}{|l|c|}
\hline
Item   & Cost, k\$ \\
\hline
Straw tubes   & 220\\
Glue      &  20\\
End-plugs & 100\\
Crimping pins & 90 \\
Anode wire  &  60 \\
Other  components & 90 \\ 
\hline
Mechanics \& C-fiber frames & 200 \\
ST tools & 160 \\
Safety equipment \& consumables & 60\\
Gas system  & 300 \\
Cooling system  & 130 \\
\hline
Front-end electronics (VMM3 \& boards) & 500\\
Back-end electronics  & 300 \\
HV components & 200 \\
LV components & 200 \\
Cables \& connectors  & 150 \\
\hline
Prototyping  & 320\\
\hline
\hline
Total   & 3100 \\
\hline
\end{tabular}
\end{center}
\label{cost_barrel}
\end{table}%

\begin{comment}
\begin{table}[htp]
\caption{Cost estimate for the barrel part of ST.}
\begin{center}
\begin{tabular}{|l|c|}
\hline
Item   & Cost, k\$ \\
\hline
Straws   & 180\\
Glue      &  10\\
End-plugs & 80\\
Crimping pins & 70 \\
Anode wire  &  50\\
Other  components & 70 \\ 
\hline
Mechanics \& C-fiber frames & 120\\
ST tools & 120\\
Safety equipment \& consumables & 50\\
Gas system  & 200\\
Cooling system  & 100\\
\hline
Front-end electronics (VMM3 \& boards) & 280\\
Back-end electronics  & 120\\
HV components & 80\\
LV components & 80\\
Cables \& connectors  & 90 \\
\hline
Prototyping  & 320\\
\hline
\hline
Total   & 2020 \\
\hline
\end{tabular}
\end{center}
\label{cost_barrel}
\end{table}%
\end{comment}



%\subsection{Cost estimate}
\subsection{ST end-caps}

The configuration for the proposed ST is based upon 16 double-layer modules in two end-cap parts (8~modules on each side). 
Each module contains 288 straws. 
Assuming one-end reading for each straw, the total number of electronic channels is 4608.

The corresponding costs for the various items of the ST end-cap are summarized in Table \ref{EC_tab3}.
%Cost estimate for {\blue the ST end-caps}  is presented in Table \ref{EC_tab3}.
%+ 240 k\$ FFE (?)
%
\begin{table}[htp]
\caption{Cost estimate for the end-cap part of ST.}
\begin{center}
\begin{tabular}{|l|c|c|c|c|}
\hline
Unit & Quantity & Unit cost, \$ & Total cost, k\$ \\
\hline
Straw tubes  (3m/straw), m & 15000 & 2.5 & 37.5 \\
Anode wire   (4m/straw), m & 20000 & 2    & 40    \\
Pins                                     & 10000 & 3    & 30    \\
End plug                              & 10000 & 2    & 20    \\
Spring contact                     & 10000 & 2    & 20    \\
Spacers                               &  5000  & 1    &  5     \\
Glue, chemical materials, consumables &&&  1     \\
\hline
Straw frame                         &      16 & 3000 & 48 \\
Rigid flat mounting frame    &        2 & 6000 & 12 \\
Covers for frames                &      80 &  100 &   8 \\
Frame for tension                 &       2 & 2000 &  4 \\
Precision rulers for 16 straw, combos & 3000 & 10 & 30 \\
Measuring table for alignment & 1 & 3000 &  3 \\
\hline
Prototype                             & 2 & 25000 & 50 \\
Gas equipment                    & & & 20 \\
Tension control equipment  & 1 & 5000 & 5 \\
Tooling for cutting                & 2 &  500 &  1 \\
\hline
Motherboard plate and frontend & 150 & 1600 & 240 \\
\hline
\hline
 Total & &  & 574.5 \\
\hline
\end{tabular}
\end{center}
\label{EC_tab3}
\end{table}


\section{Identification of particles using energy loss $dE/dx$ in straw tubes}
%\section{ $dE/dx$ particles identification with straw tube detector}

The ST  will be the only detector able to separate $\pi$/$K$/$p$ during the first stage of the SPD experiment, and its performance is crucial for many physics tasks suggested in Ref.~\cite{Abramov:2021vtu}. Particle identification in the detector is based on measurements of  ionization energy losses. The energy losses follow the Landau distribution and are subjected to strong fluctuations due to rare acts of ionization with large energy loss. 
A truncated mean method is used to achieve a good resolution.
 For this method a certain fraction (10~--~50\%) of signals with the highest amplitudes are discarded. The obtained mean value can be compared to different particle hypotheses and the corresponding probability can be assigned for each particle type.

The full simulation of PID performance must include description of the straw tracker, simulation of the ionization losses and gas gain in tubes, and response of the electronics. The simplified simulation accounting for the first two points within the SpdRoot framework has been performed, the impact of the electronics will be discussed later. The resolution dependence on the fraction of discarded signals is shown in Fig.~\ref{fig:dedx-trancation-par}  for the barrel part of the detector.  One can see that it weakly depends on truncation parameter in the range 0.3~--~0.6. For the following estimations this parameter is set to 35\%. 
The truncated mean value of $dE/dx$ calculated per track as a function of momentum follows the Bethe-Bloch distribution
and is shown in Fig.~\ref{fig:dedx-performance} for tracks crossing the ST barrel and the ST end-caps.
The particle separation capability for pions, kaons, and protons can be estimated from curves indicating $1\sigma$ and $3\sigma$ displacement intervals.

%The particle separation capability as function of their momentum for electrons, pions, kaons, and protons is shown in Fig.~\ref{fig:dedx-performance} for barrel and endcaps.

\begin{figure}[htb]
    \centering
    \includegraphics[width=.55\textwidth]{truncation_par.png}
    \caption{Dependence of the truncated mean resolution on the fraction of discarded signals for tracks, reconstructed in the barrel part of the ST detector.}
    \label{fig:dedx-trancation-par}
\end{figure}

\begin{figure}[htb]
    \centering
%    \includegraphics[width=.75\textwidth]{dedx-b}
%    \includegraphics[width=.75\textwidth]{dedx-ec}
   \includegraphics[width=.75\textwidth]{dEdx_vs_p_b}
    \includegraphics[width=.75\textwidth]{dEdx_vs_p_ec}
    \caption{The performance for particle identification with $dE/dx$ in the straw tracker. The dashed and dotted lines indicate $1\sigma$ and $3\sigma$ intervals, respectively. The upper plot shows tracks reconstructed in the ST barrel, the lower~---~in the ST end-caps.}
    \label{fig:dedx-performance}
\end{figure}

In general case, the signal amplitude is defined by a convolution of raw signal and the electronic response function. 
For the long shaping time, the amplitude will depend on the collected charge only. 
In our case, the shaping time setting for VMM3 is 100 or 200~ns, and the total drift time is about 100~ns for a 10~mm straw tube. The charge collection efficiency in this case will depend on the signal shape, which depends slightly on the track-to-wire distance. The signal duration for tracks coming close to the wire is much larger as compared to tracks passing at large distances. This requires to introduce amplitude, which can be done in a routine way.




==> tex/TDR_magnet_JINR.tex <==
\section{JINR option}
Main distinctions between the SPD magnet and the existing or projected magnets for detectors of particles are the design features of the solenoid. The technology using a hollow composite superconducting cable, proposed in the Veksler and Baldin Laboratory of High Energy Physics (VBLHEP) and well-proven in magnets of the synchrotron Nuclotron \cite{402687}, was chosen as the basis for its production. In this case, the winding is cooled by the circulation of a supercritical helium flow in the cooling channels of a hollow cable.
The SPD magnet is designed to create a uniform magnetic field with a nominal induction of 1 T in its aperture. The Superconducting Solenoid will be surrounded by an iron yoke, designed to close the magnetic flux and form a magnetic field with the required uniformity.

           The requirements to the SPD magnet are:
\begin{itemize}
\item maximum field on the solenoid axis -- $B_z\geq 1$ T;
\item uniformity of the magnetic field on the axis -- $dB_z/B_z \leq 0.05$;
\item diameter of the ''warm'' aperture -- 3.2 m;
\item solenoid length -- 3.8 m.
\end{itemize}
\subsection{Solenoid design}
The technology using a hollow composite superconducting cable (Fig. \ref{Mag1}), proposed at VBLHEP and well-proven in magnets of the Nuclotron, was chosen as the basis for the production of the solenoid. VBLHEP has a base for the production of such a cable, which only requires an upgrade of the existing equipment.

Since the solenoid operates at a constant current value, the SC wires can be soldered to the cooling tube, and the tube can be made of copper. Unlike the Nuclotron cable operating in a pulsed magnetic field, the SPD solenoid cable does not have a fixing wire.
A solenoid with an average winding radius of 1.742 m and a length of 3.8 m should have a high uniformity of the magnetic field in the aperture. The two-layer winding is planned to be made of 10 coils (see Fig. \ref{Mag2}~(a)) of 2 sections each. The 0.38 m coil, as it is shown in Fig.\ref {Mag2}~(b), contains 30 turns of a hollow superconducting cable.
\subsection{Solenoid from the Nuclotron-type superconducting cable }
\begin{figure}[!h]
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{MAG_JINR_1} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.49\linewidth}
    \center{\includegraphics[width=1\linewidth]{MAG_JINR_2} \\ (b)}
  \end{minipage} 
  \caption{ (a) Hollow SC cable of the Nuclotron and (b) the SPD solenoid: 1 -- a tube with a channel for cooling; 2 -- SC wire; 3 -- fixing wire; 4 -- polyimide tape; 5 -- glass fiber tape impregnated with epoxy compound for hot hardening.
	}
\label{Mag1}
\end{figure}
\begin{figure}[!ht]
  \begin{minipage}[ht]{0.29\linewidth}
    \center{\includegraphics[width=1\linewidth]{MAG_JINR_3} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.69\linewidth}
    \center{\includegraphics[width=1\linewidth]{MAG_JINR_4} \\ (b)}
  \end{minipage} 
  \caption{(a) SPD solenoid of 10 coils. (b) Coil winding with two sections.
	}
\label{Mag2}
\end{figure}
\begin{figure}[!h]
    \center{\includegraphics[width=0.8\linewidth]{MAG_JINR_5}}
  \caption{Elements of the SPD solenoid coil.
	}
\label{Mag3}
\end{figure}
The SPD winding of 10 coils is carried out on a mandrel, made of stainless steel. Profiled copper inserts are laid below and above each layer of the coil (see Fig. \ref {Mag3}), filling the voids between the turns. At the bottom of each layer of the coil, shunts are laid-winding heaters, which are necessary to protect against overheating at quench. A bandage of stainless steel wire is wound over the coil. After the winding of both sections of the coil, the coil is heat-treated to polymerize the epoxy compound. The coils are assembled together on a special device. In this case, the mandrels of the individual coils are mechanically interconnected. Then, the helium cooling lines of the solenoid are connected, and the electrical connections between the coils are made.

\begin{figure}[!ht]
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{MAG_JINR_6} \\ (a)}
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.5\linewidth}
    \center{\includegraphics[width=1\linewidth]{MAG_JINR_7} \\ (b)}
  \end{minipage} 
  \caption{$B_z$ as a function of radius (a) for various distances from the center of the solenoid and distances  (b) from the center of the solenoid for various radii. Detector working area is $Z \leq 1900$ mm, $r \leq 1570$ mm.
	}
\label{Mag4}
\end{figure}
\begin{figure}[!ht]
    \center{\includegraphics[width=1\linewidth]{MAG_JINR_8}}
  \caption{ Magnetic field lines.
	}
\label{Mag5}
\end{figure}

The magnetic and stress calculations have been performed using the OPERA simulation software. The value of $B_z$ component equal 1 T at the axis of the magnetic system is achieved by the current in the coils of 5067 A. The variation of $B_z$ at the axis is less than 5\%, which satisfies the requirement of the SPD magnetic system. The maximal value of the forces acting between the neighboring coils is 1.36 MN. The pressure of the magnetic field on the solenoid is 0.398 MPa. Dependence of $B_z$ on radius $r$ and $z$ coordinate is shown in Fig. \ref {Mag4}.  The magnetic field lines of force are shown in Fig. \ref {Mag5}. 

The characteristics of the SPD cable and winding are presented in Table \ref{mag_jinr_tab1}.

\subsection{Cooling system}
The solenoid winding is cooled by a supercritical pressure helium flow, which is pumped inside the cooling channel of the cable. In total, there are 20 parallel cooling channels (10 coils of 2 sections each). Each section of the solenoid is connected in parallel to the supply and return helium collectors. The operating temperature of the winding is 4.8 K, the nominal flow rate of liquid helium through the solenoid is about 16 g/s. The cold mass of the solenoid is about 7.9 tons. Cooling of the solenoid is planned by a helium refrigerator with a nominal cooling capacity of 100 W, which will be installed close to SPD. Some characteristics of the cold mass and cooling system are presented in Table \ref{mag_jinr_tab2}. 

\begin{table}[htp]
\caption{Characteristics of the SPD solenoid.}
\begin{center}
\begin{tabular}{|l|c|}
\hline
\multicolumn{2}{|c|}{Cable} \\
\cline{1-2}
\hline
Parameter & Value \\
\hline
Helium cooling channel diameter, mm & 4\\
Cooling tube outer diameter, mm & 5\\
Cooling tube material 	& Cu\\
Number of strands		&19\\
Lay pitch of strands, m	& 0.1\\
Diameter with insulation, mm &	7.44\\
Copper sectional area, mm$^2$ &	15.77\\
Superconductor sectional area	mm$^2$	& 3.38\\
Cu/SC ratio	&	4.66/1 \\
Length in section, m	& 328.3 \\
Total length in the winding, m &	6566 \\
\hline
\multicolumn{2}{|c|}{Strand} \\
\cline{1-2}
\hline
Diameter, mm	& 0.9 \\
Superconductor & Nb--Ti/Cu \\
(Nb--Ti)/Cu -- volumetric ratio	&	1/2.57 \\
Nb--Ti filament diameter, $\mu$m &	7 \\
Operational current $I_{max}$, A &	270 \\
Critical current at 2 T and 4.2 K, A &	$\geq$ 670 \\
\hline
\multicolumn{2}{|c|}{Supporting cylinder} \\
\cline{1-2}
\hline
Inner diameter, m  &	3.455 \\
Outer diameter,	m  &	3.465 \\
Material	&	Steel 12X18H10T \\
\hline
\multicolumn{2}{|c|}{Winding} \\
\cline{1-2}
\hline
Nominal (maximal) magnetic field $B_0$,	T & 1.0 \\
Inner diameter, m &	3.465 \\
Outer diameter, m & 3.498 \\
Length,  m	& 3.8\\
Number of layers	&	2 \\
Number of winding sections	&	2 $\times$10 \\
Number of turns	&	$30 \times 2 \times 10$ \\
Operational current $I_{max}$,	A	& 5067 \\
Inductance  $L$,	H	& 1.144 \\
Stored energy $E$ at $I_{max}$, MJ	& 14.7 \\
\hline
\end{tabular}
\end{center}
\label{mag_jinr_tab1}
\end{table}%

\begin{table}[htp]
\caption{Some characteristics of the SPD solenoid cold mass and cooling system.}
\begin{center}
\begin{tabular}{|l|c|}
\hline
\multicolumn{2}{|c|}{Cold mass at 4.8 K, kg} \\
\cline{1-2}
\hline
Parameter & Value \\
\hline
Cu in conductor, $M_1$	& 560 \\
Cooling tube, $M_2$	 & 413 \\
Cu inserts in winding voids, $M_3$	&	2402 \\
Brass electrical shunts	&	162 \\
SS bandage	&	1670 \\
SS mandrel	&	2500 \\
Nb--Ti alloy in strands	&	158 \\
\hline
Total	 &	7865 \\
\hline
\multicolumn{2}{|c|}{Cooling} \\
\cline{1-2}
\hline
Operating temperature, K	& 4.8 \\
Operating pressure, MPa	& 0.3 \\
Heat load at operational condition, W & $\leq40$ \\
Heat load at energy input,	W &	$\leq 74$ \\
Nominal He mass flow rate, g/s	 &16 \\
Number of parallel cooling channels	& 20 \\
Nominal pressure drops in channel,	kPa	& $\leq 50$ \\
Pressure in cooling channel,	MPa & 	$\leq 3$ \\
Cool down time from 300 K to 4.8 K,	hours &	 $\geq50$ \\
\hline
\end{tabular}
\end{center}
\label{mag_jinr_tab2}
\end{table}%
The calculated values of the heat load on the cooling system are shown in Table \ref{mag_jinr_tab3}.

\begin{table}[htp]
\caption{Calculated values  of the heat load on the SPD magnet cooling system.}
\begin{center}
\begin{tabular}{|l|c|}
\hline
Heat inflow &  Value, W \\
\hline
Residual gases &	7.6 \\
Thermal radiation	&	6.2 \\
By suspensions	 &	14.4 \\
By current leads &	11.0 \\
\hline
Total	W &	39.2 \\
\hline
\end{tabular}
\end{center}
\label{mag_jinr_tab3}
\end{table}%


\subsection{Quench protection system}
Protection of the magnet against overheating at its transition from the superconducting state to the normal state is achieved by solenoid sectioning \cite{Wilson} and uniform dissipation of energy over the whole winding. For this purpose, the winding is divided into 20 electrical sections.
The energy stored in the magnet is dissipated both on the external resistance and on 20 shunts -- heaters, located on the inner radius of each layer of the winding. The external resistance R$_e$ = 0.04 $\Ohm$ limits the maximum voltage, with respect to ground to $\pm$100 V. The shunts divide the winding into 20 sections, in each of which a shunt made of brass tape is connected in parallel to the winding section (see Fig. \ref {Mag6}). The shunt is electrically connected in parallel to the SC cable of its section and has good thermal contact with the SC cable along its entire length, which provides a very high velocity of the normal zone propagation in the winding.
\begin{figure}[!ht]
    \center{\includegraphics[width=0.4\linewidth]{MAG_JINR_9}}
  \caption{ Electrical circuit diagram of the one section.
	}
\label{Mag6}
\end{figure}

Part of the energy released in the winding will be about 54\% of the energy stored in the solenoid or 7.9 kJ, and the time constant of the energy dissipation process will be about 13 s, calculated by the following equation:
\begin{equation}
\tau_1= L / (R_{e}+\sum R_{sec. aver.}),
\end{equation}
where $\tau_1$ is a time constant of energy dissipation, $L$ is the inductance,  $R_e$ and  $R_{sec. aver.}$ are the external resistance and  average resistance per section, respectively.

An estimated maximum heating temperature of the winding (at initial winding temperature $T_0 = 4.2$ K), as a result of its transition to the normal state (quenching) is calculated under the following assumptions: 
\begin{itemize}
\item  energy, released in the solenoid, dissipates in the superconducting wires, a copper tube, and copper inserts;
\item normal zone propagation velocity $v = \infty$.
\end{itemize}
So, 
\begin{equation}
\Delta T \approx 0.54 E / (M \times C),
\end{equation}
where $\Delta T$, K is the temperature rise after the quench at the point of origin of the normal zone; $E$ is the stored energy at maximum current $I_{max}$. $M = M_1 + M_2 + M_3$, where $M_1 = 560$ kg is the mass of copper in the SC wire, $M_2 = 413.2$ kg is the mass of the copper tube, and $M_3 = 2402$ kg is the mass of the copper inserts. $C = 39.31$ J/ (kg$\times$K) is the heat capacity of copper at an average temperature of 34.1 K. $\Delta T = 59.8$ K, thus the maximum temperature of the winding after the quench is $T_{max}=T_0+\Delta T \leq 65$ K.

\subsection{Cryostat}
The cryostat for the SPD solenoid is being developed. The design of the solenoid suspension system in the cryostat is underway. The basic characteristics of the cryostat are presented in Table \ref{mag_jinr_tab4}. 

\begin{table}[htp]
\caption{Basic characteristics of the cryostat.}
\begin{center}
\begin{tabular}{|l|c|}
\hline
Parameter & Value \\
\hline
Length, m	& 4.0 \\
\hline
\multicolumn{2}{|c|}{Diameter of the heat shield at 80 K} \\
\cline{1-2}
Inner shield, m	 & 3.305\\
Outer shield, m	 & 3.617\\
\hline
\multicolumn{2}{|c|}{SS vacuum shell diameter} \\
\cline{1-2}
Inner shell	, m&	3.175 \\
Outer shell, m&	3.767 \\
Number of solenoid supports	&	24 \\
Mass of vacuum shells, kg	&15330 \\
Mass of thermal shields, kg&	1340 \\
Total mass of the cryostat, kg&	16700 \\
\hline
\end{tabular}
\end{center}
\label{mag_jinr_tab4}
\end{table}%

The design of a Superconducting Solenoid made of a Nuclotron cable is proposed based on the technology developed at VBLHEP in the production of magnets for the Nuclotron and NICA accelerators \cite{Khodzhibagiyan:2014jma}. The use of this technology makes it possible to produce a solenoid at JINR involving enterprises of the Moscow Region. Calculations show that the solenoid will have the required field quality, the reliable cooling and quench protection system, and maintainability. Less time and money are expected to be spent for producing a solenoid using the Nuclotron technology, compared to a commercially available solenoid produced using traditional technology.


==> tex/conclusion.tex <==
\chapter{Conclusion}
The proposed physics program and the concept of the SPD facility presented in the document, are open for exciting and challenging ideas from theorists and experimentalists worldwide.  The Conceptual Design Report of the Spin Physics Detector was presented and discussed at the 54th meeting of the JINR Program Advisory Committee for Particle Physics on January 18, 2021. The following recommendations were obtained: 
{\it 
      The PAC thanks the SPD (proto-)collaboration for the preparation of the comprehensive CDR and recommends the NICA management to appoint an appropriate Detector Advisory Committee for a thorough review of the CDR and its subsequent evolution into an SPD TDR (Technical Design Report). The PAC encourages the team to pursue every effort to form an international collaboration, find adequate resources and attract students and young scientists.
}



==> tex/detector.tex <==
\chapter{Detector layout \label{ch:DL}}
\input{detector_general}
\input{magnets}
\input{beampipe}
\input{vertex}
\input{straw.tex}
\input{ECAL.tex}
\input{RS.tex}
\input{tof.tex}
\input{t0}
\input{ZDC}
%\subsection{Luminosity monitors and t0 counters}
%\subsection{Zero degree calorimeter (tagging station)}
\input{polarimetry.tex}



==> tex/detector_general.tex <==
\section{General design}

The physics tasks presented in Chapter \ref{chapter2}  impose general requirements on the concept of the Spin Physics Detector.  
Unlike the case of high-energy collisions where the collision energy $\sqrt{s}$ is a few orders of magnitude higher than a typical hard scale $Q$
of the studied reactions, at the SPD energies for all the probes planned to be used to access the gluon content of the colliding particles $Q\sim M_{J\psi} \sim 2M_{D}\sim p_{T\gamma~min}$ is just a few times less that $\sqrt{s}/2$.
Therefore, one should expect quite a uniform  distribution of all signal particles (muons from the $J/\psi$ decay, prompt photons, products of $D$-mesons decay, etc.) over the kinematic range. In other words, there is no preferable range in rapidity, which could be specified for each probe for the optimal overall performance. Together with  relatively small cross-sections of the discussed probes, this fact leads one to a requirement of $\sim4\pi$ coverage of the SPD setup.

The Spin Physics Detector must have sufficient tracking capabilities and a magnetic system for spectrometric purposes  for the majority of the addressed physics tasks. It has to be equipped with a  muon system thick enough for effective separation of muons and hadrons to make it possible to deal with the decay $J/\psi\to \mu^+\mu^-$. A precision vertex detector is needed for the recovering of the secondary vertices from the decays of $D^{\pm/0}$ mesons and other short-lived particles. An electromagnetic calorimeter ensures capability to detect signal and background photons. A low material budget and general transparency of the setup should also provide favorable conditions for the photon physics. Hadron identification capability  is needed for any physics task with protons and/or kaons in the final state, in particular,  to enforce a signal-to-background ratio for $D$-mesons selection, and also to improve tracking at low momenta.  Since tiny effects are intended to be investigated, a triggerless DAQ system is planned in order to minimize possible systematic uncertainties of the measurements.

Strict limitations to the SPD detector layout arise from the external conditions, such as the maximal possible load to the floor of the SPD experimental hall (1500 tons together with the lodgement and the detector moving system).  Together with the requirement to have the overall thickness of the muon system not less than 4 nuclear interaction lengths ($\Lambda_I$), this limits the outer size of the SPD detector and the size of the inner part of the detector. The location of the collider infrastructure, in particular, focusing elements, also defines the size of the SPD setup along the beam axis. 
More details could be found in Chapter \ref{chap:beams}.

%The design concept of a detector which would be capable to exploit the broad spin physics potential of the high luminosity NICA collider is a one of the main task of the project. 
%The proposed detector design would meet with set of requirements developed on basic the main physics
%programme tasks given in Chapter 1 and in \cite{Savin:2014sva}:
The general layout of the SPD is shown schematically in Fig. \ref{fig:spd1}. The detailed description of each subsystem could be found below. Table \ref{tab:main_det} brings together the elements of the SPD physics program and the requirements to the experimental setup.  We would like to  emphasize here that the most part of the SPD gluon program can not be performed at MPD \cite{MPD_CDR}, another detector at the NICA collider, optimized for operation  at a high multiplicity of charged tracks and relatively low luminosity.

%\begin{figure}
%\begin{center}
%\includegraphics[scale=0.6]{SPD_sketch.png}
%\caption{General layout of the Spin Physics Detector.}
%\label{fig:spd1}
%\end{center}
%\end{figure}

\begin{figure}[!h]
\begin{center}
  \begin{minipage}[ht]{0.56\linewidth}
    \center{\includegraphics[width=1\linewidth]{det1} }
  \end{minipage}
  \hfill
  \begin{minipage}[ht]{0.6\linewidth}
    \center{\includegraphics[width=1\linewidth]{det22}}
  \end{minipage}
  \caption{General layout of the Spin Physics Detector. All dimensions are in millimeters.}
  \label{fig:spd1}  
\end{center}
\end{figure}

\begin{table}[htp]
\caption{Required setup configuration for each  point of the SPD physics program. (+++) - absolutely needed, (++) - extremely useful,
(+) - useful, (-) - not needed.}
\begin{center}
\begin{tabular}{|l|c|c|c|c|c|c|c|c|}
\hline

Program & Vertex     & Straw   & PID      & Electromagnetic & Beam-beam &  Range  \\
               & detector  & tracker & system & calorimeter         & counter         &   system        \\
\hline
\hline
%\cellcolor{yellow}
Gluon content with:&            &           &               &                       &                     &           \\
~~~charmonia &    +   &    ++       &   +           &    ++               & +                  &    +++     \\   
~~~open charm&   +++ &  ++       & ++          &    +                  & +                  &    ++     \\
~~~prompt photons& +& +         &  -            &   +++               & +                  &    -      \\
\hline
SSA for $\pi$ and $K$& + & ++  &   +++      &    ++                & +                  &    -     \\
Light vector meson production & +& ++ &  -         &    +                  & +                  &  - \\
Elastic scattering                    &  +  &  ++ & -        &     -           &  +++             &   -  \\
$\bar{p}$ production       &      +     & ++   &  +++   &  ++         &   +                &  -   \\
Physics with light ions    &    ++     & +++ &  +       &  ++         &   ++                &  +   \\
\hline                 

\end{tabular}
\end{center}
\label{tab:main_det}
\end{table}%



==> tex/synchNICA.tex <==
\section{Synchronization with NICA}
\label{sect:daq-synchNICA}

At the moment of writing this we assume the WR will be used by NICA to clock
synchronization but not for collider rings control.

We need the time of bunch crossings:
\begin{itemize}
\item With accuracy at least 1~ns or better.
(This means that we can't simply use WR TAI timestamp as bunch
crossing time because former has 8 (16?)~ns granularity corresponding to 125
(62.5)~MHz WR frequency.)
\item Incorporated into frames and slices of data structure produced by the SPD DAQ.
(This means time of each
bunch crossing could be calculated by online filter software using the same
procedure as described in
\ref{sect:daq-sync_and_time}th
section
% of the TDR DAQ chapter
for any regular hit timestamp.)
\end{itemize}

Such requirements could be satisfied if:\\
- some periodic signal with radio frequency (RF) of bunch crossings, synchronous
with them, and with known (or already aligned) propagation delay will be
measured anywhere in the SPD
by some non-expensive TDC of 0.5--1~ns resolution.

With the proposed slice duration of 10--100~\textmu{}s and nominal RF period
of $\sim 76$~ns the required TDC clock counter depth is 12~bit.
Because the RF should be very stable during each filling of collider rings,
we could reduce the data rate of bunch crossing timestamps simply by down-scaling
input RF signal with the factor of 10 or 100, which leaves 132 or 13 bunch
crossing timestamps
per slice, what seems enough for online filter software. Also the required
counter depth will be decreased to 9 or 6 bits respectively. However RF depends
on beam energy and as such could be differ from run to run instead of WR
frequency so can't be transferred by means of WR. Of course, NICA and SPD
global clocks synchronization by WR could be still required for other reasons.

Let's note this approach (measurement by TDC) could be used also for any
periodic or non-periodic events ($T_0$, some trigger conditions, etc.) needed
to be registered as time references in the data stream produced by the SPD DAQ.
Seems this is only way to do so in the self-triggered (free-running) DAQ.
So possibly we need to equip some fictitious 'sub-detector' by 8--32 channels
TDC for these purposes.


